Hijacking Bitcoin: Routing Attacks on Cryptocurrencies

As the most successful cryptocurrency to date, Bitcoin constitutes a target of choice for attackers. While many attack vectors have already been uncovered, one important vector has been left out though: attacking the currency via the Internet routing infrastructure itself. Indeed, by manipulating routing advertisements (BGP hijacks) or by naturally intercepting traffic, Autonomous Systems (ASes) can intercept and manipulate a large fraction of Bitcoin traffic. This paper presents the first taxonomy of routing attacks and their impact on Bitcoin, considering both small-scale attacks, targeting individual nodes, and large-scale attacks, targeting the network as a whole. While challenging, we show that two key properties make routing attacks practical: (i) the efficiency of routing manipulation; and (ii) the significant centralization of Bitcoin in terms of mining and routing. Specifically, we find that any network attacker can hijack few (<100) BGP prefixes to isolate ~50% of the mining power---even when considering that mining pools are heavily multi-homed. We also show that on-path network attackers can considerably slow down block propagation by interfering with few key Bitcoin messages. We demonstrate the feasibility of each attack against the deployed Bitcoin software. We also quantify their effectiveness on the current Bitcoin topology using data collected from a Bitcoin supernode combined with BGP routing data. The potential damage to Bitcoin is worrying. By isolating parts of the network or delaying block propagation, attackers can cause a significant amount of mining power to be wasted, leading to revenue losses and enabling a wide range of exploits such as double spending. To prevent such effects in practice, we provide both short and long-term countermeasures, some of which can be deployed immediately.

==> interception.tex <==
\section{Measurement Analysis - Insides}
\label{sec:topology}

In this section, we explain the datasets and the techniques used to infer the
Internet and Bitcoin topologies including a thorough study of mining pools
connectivity.

We inferred our datasets in four steps. First, we obtained the AS-level
topology and AS-to-AS forwarding paths using BGP control-plane information.
Second, we collected the bitcoin IPs of the public nodes using a supernode.
Third, we assigned mining power to pools. Fourth, we mapped the connectivity of
each pool using its Stratum servers along with delay information collected by
our supernode which enables us to study the impact of routing attacks in
function of the multihoming degree of pools.

We now describe each step as well as the datasets used. Our full dataset spans
between October 2015 and March 2016. As the results of our analysis
do not change much through time, we focus on the results computed over a 10-days period between November 5 and November 2015 unless noted otherwise.

\myitem{Step 1: BGP AS-level topology and AS-to-AS forwarding paths} We
collected \emph{2.5 million} BGP routes (covering all Internet prefixes) along
with \emph{4 billion} BGP updates advertised on 182 BGP sessions maintained by
3 RIPE BGP collectors~\cite{ripe:ris} (rrc00, rrc01 and rrc03). We collected
these routes and updates daily, for 4 months, between Oct 2015 and Jan 2016. We
also collected inferred AS-level topologies computed by
CAIDA~\cite{caida_as_level}. An AS-level topology is an undirected graph, in
which a node corresponds to an AS and a link represents an inter-domain
connection between two neighboring ASes. Links are labeled with the business
relationship linking the two ASes (customer, peer or provider). Using this
data, we computed the forwarding path taken by each AS following the routing
tree algorithm described
in~\cite{goldberg_how_secure_are_interdomain_routing_protocols}, which takes
into account the business relationships between ASes.

%Using this data, we identified which AS is hosting each Bitcoin node by mapping
%its IP address with the AS advertising the most-specific covering prefix. To
%protect our mapping from BGP hijacks, we only consider prefixes that have been
%advertised consecutively for at least one day. We then computed the sequence of
%ASes traversed when any two Bitcoin nodes communicate. 

\myitem{Step 2: Bitcoin nodes IP addresses} Each day, for 10 days, we collected
around 6{,}000 IP addresses of Bitcoin nodes using a Bitcoin supernode which
continuously crawled the Bitcoin network to discover new nodes. Our supernode
connected to approximately 2{,}000 bitcoin nodes per day (with a mean of 2174
and a median of 1875). It saw a total of 7{,}477 distinct IPs during the 10
days and was relayed a total of 1{,}440 blocks. By combining this dataset with the BGP one, we then created  node-to-AS mapping
each Bitcoin IP address to the origin AS advertising the most-specific prefix
covering it, giving us a .

%The list of IP addresses is available online~\cite{bitcoinstats_census}.

\myitem{Step 3: Mining pools distribution} We collected the
list of mining pools along with the blocks they mined using publicly-available
statistics computed on the blockchain~\cite{blockchain}. We then attributed a
share of the total mining power to each pool proportionately to the blocks
mined by the pool during the 10 days. As highlighted by previous
studies~\cite{pools,miller2015discovering}, mining power is highly skewed, with
{\raise.17ex\hbox{$\scriptstyle\sim$}}70\% of the mining power held by four
mining pools: F2Pool (21\%), AntPool (19\%), Bitfurry (15\%) and BTCC
(13\%).

\myitem{Step 4: Mining pools connectivity} For each mining pool, we
inferred the AS it uses to interconnect to the Bitcoin network. We assign pools
to ASes, taking into account multi-homing, in two consecutive steps: \emph{(i)}
considering the location of their (publicly known) Stratum server; and
\emph{(ii)} by using block propagation information crawled by our supernode.

As described in Section~\ref{sec:background}, Stratum servers are publicly
known servers used by miners to connect to the pools.
Coinscope~\cite{miller2015discovering} noted that Stratum servers tend to be
co-located in the same AS as the pools gateway to the Bitcoin network. We
therefore assign pools to ASes using the public IPs of the Stratum servers.
Overall, we found more than thirty IPs pertaining to the fifteen largest pools
by searching their websites and/or by connecting directly to them.

Relying only stratum servers to infer the gateways result in only few pools
being multi-homed. As in practice pools tend to be
multi-homed~\cite{miller2015discovering}, we augmented our pool-to-AS mapping
by considering the timing of the \textsf{INV} messages received by our
super-node. In particular, we considered that pool gateways are most likely to
be the first to learn about the blocks each pool mines. As such, we infer the
position of extra gateway nodes used by a pool by tracking down the number of
times a node is amongst the first ones to propagate a block mined by that pool.
To avoid outliers, we only consider a node as possible gateway for a pool only
if it has relayed blocks of that pool more than once during the 10-days time
frame. Using this technique, we mapped each pool to all the nodes located in (a
maximum of) 1,5,10,15 ASes by selecting the most frequent nodes in descendent
order.

\laurent{Clarify all these levels: IPs, nodes, ASes, it is not very clear at which one we operate right now.}





\begin{table}[t]
\centering
\small
\def\arraystretch{1.1}
\begin{tabular}{@{}lccccc@{}}
\toprule
%Attack && Active(How much) && Passive(Who can) &&  \% ForkRate && Implications\\
\textbf{Degree of multi-homing} && {\emph{1}} & \emph{5} & {\emph{10}} & \emph{15} \\
\color{gray}{\# ASes used to access the Bitcoin network} && & & & \\
\midrule
\textbf{F2Pool} && 1 & 10 &  16 & 22  \\
\textbf{AntPool} && 1  & 8 &  17 & 23 \\
\textbf{Bitfurry} && 1  & 5 &  13 & 19  \\
\textbf{BTCC}  && 1 & 6 &  11 & 17  \\
\bottomrule
\end{tabular}
\caption{Number of gateways for each of the four biggest pools as a function of the degree of multi-homing they adopt.}
\label{tab:ips}
\end{table}






\begin{figure}[t]
 \centering
 \includegraphics[width=.65\columnwidth]{figures/nb_hijacks_required_pools}
 \caption{The number of prefixes to hijack needed to isolate a mining pool increases as they get better connected. Yet, hijacking only 246 prefixes is enough to isolate F2Pool, the largest pool with 21\% of the mining power. Overall, hijacking less than 400 prefixes is needed to isolate 50\% of the mining power assuming pools are multi-homed in 15 ASes. This is \emph{well} within what is currently seen in the Internet (see Fig.~\ref{fig:hijack_number}).}
 \label{fig:interception_pools}
\end{figure}

%%
%%
%%%% SECTION BEGINNING
%%
%%

We start the section with describing some key-characteristics of the bitcoin network that enable passive and active attackers to intercept a large amount of bitcoin traffic ~\ref{ssec:bitcoin_topology}. As passive adversaries have no control of which connections they will intercept, we elaborate only on how active adversaries can pick a suitable set of prefixes to hijack to increase their effectiveness in ~\ref{ssec:active_interception_attacks}.



\subsection{Measurement analysis}
\label{ssec:bitcoin_topology}



 In the  following we summarize the characteristics that render the network extremely vulnerable to AS-level adversaries. results are based on routing and Bitcoin measurements described described in Section~\ref{sec:datasets}



\myitem{The Bitcoin network is \emph{extremely} centralized} Very few ASes host the
majority of the nodes in the network. Fig.~\ref{fig:cdf_bitcoin_per_ases} depicts the
cumulative fraction of Bitcoin nodes as a function of the number of hosting
ASes. We see that only 13 (\emph{resp.} 50) ASes host 30\% (\emph{resp.} 50\%) of the entire
Bitcoin network. %Table~\ref{tab:ases_number_ranking} lists the top 10 ASes in terms of
%hosted number of nodes. 
These ASes pertain to broadband providers such as Comcast (US), Verizon (US) or Chinanet (CN) as well as to cloud providers such as Hetzner (DE), OVH (FR) and Amazon (US). We observe the same kind of concentration, at the distribution of Bitcoin nodes per IP prefix: only 63 prefixes
(0.012\% of the Internet) host 20\% of the network.

\begin{figure}[t]
 \centering
 \begin{subfigure}[t]{0.47\columnwidth}
\includegraphics[width=.9\columnwidth]{figures/bitcoin_per_ases_cummulative}
	 \caption{Only
13 ASes host 30\% of the entire network, while 50 ASes host 50\% of the
network.}
	 \label{fig:cdf_bitcoin_per_ases}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.47\columnwidth} 	\includegraphics[width=.9\columnwidth]{figures/crossed_connections_per_as_cummulative}
	 \caption{Few ASes intercept large percentages of Bitcoin traffic: 3 of them intercept 60\% of all possible Bitcoin connections.}
	 \label{fig:cdf_connection_per_ases}
 \end{subfigure}
 \caption{Bitcoin is heavily centralized from a routing viewpoint.}
 \label{fig:centralization}
\end{figure}
%(Hurricane, Level3 and Telianet)

\myitem{Few ASes see a substantial part of Bitcoin traffic}
Fig.~\ref{fig:ases_connections} depicts the cumulative percentage of
connections that can be intercepted by an increasing number of ASes
(\emph{e.g.}, by colluding with each other). We see that only \emph{three}
ASes, namely Hurricane Electric, Level3, and Telianet, can together intercept
\emph{more than 80\% of all possible Bitcoin connections}, with Hurricane alone
being on path for 32\% of all connections. In general, large transit
providers (\emph{i.e.}, Tier-1s) are traversed by a large fraction of all Bitcoin connections.

%Table~\ref{tab:ases_ranking_connections} lists the top 7 ASes in terms of the
%percentage of total connections they can intercept. We see that large transit
%providers (\emph{i.e.}, Tier-1s) are traversed by a large fraction of
%all Bitcoin connections.

\myitem{$>$90\% of Bitcoin nodes are vulnerable to hijacks} 93\% of all
prefixes hosting Bitcoin nodes are shorter than /24, making them vulnerable to
a global IP hijack using more-specific announcements. Indeed, prefixes strictly
longer than /24 are typically filtered by default by many ISPs. Note that the
remaining 7\% of nodes that are in /24 prefixes are \emph{not} necessarily
safe. These can still be hijacked by another AS performing a shortest-path
attack, i.e., the attacker, who will advertise a /24 just like the victim will
attract traffic from all ASes that are closer to it than they are to the victim
(in terms of number of hops).
%This will, on average, allow him to hijack traffic to the
%victim from around half of the internet.
 %(but really depends on the exact topology).

\myitem{Bitcoin routing properties are stable} While numerous nodes join and
leave the Bitcoin network all the time, the routing properties highlighted in
this section are stable. For validation, we ran our analysis daily over a 4
month period, during which the same IPs were present on average for 15.2
consecutive days (excluding IPs that were seen only once). Moreover, our
observations regarding the network's centrality are also extremely stable: 50
ASes hosted each day 49.5\% of Bitcoin clients (standard deviation: 1.2\%)
while 24.7\% of Bitcoin nodes are found daily in just 100 prefixes (standard
deviation: 1.77\%).

\subsection{Actively Interception attacks using centralization}
\label{ssec:active_interception_attacks}
%who?
In this section we show how an active or hybrid adversary can overcome the challenges of multi-homing, NATed nodes, and relays as well as reduce the cost of the attack in diverted bandwidth and number hijacked of prefixes. 
%how
We particularly focus on a 50\% partition, intuitively any smaller partition is easier to be formed.








Active attackers are able to completely isolate
any set containing regular nodes or/and multi-homed pools, effectively creating a 
partition of nodes or mining power respectively even as large as 50\%. 
For isolating any set of regular nodes an AS adversary would need to 
intercept all their traffic. By hijacking all the prefixes of these nodes the attacker 
intercept all traffic destined to them. As such the attacker can simply prevent them 
from connecting to any node outside the set.
For isolating a pool an attacker needs to make sure  all  
gateways of a pool are hijacked. For that an AS adversary would need to know all gateways belonging to the pools he wants to include in the isolated set. 




\myitem{NATed or hidden nodes cannot bridge the partition.}
NATed nodes can only connect to public IPs. By hijacking the prefixes corresponding to a 
partition, the attacker gains control over every connection crossing it, including the 
ones from NATed nodes. By killing any bitcoin connection crossing the partition, the 
attacker effectively disconnects any bridge created by a NATed node. 

\myitem{New nodes that join the network cannot bridge the partition.}
New nodes that are in the hijacked prefixes would 
have all their connection to the other side of the partition dropped by the attacker.
Similarly nodes that are not in the hijacked partition would never be allowed to connect to
the hijacked side.

\myitem{Bitcoin relays ~\cite{relays} cannot guarantee the security of the protocol.}
They indeed improve the performance of Bitcoin. They might even be able to secure bitcoin 
against known attacks but they are still far from guaranteeing routing security. Indeed, 
the IPs of the relays are publicly available; ISPs are sometimes chosen based on pricing (
acknowledged on the website), and BGPSec is not used. All these facts make relays also 
vulnerable to both hijacking and passive attacks.

\myitem{Multi-homed pools do not prevent a partition}
Indeed multi-homing is a practice which make the network much more robust to routing 
adversaries. Even so, an active attacker can hijack all gateways of a pool effectively 
placing the whole pool in one side of the partition, given that the attacker knows the 
complete set of gateways of that pool.
In Section~\ref{sec:discussion} we further investigate how an attacker can use hijacking to discover unknown or hidden gateways.
 

\myitem{nodes in the same AS should be in one side}
Nodes in the same AS should be either all included in isolated set or all excluded from it. 
 This is because an active attacker cannot intercept the communication between nodes in the same AS. For instance in Figure~\ref{fig:overview} assume that nodes A and B have IPs 1.0.1.2 and 1.0.2.2, these belong to different /24 prefixes. If the attacker hijacks only 1.0.1.0/24 he would intercept all traffic destined to A except from the traffic from B to A. This essentially means that if the two nodes are placed in different parts of a partition they would act as a bridge if they connect to each other. Thus, in the following we assume that an attacker either hijacks all prefixes with bitcoin nodes of an AS or none. 



%

After ensuring a complete cut between the two parts The attacker's goal is to lower its footprint,
\emph{i.e.} the amount of prefixes hijacked. In the following we explain the methodology we used to estimate the smallest amount of prefixes needed to create partitions of diffrent sizes.
We always consider
the
extreme case, in which the AS-level adversary: \emph{i)} does not see \emph{any} traffic
naturally; and \emph{ii)} does not host any Bitcoin nodes.
Especially for the partition of mining power we further investigate the influence of multi-homing degree per pool in the cost of such a partition.

 
\myitem {Estimating the cost of isolating mining power.}
For each mapping of IPs to a pool we calculate the cost of isolating it in number of prefixes 
that need to be hijacked. The exact results for the four biggest pools under five 
assumptions regarding the degree of multi-homing are 
presented in Table~\ref{tab:hijacks50}  Due to the concentration of bitcoin from the 
routing perspective we found 
significant overlap among the required hijacked prefixes to isolate distinct pools. As such 
the cost of a largest partition is considerably limited in comparison to the sum of prefixes 
required per pool. We present the results for partitions containing from 49\% to 50\% of mining power. Intuitively there are smaller partitions that require  require less prefixes. We calculated these numbers using exhaustive search over all the subsets of pools partitions of 49\% to 51\% and picked the one with the least required prefixes. We found that 
only 381 prefixes needed to be hijacked even in the extreme case that the four biggest 
pools accounting for almost 70\% of mining power are hosted in 15 ASes each. When considering lower degree of multi-homing such as 5 ASes per pool  the number is reduced to half.

\myitem {Estimating the cost of isolating regular 
nodes.} For each AS with bitcoin nodes we assign a score that equals to the ratio of the number of nodes nodes it
contains over the number of prefixes with Bitcoin nodes it advertises. The
attacker then hijacks the ASes with the higher scores first. We found that \emph{870 prefixes} need to be hijacked to isolate 50\% of the public bitcoin nodes while 119 hijacked [refix would isolate 20\% of the public bitcoin nodes.% until reaching 50\% of all mining power.



\myitem{Dealing with hijacked bandwidth}
While deciding the right prefixes to hijack an attacker should also take bandwidth demands associated with the hijacked prefixes into consideration. In light of that the attacker might prefer to increase the hijacked prefixes to decrease the traffic that would be diverted to his infrastructure even if such a practice requires hijacking more prefixes. 
Going back to our example in figure ~\ref{fig:overview} if AS8 can indeed hijack one prefix namely 1.0.0.1/16 to intercept all traffic destine to nodes A and B. In this case the attacker would have to deal with all the traffic destined to a /16 prefix. However if A and B belong to a common more specific prefix then an attacker would for sure prefer to hijack this one as the diverted load would be less. The attacker can reduce the load even further by advertising only /24 prefixes even if that means he needs to advertise more prefixes. 

 \laurent{Rephrase the above in lights of the hijack study}.




%Indeed, almost of all of the mining power
%is distributed in only 20 pools, 7 of which together reach 88\%. From the
%network perspective, mining pools are \emph{even more centralized} with 15 ASes
%(in the \emph{distributed} case) or 13 (in the \emph{centralized} case) hosting
%90\% of mining power.



\myitem{Hybrid attackers} 
%
In practice, nothing prevents AS-level adversaries to combine active and passive
attacks to reduce their footprint even
further. To give an idea of such approach we present what the cost of creating the same partitioning would be if performed by the AS that was harder to hijack  (require more prefixes). For isolating 50\% of the nodes , X
prefixes are enough for a hybrid attacker. For isolating 50\% of mining power a hybrid attacker would need 13, 123,253 and 337 prefixes under the assumption that mining pools are hosted at most at 1,5,10 and 15 ASes respectively.  







\begin{table}[t]
	\centering
	\small
	\def\arraystretch{1.1}
	\begin{tabular}{@{}lclcccc@{}}
		\toprule
		\cmidrule(lr){5-6}
		\textbf{Country} && \textbf{Connections} (\%) && \emph{Partition regular nodes} \\			
		\midrule
		US && 89.8 && 37.0 \\
		DE && 32.8 && 8.8  \\
		GB && 31.4 && 5.4  \\
		SE && 26.7 && 2.0  \\
		CN && 12.2 && 5.4  \\
%		HK && 11.3 && 0.7 && 0.0 \\
		\bottomrule
	\end{tabular}
	\caption{Cumulated power ASes in the same country have over Bitcoin measured in \% of connections they intercept and the most disruptive partition of regular nodes they can achieve. \laurent{Update results} %Values are computed assuming a complete graph ie each node is connected to every other  
	}
	\label{tab:country_partition}
\end{table}











==> partition.tex <==
\section{Partitioning Bitcoin }
\label{sec:partition}

In this section we will extensively describe how an attacker plans, enforces and maintains a partition.
For clarifying the procedure we included a piece of pseudo-code summarizing the most important steps of the attack which we explain in detail in the following.

\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother

\begin{algorithm}
\caption{Create an effective partition}\label{euclid}
\begin{algorithmic}[1]
\algrenewcomment[1]{\(\triangleright\) #1}

%import bitcoin node IPs
%hijacked\_nodes;;;;

\Procedure{Partition}{}


\Comment{ \textbf{Attack Planning}} \ref{ssec:plan}

\State $\textit{IP\_list} \gets \text{list of IPs of bitcoin nodes }$




\State  $\textit{hijacked\_nodes} \gets \textit{pick\_component(IP\_list)}$


\Comment {\textbf{ Disconnect }} \ref{sssec:disconnect}

\For{each node $n$ in $hijacked\_nodes$}
%\State \texttt{<do stuff>}
\For{each node $p$ in $n.peers$}
\If {$p$ not in $hijacked\_nodes$}
\State drop connection(p, n)

\EndIf
\EndFor
\EndFor


\Comment {\textbf{ Maintain partition }} \ref{sssec:leakage}
\While {true}

%while true: if leakage is detected:
%node= leakahe
\State $\textit{node} \gets \text{Detect\_leakage()}$

\For{each node $p$ in $node.peers$}
\If {$p$  in $hijacked\_nodes$}
\State drop connection(p, node)
\EndIf
\EndFor
\EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{\textbf{Attack Planning}}
\label{ssec:plan}
We first look at how the attacker prepares his attack. The preparation phase includes two phases: \emph{(i)} discovering IPs of active bitcoin nodes;  \emph{(ii)} deciding on a partition.



\subsubsection{\textbf{Phase \#1: Inferring topology}} 


\label{ssec:augement_topo}

During this phase the attacker composes a list the active bitcoin nodes' IPs. Optimally, this list is accompanied with some of the gateways of known pools. We will refer to this information as topology. The attacker can simply downloading such a list from one of the known bitcoin sites to infer the topology \cite{bitnodes}. The effectiveness of the attacker though, can be significantly increased, had he used a more precise topology. To do that the attacker can
 discover more nodes and/or identify the pool gateways in the topology. 

Before mentioning some of the ways an attacker can discover more nodes we look at the reasons why the publicly available lists might be incomplete. Nodes that do not accept incoming connections to prevent DDoS attacks or just because they are behind a NAT, as well as nodes that are very new to the network are most likely not included in those list. That is due to the way nodes are discovered and of the time a complete crawling of the network takes. Among other things, the attacker could very easily use the following two methods to discover unknown nodes. First, the attacker can by itself have some bitcoin nodes which it uses to learn more IPs. Even a node that does not accept incoming connections is indeed connected to some nodes which are likely to advertise its IP via \textsf{ADDR} messages. Second, the attacker could combine different sources of information such as multiple sites as well as multiple consecutive versions of lists from the same source. Different source might have different ways of collecting the IPs and also combining information from multiples time frames limits the risk of not including nodes that were not active just during the crawling.


In addition, it would be also useful for the attacker to identify nodes as gateways of specific pools. This information can significantly help him in planning the partition as we will explain in the following Subsection \ref{ssec:plan} . To do that the attacker can use the techniques described in research papers such as \cite{coinscope} and/or leverage the access he can obtain to bitcoin traffic via hijacking as an active way to learn the topology. We briefly introduce two such methods.
First, the attacker may hijack the pool's stratum servers to discover connections that they establish and thus reveal the gateways they connect to. Connections to formed between the pool's stratum server and its gateways are via bitcoind's RPC access, and can be easily distinguished.
Second, the attacker can hijack the relay network to discover connections used by the large mining pools. The relay network has a public set of six IPs that pools connect to. By hijacking these, one may learn very critical points of the pool's infrastructure. Specifically, it will not be hard to identify a pool by observing the blocks it publishes to the relay network. 



\subsubsection{\textbf{Phase \#2: Finding a cut}}
\label{ssec:plan}


During this phase, the attacker decides which nodes one of the two components contains. The goal of the attacker is to find a partition that is more likely to be effective. We will first discus which partitions are effective as well as how the attacker can approximate such a partition.

%\myitem{Effective partition}
 The main threat of a partition's effectiveness is leakage. Leakage can occur when two nodes in different components are connected through a channel that the attacker cannot intercept. If all those connections (all pairs of nodes with such connections) are within one component the corresponding  partition is effective.
 We distinguish three types of connections the attacker cannot intercept: \emph{(i)} intra-AS connections;  \emph{(ii)} intra-pool connections; \emph{(iii)} direct pool to pool connections.

\myitem{intra-AS} Connection within the same AS cannot be intercepted by the attacker because their traffic is local to the AS and will thus not leave the AS.\maria{@laurent can you say it better?} For example, in Figure \maria{FILLME} nodes A and B are in the same AS. The traffic between them will never get outside of their AS even during a hijack. This situation can be problematic for the partition, if nodes A and B connect to each other and belong to different components of the partition. In this case they will exchange the state of the components they belong to, effectively leaking information from one component to the other. To address this issue the attacker would always put nodes of the same AS in the same component. This can be easily guaranteed as the attacker can easily infer which AS each IP is hosted to.

\myitem{intra-pool} Connections among nodes that belong to the same pool cannot be intercepted because they might use proprietary protocols. Since mining pools are multi-homed and distributed among different locations, their gateways might be hosted in different ASes, which can of course be placed in different components. If that happens, the pool they belong would get information from both components and probably disseminate this information from one component to the other, effectively acting as a bridge between them. For example in Figure \maria{FILLME} if AS1 is placed in one component and AS2 in the other then the green pool will get information from both components. The green pool then can instruct its gateways nodes E and D to propagate the learned information from E to D and from C to B. In this case, although there is no bitcoin connection crossing the partition the two components will still be connected. 
Intuitively, the attacker would need to include all gateways of a pool in the same component to address this issue. If the attacker is aware of all the gateways of a pool, he can easily avoid this indecent. If the attacker only knows some of the gateways or none at all, he can still try a partition and modify it on-the-fly until it is effective. We explain this procedure in \ref{sssec:leakage}.  


\myitem{Pool to Pool} 
Some pools might connect directly to each other with protocols different than bitcoin. Such a mesh connecting many large pools today is the bitcoin relays. 
Since the IPs of the relays are publicly available and the BGPsec is not used the attacker can hijack the relays and easily disconnect them. Note that this is different from a DoS attack directed to the IPs of relays, which are indeed easier to handle.
If pools have secret agreements to each other then they should be both placed in the same component. That cannot be done a priori as the attacker might not have  that information. However, the attacker can still infer such relations on-the-fly as explained in \ref{sssec:leakage} \maria{should we say here about the security/ obscurity?}


\subsection{\textbf{During the attack}}



The actual attack can be split into two phases. In the former phase the attacker cuts all connections between nodes of different components. In the latter phase the attacker continually detects leakage and disconnect its source from one of the component.


\subsubsection{\textbf{Phase \#1: Disconnect}}
\label{sssec:disconnect}

 Once the attacker decides on a partition, he needs to hijack all the prefixes that correspond to nodes in one of the components. We will refer to these nodes as hijacked nodes, the component they belong to as hijacked component and the ASes these nodes are hosted in as hijacked ASes. 

 The attacker will receive the traffic that is destined to the nodes whose prefixes he hijacked. At this point, he distinguishes the bitcoin traffic from the regular and investigate it further before sending it to the actual destination. From this traffic the attacker can discover all the connections the hijacked nodes have. He then classifies the connections each hijacked node has as one of three types: \emph{(i)} connections to peers hosted in hijacked prefixes; \emph{(ii)} connections to peers hosted in hijacked ASes but whose prefixes are not yet hijacked; \emph{(iii)}connections to peers hosted in hijacked ASes that are not hijacked. Connections are treated differently based on their type.
The first type of connections are entirely within the hijacked component and are thus allowed by the attacker. With regards to the second type, the existence of a peer hosted within the hijacked ASes, but whose prefix is not hijacked denotes that the attacker was unaware of this node. Since the attacker needs to include all nodes of an AS within the same component, the attacker would have to hijack the prefix of the sofar-unknown node as well. After that the connection would be allowed as it will be classified to the first type of connections. 
The third type of connections are connections that cross the partition. The attacker would drop such connections. If the connections was initially established by the hijacked node, it will try to establish a new connection to replace the dropped one. The new connection would be again classified and treated as described above.




\subsubsection{\textbf{Phase \#2: Partition Maintenance}}
\label{sssec:leakage}



 The methodology described above is enforced throughout the attack to ensure that there is no connection the attacker can control that crosses the partition. Even so, there will be connections that the attacker would not be able to intercept and do cross it. Thus the attacker would need to first detect the end of the connection that is within the hijacked component and then disconnect it from the rest of the nodes of this component.

Particularly, if there is a node within the hijacked nodes that is connected to the other component, it will learn about blocks that are mined in the other component. To propagate these blocks to nodes within the hijacked component it would first send an inventory message with the block's hash to a node in the component. As the attacker sees all traffic to the hijacked nodes and the hijacked nodes are only connected to each other, he sees all exchanged traffic/information within the partition. Once the attacker sees the hash being advertise he concludes that the sender has a connections to the other component. To avoid leakage of information from this node to the hijacked component the attacker cuts all its connections to the hijacked nodes. If the node never tries to propagate the block, it will indeed never be detected, but it will also never cause leakage, in which case it is not a threat for the partition. 
As the node might also have connections that the attacker cannot intercept within the hijacked component, cutting its bitcoin connections to hijacked nodes might not be enough to stop the leakage. In this case the nodes it is connected to will be also detected as points of leakage and excluded from the hijacked component. 


%when does leakage happen
%when is it dangerous for the partition




\remove{


\subsubsection{Why leakage can occur}

\myitem{The attacker might have an incomplete or obsolete topology view.}
In othe r owrds the attacker might not be aware of the existance of node X.
Node X who is hosted in ASX and routed according to PrefX can bridge the partition if and only if all the following hold
\begin{itemize}
\item ASX is within the isolated-hijacked part (if it is in the other half X will never be allowed to connect to any of the isolated nodes)
\item There is no other node is in the same prefX (if there is prefX is already hijacked)
\item X connected to at least one node in ASX (unlike to happen based on the prefix preference in bitcoind)
\item X connected to at least one node from the other part (to act as a bridge)
\end{itemize}

\myitem{Mining pools are mostly multi-homed and their internal structure and/or protocols are private and complex.}
This can be problematic for the partition if there is an unknown gateway unknown gateway G of pool X in ASX such that:
\begin{itemize}
\item G belongs to the isolated part
\item ASX is not in the isolated part 
\end{itemize}


  (b) Mining pools are mostly multi-homed and their internal structure and/or protocols are private and complex. (c)Hijacks cannot divert inra-AS traffic.






\subsection{Limitations -Leakage}

\subsubsection{Circumstances that can break the partition}

\myitem{a node X hosted in ASX and routed according to PrefX can break the partition iff}
\begin{itemize}
\item X is a new node (otherwise the adversary would know based on the assumptions and would have hijackes its prefix) \maria{maybe remove that to talk about pre-attack plans}
\item ASX is within the isolated-hijacked part (if it is in the other half X will never be allowed to connect to any of the isolated nodes)
\item There is no other node is in the same prefX (if there is prefX is already hijacked)
\item X connected to at least one node in ASX (unlike to happen based on the prefix preference in bitcoind)
\item X connected to at least one node from the other part (to act as a bridge)
\end{itemize}


\maria{not sure if we want to include this case , maybe it is covered by the assuption that the attacker knows the topology }

\myitem{secret agreement between pools in different parts}
The partition is not feasible the two pools must be seen as one. The attacker has to find another partition or drain all the hijacked traffic. But we focus on the default protocol



\subsubsection{Circumstances that cannot break the partition}
\maria{or find a way to include this cases above}



\myitem{NATed or hidden nodes cannot bridge the partition.}
NATed nodes can only connect to public IPs. By hijacking the prefixes corresponding to a 
partition, the attacker gains control over every connection crossing it, including the 
ones from NATed nodes. By killing any bitcoin connection crossing the partition, the 
attacker effectively disconnects any bridge created by a NATed node. 


\myitem{Bitcoin relays ~\cite{relays} cannot guarantee the security of the protocol.}
They indeed improve the performance of Bitcoin. They might even be able to secure bitcoin 
against known attacks but they are still far from guaranteeing routing security. Indeed, 
the IPs of the relays are publicly available; ISPs are sometimes chosen based on pricing (
acknowledged on the website), and BGPSec is not used. All these facts make relays also 
vulnerable to both hijacking and passive attacks.


\subsection{Detecting leakage}


\subsection{Reacting to leakage}
\begin{itemize}
\item increase hijacked prefixes randomly or based on the address books of nodes look for nodes even though they do not seem active at the moment  (new node)
\item analyze Stratum server (and relays) traffic to find which are the nodes they communicate with (new gateway)
\item act as a black hole (secret agreement)
\item recalculate a feasible partition assuming two pools as one (secret agreement)
\end{itemize}

\maria{In general this part is weak I think we should avoid saying that we do staff to discover the topology}
}







==> results.tex <==
\section{Simulation Results}
\label{sec:results}

\subsection{Validation Metrics}
Some of the simulation parameters are slightly modified for the needs of each attack and topology. For that reason  each time we study an attack scenario we will run the same simulation assuming there is  no network adversary. The measured values in the extra run is then compared to the corresponding values when an attack takes place to depict the impact of the attack and to the ground truth, to measure the reliability of each simulation instance.


\textbf {50th Percentile Delay:}  Average time until half of the network is informed about a specific block. A reasonable value for the time window the simulation refers to is (5..8sec) as it is reported in []\\

\textbf {outgoing block rate:} The average number of blocks a full node sends in a given time frame. This number is used to calculate the average outgoing bandwidth (excluding transactions)  per node and compare it with that of  our live nodes .  A reasonable value for the time window the simulation refers to is  (incoming ~ 13KBps, outgoing 65 KBps)

\textbf {incoming inv rate:} The average number of  inventory messages for blocks a full node receives in a given time frame. This number is used to calculate the average incoming bandwidth (excluding transactions) per node and compare it with that of our live nodes   A reasonable value for the time window the simulation refers to is DON’T KNOW YET

\textbf {Orphan rate:} the percentage of blocks that were mined but were not included in the blockchain.  reasonable value for the time window the simulation refers to is  1%-3%

\subsection{Evaluation Metrics }

\textbf {Orphan rate:} the percentage of blocks that were mined but were not included in the blockchain. Each time there is a fork ie two different versions of the main blockchain at least an orphan block is produced The consequences of an higher orphan rate for the currency could be summarized as follows.
1. Bitcoin mining becomes an unprofitable and thus unpopular investment.  The miners that produced the orphan blocks lose the corresponding revenue for their work. 
2. Bitcoin becomes a highly insecure currency. Two blocks of the same height can include conflicting transactions i.e double spends. In this case even a careful merchant that waits at least up to 20 minutes can be deceived. 
3.  Bitcoin becomes unsuitable for quick payments. The computational power, and consequently  the amount of generated blocks are stable. Each block is connected to the previous one so one could imagine that blocks form a tree whose longest path - ( height of the tree) is the Main chain. A higher node degree results in a shorter tree (of the given number of nodes). Equally more forks result in a shorter Main Chain. A shorter Main chain essentially means  lower block generation rate which increases the time it takes for a transaction to be included in a block.\\


\maria{\textbf{@aviv:} Can you descriope Bet over Lamda?}




\textbf {Generated blocks - In-chain Blocks:} This two metrics refer to the number of blocks a specific pool has mined and to the number of blocks she received revenue for. The former is always proportionate to the computational power of the pool. A large relative increase in the latter is interpreted as malicious behavior that was successful for the attackers, while a decrease denotes malicious behavior that resulted loss of revenue for the attacker it self.We will study the corresponding metrics of one specific pool which will also serve as attacker to have a consistent view of the impact the attack has in the network.


Graph1-Passive: Y: number of colluding ISPs, X orphan rate 3 lines Equal distribution, Decentralized Pools ,Centralized pools

Graph2-Passive-Active: Y: number of colluding ISPs, X orphan rate  -3 lines Equal distribution and 100 hijacked prefixes, Decentralized Pools 20 Hijacked Prefixes,Centralized pools, 10 hijacked prefixes Should that be one graph? or many

Graph 3 Passive-Pool :  Y:number of  ISPs that collude , X \% of unfair share gained. For example pool X has 20 \% mining power and she colludes with the ISPs she manage to put 25\% of her blocks in the Blockchain. We will see an increase because the always works on the latest block (The ISPS do not delay packets in her connection). She can follow 2 policies - two lines in the graph. Policy 1 propagate her blocks but not blocks mined by others. Policy 2 Do does selfish mining !!!!! for that we make an extra assumption  that she chooses other pools as her peers.

Graph 4 Passive-Active-Pool :  Y:number of  ISPs that collude , X \% of unfair share gained. 

Graph 2.1 2.2 2.3 2.4   Y:number of  ISPs that collude  :Lamda 



\subsection{Pure Networking Attacks}\laurent{The ``pure'' is ackward}
 
\myitem{Description:} At first we consider pure networking passive attacks, in that a number of AS (0 to 5) collude to attack bitcoin community exclusively by delaying unpreferentially all block messages that are naturally routed through their infrastructure. The aim of the attacker in this case is to destroy the currency by increasing the fork rate.


D0T0T0   23/28\% --> 23/29\%        2\%         100\%            6-11           6-11-7
D1T0T0   19/18\% --> 18/18\%        8\%         0\%             7-2430          7-12-7
D2T0T0   19/17\% --> 15/18\%        28\%        11\%            10-22024        7-12-7
D3T0T0   22/20\% --> 20/32\%        42\%        5\%             1217-23924      7-11-7
D4T0T0   25/27\% --> 23/46\%        47\%        3\%             1219-42965      6-11-6
D5T0T0   21/17\% --> 18/25\%        43\%        17\%            1223-38944      7-12-7

\textbf {Comments:}  If  network level adversaries collude then they can cause 30\% fork rate aka almost one out of three mined blocks are orphans. This percentage raises as more ISPs are added to the attacker's group. It is extremely worrying that only 6 ASes are enough to render most of the generated blocks orphans ie waste most of the computational power that is devoted to Bitcoin. Moreover, the network becomes more unfair as the attackers become more powerful. 50\% percent unfairness means that in half of the block races the node that generated the block first loses the corresponding revenue.


\textbf {Description:}	In this experiment we consider the case of a pool that colludes with ISPs. The ISPs are again  passive attackers, in that they only delay block messages. However in this instance of the simulation the network adverseries do not delay blocks that are destined to or send by the colluding pool. The pool never propagates the blocks which were mined by others. In other words she never uses its propagation advantage for serving the community. In regards to propagating the blocks she mines. she follows three different policies.\\
\textbf {Policy v1:}	The pool propagates the blocks she mines immediately.\\
\textbf {Policy v2:}	The pool performs shellfish mining in that she keeps a private chain of blocks she mined and works on them without propagating them to the network. The aim is to force the rest of the network to work on blocks that are destined to become orphans. Such an attack is successful if the pool manages to create a private longer chain which is then announced to the network, nullifying the work of the benign miners and gaining more revenue than her fair share.In our case (policy v2)  when the pool is on a block race (a block of of height equal to height of a block in the private chain  is propagated in the network), she propagates exactly one block, the one that has the same height as the one that is propagated regardless of the length of the private chain.\\
\textbf {Policy v3:}	The pool performs shellfish mining but propagates 2 blocks from the private chain when a block race occurs if possible (if the private chain contains at least 2 blocks)\\

Policy v1:\\
D0T8T0   26/25\% --> 26/25\%        0\%         0               5-11            6-11-17\\
D1T8T0   22/20\% --> 22/28\%        30\%        3\%             6-17340         7-11-15\\
D2T8T0   20/24\% --> 20/30\%        21\%        0\%             6-19037         8-12-16\\
D3T8T0   21/21\% --> 21/30\%        32\%        7\%             9-39220         7-11-14\\
D4T8T0   29/27\% --> 29/37\%        28\%        3\%             6-39329         7-12-15\\
D5T8T0   21/21\% --> 21/31\%        34\%        4\%             6-41463         7-12-14\\


Policy v3:\\
D0T8T2   21/23\% --> 18/26\%        25\%        13\%            6-12444         6-11-11\\
D1T8T2   23/25\% --> 17/25\%        28\%        28\%            6-33758         6-11-10\\
D2T8T2   22/17\% --> 21/27\%        38\%        2\%             8-30592         7-12-10\\
D3T8T2   29/26\% --> 27/40\%        39\%        5\%             7-37725         6-11-9\\
D4T8T2   24/21\% --> 24/35\%        39\%        0\%             6-35429         7-12-11\\
D5T8T2   19/20\% --> 18/33\%        43\%        9\%             9-37970         6-11-9\\

 When there is  no network adversary and no pool behave malisciously the fork rate is 1\%. When there is a pool that does selfish mining the fork rate increases as one would expect since this is a consequence for the attack. The crucial thing about our results which serves as a validation point is that the selfish pool does not manage to gain more revenue than her fair share despite its behavior when there is no network-level support .?? This is due to the fact that its computational power is beyond the limit of 33\% that is proven to be the minimum for performing a successful selfish mining attack in []:

The level unfairness also increases. I HOPE!!!!




==> reviews.tex <==
\section{Previous reviews}

Prior to being submitted to IEEE Security \& Privacy 2017, this paper was
submitted to ACM CCS 2016 (where it was heavily discussed at the TPC meeting,
see highlighted part of Review \#262B below) and at USENIX Security 2016
(preliminary version). We include the reviews verbatim below.

The paper has been \emph{thoroughly} revised since then. We highlight (in 500
words) the improvements made to the paper and how we incorporated the feedback
from the reviewers in Appendix~\ref{appendix:answers}. We also add clickable references to the reviews below pointing to our answers.

\subsection{\textbf{Reviews from ACM CCS 2016}}

%---------------------------------------------------------------------------
\myitem{Review \#262A}
%---------------------------------------------------------------------------

\medskip
\noindent{\emph{Decision:}} 2. Reject (will argue against)

\medskip
\noindent{\emph{Summary:}} This paper studies large-scale network attacks on Bitcoin. It considers AS-level adversaries and traffic interception, routing, and traffic delay attacks.

\medskip
\noindent{\emph{Paper strengths:}} \\
- measurement study of Bitcoin using real world routing data \\
- experiments with partitioning, traffic delays

\medskip
\noindent{\emph{Paper weaknesses:}} Not sure to what extent these findings are about Bitcoin rather than about
Internet in general. I think the results would not change if you would select
6000 random servers on the Internet. So it is more about centralization of
global traffic by ASes and country-wise biases in global usage of Internet \reviewref{ans:bitcoin-specific}.

Another shortcoming is in oversimplified assumptions about miners, and their
network infrastructure. Miners are not simple peers, they are multi-homed, and
major pools form fully connected graph with direct links \reviewref{ans:multi-homing}.

\medskip
\noindent{\emph{Additional comments for authors:}} I think the paper would benefit from a more carefully study of several major mining pools, their topology and connectivity to each other and to the rest of the peers. There are some recent studies of topology of the bitcoin network, this could be a starting point. I think your Section 6 is closer to how such a study might look like \reviewref{ans:multi-homing}.

\medskip
\noindent{\emph{Response to rebuttal:}} I am still not convinced that 15 major pools are connected to the rest of the world by just 30 IPs. This would be prone to easy DoS attacks, and we know that major pools are frequently under DoS attacks and learned to survive them. It should be possible to find the real miner connectivity via methods used by recent topology discovery papers (i.e. make multiple connections to many peers over extended periods of time and discover peers who are the first to relay the blocks) \reviewref{ans:multi-homing}.


%===========================================================================
\myitem{Review \#262B}
%---------------------------------------------------------------------------

%---------------------------------------------------------------------------

\medskip
\noindent{\emph{Decision:}} 5. Accept (will argue for)

\medskip
\noindent{\emph{Summary:}} The authors investigate a number of disruption attacks on the Bitcoin network, which can be conducted by controlled groups of IP addresses (ASes). An attacker exploits the routing BGP protocol, which diverts the IP traffic using announcements of IP prefixes to neighbor ASes. They show that the centralization of the Bitcoin network makes it possible for a single AS to intercept 50\% of traffic by hijacking only about 800 BGP prefixes. The authors also discuss variations of the attack differing in visibility and effectiveness and propose countermeasures.

\medskip
\noindent{\emph{Paper strengths:}} \\
- Insight into the power of BGP hijacking attacks in the application to Bitcoin.\\
- A vast number of attacks with different profiles.\\
- Mining power centralization is taken into account.\\
- Detailed simulations.

\medskip
\noindent{\emph{Paper weaknesses:}} \\
- Bitcoin nodes behind NAT are not considered \reviewref{ans:nated-node}.\\
- BGP description is missing.

\medskip
\noindent{\emph{Additional comments for authors:}} The vast majority of Bitcoin nodes do not actually have a public IP and can not accept connections. As noted in Biryukov et al. ``Deanonymisation of clients in Bitcoin P2P network'', there are 10-12x more such nodes than regular ones, considered in this paper. Nevertheless, they can forward blocks and transactions. Thus even if you isolate public-IP nodes, the latter still may communicate through the NAT-hidden nodes. This will probably makes your attacks more difficult \reviewref{ans:nated-node}.

\medskip
\noindent{\emph{Comment after discussion:}} Please elaborate on how exactly the intercepting attack on Bitcoin would work. Do you break the miners-pool connections? Pool-Pool? Pool-Peer? Peer-peer? Note that in all cases but the last one the Bitcoin protocol is not used, and the number of 6000 nodes is irrelevant \reviewref{ans:confusion}. 

It is important to relate your attack to the following paragraph:
"In the centralized distribution, we attribute most of the
hash rate to few ASes. We attribute 92\% of the mining power
to pools and assume that the remaining 8\% is equally distributed
among all other nodes. We infer the distribution of
mining power among pools from [6], which contains statistics
sourced from the blockchain itself and refer to the first
week of Nov 2015. We assign pools to ASes using the public
IPs of the Stratum servers that are used by miners to connect
to those pools." Please elaborate how you got these IPs.

\medskip
\noindent{\emph{Response to rebuttal:}} The rebuttal addressed most the issues
I raised, though not to the sufficient detail due to the lack of space. The
authors should nevertheless elaborate on the attack description in the future
edit of the paper.

\textbf{After a very long discussion}, the paper was rejected because of: 1) a bit of overselling \reviewref{ans:overselling}; 2) the actual feasibility of the attack is in question \reviewref{ans:practicality}; 3) the reviewers do not believe that the pools have so weak connectivity in reality \reviewref{ans:multi-homing}.

I personally think that the paper will be a strong accept at a less competitive conference.

\newpage
%===========================================================================
\myitem{Review \#262C}
%---------------------------------------------------------------------------

\medskip
\noindent{\emph{Decision:}} 3. Weak reject (will not argue against)

\medskip
\noindent{\emph{Summary:}} Attackers can cause partitioning and other attacks on Bitcoin via BGP prefix hijacking.

\medskip
\noindent{\emph{Paper strengths:}} \\
- The P2P network is arguably the weak underbelly of cryptocurrencies, so network attacks deserve more research attention.\\
- There are several nice measurement results about the Bitcoin network, especially its centralization.\\
- Interesting simulation-based results on the time to recover from a partition.\\
- Good discussion of possible countermeasures.

\medskip
\noindent{\emph{Paper weaknesses:}}
The authors do not adequately justify their claim that hijacking hundreds of prefixes is feasible. The closest they come is in pointing out that BGPStream reported 1616 prefix hijacks in 6 months or ~8.8 per day. But it seems that the paper's attack would require hundreds of prefixes to be hijacked at the same time, which is orders of magnitude more than the reported rate \reviewref{ans:hijacking_many_pfxes}.

Most large miners run more than one node; in fact, they have geographically distributed setups. They do this to minimize latency, but it also helps resist partitions. This fact is also not considered \reviewref{ans:multi-homing}.

While the time to recover from a partition is important to know, the time to detect a partition is also important and should be considered. Exchanges and other entities have measures in place to freeze funds and minimize damage if a partition is detected. The authors should discuss in more detail how nodes might be able to detect a partition or other attacks.

Attacking mining pools might not be sufficient to isolate mining power, since miners can quickly switch to different pools.

\medskip
\noindent{\emph{Additional comments for authors:}} The summary of my comments above is that the paper seems to overstate the practical feasibility of the attack in various ways. It doesn't uncover any fundamental weakness of the protocol, but rather points out that a powerful adversary will be able to cause mayhem on the network. The crucial question for the paper, then, is just how powerful that adversary needs to be. While the paper goes a fair way toward answering this question using measurements and simulation, there are additional factors to be taken into account as pointed out above \reviewref{ans:overselling}.

The suggestion that "nodes should deploy anomaly detection mechanisms to
recognize sudden changes and alert operators" is a very good one. It would be nice to see a couple of such techniques prototyped and evaluated.

``Hosting all Bitcoin nodes in /24 would prevent such attacks at the cost of a marginal increase (1\%) of the total number of Internet prefixes.'' 1\% sounds like a pretty big increase.

A more equivalent but more scalable countermeasure can be found in 
``We show that a single AS could increase the orphan rate by a factor of 10 with respect to that of the current Bitcoin network, while the US could increase orphan rate up to 50\% and Germany up to 29\%.'' This statement was unclear at first. Clarity that you mean a single AS could increase it from 1\% to 10\%.

The number of prefixes that need to be hijacked when taking mining power into account is variously reported as 31\% and 37\%.

\medskip
\noindent{\emph{Response to rebuttal:}} After discussing the rebuttal with the
other reviewers, I'm unconvinced that the attack is as practically feasible as
the authors claim.

This paper makes a nice contribution, but the hyperbole detracts from its
value. My score is thus unchanged \reviewref{ans:practicality}.


\subsection{\textbf{Reviews from USENIX Security 2016}}

\myitem{Review \#52A}

\medskip
\noindent{\emph{Decision:}} 3. OK paper. I hope we can find better papers to accept.

\medskip
\noindent{\emph{Expertise:}} 3. Knowledgeable

\medskip
\noindent{\emph{Summary:}} This paper studies AS-level network disruption attacks on Bitcoin.

\medskip
\noindent{\emph{Paper strengths:}} This is an interesting, messy layer of Bitcoin that hasn't been studied in detail and there are some interesting conclusions and a good list of countermeasures is proposed. This paper serves reasonably well as a taxonomy of routing attacks on Bitcoin and countermeasures.

\medskip
\noindent{\emph{Paper weaknesses:}} The analysis is not very deep. In particular, I think the paper took the tack of trying to claim very powerful attacks are possible to make it look like a surprising result is being had here, at the expense of a balanced investigation into what kinds of attacks are possible or likely \reviewref{ans:overselling}. Lots of more subtle attacks aren't really analyzed.

\medskip
\noindent{\emph{Comments for authors:}} Most of the attacks here are
conceptually known in the Bitcoin community and it is not surprising that major
ASes could wreak havoc on Bitcoin if the desired. This is a very powerful
adversary (an AS willing to risk it's reputation by performing network
manipulation) and it's not clear an entity with this ability would want to do
this \reviewref{ans:practicality}.

In particular, the claims of ``only a few ASes need collude'' are somewhat weak
because these are huge ASes, e.g. Comcast. Does Comcast really want to risk a
major damage to its billion dollar business to fiddle with Bitcoin? These
attacks make more sense in the ``Goldfinger'' attack setting where the
attacker's goal is to take down Bitcoin for no monetary gain (e.g. a national
Chinese AS). They also probably could do this without sophisticated attacks and
this isn't surprising. Furthermore, Bitcoin would likely adapt \reviewref{ans:overselling}.

I think it would have been much more compelling to focus the paper not on what
a small coalition of the most prominent ASes could achieve (who are highly
unlikely to attack) but a smaller AS (or group) which is more reasonable to
assume would go rogue. I think this is a major drawback of this paper, as it
really only focuses on what the most powerful attackers could do \reviewref{ans:overselling}.

While this paper assumes a powerful attacker, it then makes very generous
assumptions about the Bitcoin network being highly connected. I understand the
authors did not crawl the Bitcoin network to observe its actual topology, but I
have no idea why they didn't just simulate a random network with Bitcoin's
degree of connectivity, which is what Bitcoin is meant to create anyways \reviewref{ans:multi-homing}.

The assumptions about the distribution of mining power were also somewhat
simplistic. I think it would have been very intersting to assume that certain
pools are actually multi-homed at different nodes and see how that affects
things. This is clearly the next step in how mining pools will adapt to routing
attacks \reviewref{ans:multi-homing}.

This paper misses quite a few types of attacks to discuss. Most prominently, an
AS could attack while new nodes are joining the network (or finding peers) to
try to ``shape'' the network. I was disappointed to see this possibility not
mentioned in the paper.

The discussion of partition attacks was very simplistic. A true partition
attack is probably impossible as all it takes is one node which is multi-homed
and relaying data between the partitions on a covert channel. The paper ignores
such dedicated ``relay networks'' based on a very shaky assumption in the
appendix that they could also be attacked. These are much easier however to
hide and move around and avoid attacks, I think it would be quite hard to block
all of them \reviewref{ans:practicality}.

Given that a full partition would probably not be stable, the paper fails to
provide a more nuanced discussion of what can be done with a near partition. In
particular, such an attacker can still delay propagation significantly and can
frontrun transactions and block (e.g. see transactions and replace them with
competing transactions) with high success. Even without partitioning the
network, this is a powerful attack. It make selfish mining attacks and many
other approaches possible even without a complete partition. This is usually
modeled in more recent selfish mining papers by a parameter $\gamma$, measuring
the fraction of the network for which the attacker can replace a targeted
transaction/block \reviewref{ans:practicality}.

With all of these limitations, the analysis in the paper was not as compelling
as it could have been. I still think this is important work and with some
refinement this will be a very strong paper, the modeling is just a bit simple
right now.

%===========================================================================
\myitem{Review \#52B}
%---------------------------------------------------------------------------
%---------------------------------------------------------------------------

\medskip
\noindent{\emph{Decision:}} 2. Weak paper. This paper should be rejected but I will not fight strongly against it.
                
\medskip
\noindent{\emph{Reviewer expertise:}} 4. Expert

\medskip
\noindent{\emph{Summary:}} This paper describes two attacks on Bitcoin based on
network concentration, assuming real world AS topology and IP usage, but
synthetic mining power distribution.

\medskip
\noindent{\emph{Paper strengths:}} Use of real world network topologies for
evaluating attacks is an excellent approach.

\medskip
\noindent{\emph{Paper weaknesses:}} The mining power distribution is the big
question: Mining power is known to be heavily concentrated in the hands of a
few players, but at the same time the miners, since they are negatively
effected by the attacks more than any other paper \reviewref{ans:multi-homing}.

Rather esoteric in actual practice, it may be more appropriate for a narrower
interest conference.

\medskip
\noindent{\emph{Comments for authors:}} You correctly flag that mining
distribution is the key parameter to evaluate the actual practicality of these
attacks, but at the same time, you simply state that it is a ``hard problem''
and use synthetic data. 

This paper would be much better if you solved that ``hard'' problem, because that problem is not that hard. Most miners advertise in the blocks themselves that they are responsible for discovering in the coinbase (it acts as both advertising and is commonly used for voting as well). So you can use that to mostly model the actual distribution of miners \reviewref{ans:multi-homing}.

Similarly, by crawling the Bitcoin network, you can also identify the set of
nodes responsible for creating these blocks. Yes, you won't always see the
origin IP for any given block, but you can take advantage of this
centralization and, by acting as a heavy block propagator in your network, also
exclude nodes as possible sources. Using this, you should be able to do a much
better evaluation of how the Bitcoin network generates new blocks \reviewref{ans:multi-homing}.

This would also be interesting from a social/measurement standpoint, since my
hunch is that ``the miners are Chinese, the users are American'', and this
would allow you to evaluate this maxim to see if it is true.

There is also, as a consequence of centralization, another defense to your
block slowing attack: The few centralized miners could run a few additional
scattered nodes, and maintain VPN tunnels to these nodes (so an adversary can't
see the traffic and the nodes can know if the trafic is being delayed or
disrupted by including heartbeats in the VPN), with these nodes acting to
aggressively rebroadcast blocks they discover. Since this also acts to reduce
the problem of orphan blocks for the miners, this provides a benefit even in
the absence of a routing attacker \reviewref{ans:multi-homing}.

I also think this would be better suited for a more narrowly focused
conference: This work isn't applicable to other networks, or necessarily even
other crypto-currencies, as it largely depends on:

\noindent1:  The deep centralization present in Bitcoin;\\
2:  The ability to easily distinguish Bitcoin traffic;\\
3:  The economic motivation present in Bitcoin to launch such an attack \reviewref{ans:bitcoin-specific}.

==> small_summary.tex <==
%preamble 
\section{Routing attacks on Bitcoin}
\label{sec:summary}

In this section we give an overview of the various network attacks that we
consider in this paper (see Fig.~\ref{fig:taxonomy}). 

\myitem{Attacker model:} We consider that an AS-level attacker can \emph{only}
manipulate ``pure'' bitcoin connections and assume that mining pools can use
\emph{any} proprietary, secure and private protocol internally. The attacker
aims at disrupting either a given set of nodes ranging from a single node to
nodes controlling 50\% (or more) of the mining power. In the case of attacks
against mining power, the attacker should know at least some of the gateways.
We explain in Section~\ref{} how an attacker can discover these gateways using
publicly known information such as Stratum servers. The overall attack is split
into consecutive steps. In Step 1 (\textbf{[S1]}), the AS-level attacker
performs a hijack or leverage natural routing (if possible) to intercept the
relevant Bitcoin traffic (Section~\ref{ssec:summary_intercept}). After that, in
Step 2 (\textbf{[S2]}), the attacker either: \emph{(i)} isolates the set of
nodes (\textbf{[A1]}); or \emph{(ii)} delay the delivery of blocks towards them
(\textbf{[A2]}).

%the AS-level attacker exploits access this Bitcoin traffic to disrupt either a small set of nodes or the system as a whole (Section~\ref{ssec:summary_attack}).

\begin{figure}[t]
 \centering
 \includegraphics[width=\columnwidth]{figures/summary_figure}
 \caption{Illustration of how AS-level adversaries can intercept Bitcoin traffic by hijacking prefixes or leveraging natural connectivity and then attacking either specific nodes of the network as a whole. \laurent{Update caption}}
 \label{fig:overview}
\end{figure}

We now illustrate how each steps of the routing attacks work along with the
potential impact for Bitcoin. As an illustration, we consider a simple example
(Fig.~\ref{fig:overview}). Bitcoin nodes are connected to AS1, AS2, AS3, AS4,
AS5 and AS6. Each AS\emph{X} advertise one IPv4 prefix: \emph{X}.0.0.0/16. For
instance, AS1 advertises 1.0.0.0/16. Two mining pools are depicted as a green
(left) and a red (right) region. Both pools are multi-homed: they have gateways
in more than one AS. For instance, the right pool is hosted in 3 ASes, AS4,
AS5, AS6 hosting its gateways nodes, I, J, F.


%We start by describing how the attacker can get on path and discusses how does
%the attacker figures out what to hijack later.

\subsection{\textbf{[S1]} Intercepting Bitcoin traffic}
\label{ssec:summary_intercept}

Routing attacks are performed either by \emph{passive attackers} who intercept
Bitcoin traffic naturally, or by \emph{active attackers} who perform BGP
hijacks to actively get on path. Passive attackers are usually the direct
providers of the bitcoin nodes whose traffic they intercept or large,
well-established ASes that are crossed by many connections. Passive attackers
are only effective against specific connections but they can act almost
invisibly on them. For instance, AS3 can intercept the connections from node J
to nodes A and B but not from node J to node H. In contrast, the effectiveness
of active attackers grows as they increase the number of prefixes they hijack,
but their attack is highly visible. For instance AS8 could hijack 1 prefix to
intercept all traffic destined to bitcoin nodes A and B, except the traffic
between them.

\subsection{\textbf{[S2]} Attacking Bitcoin consensus}
\label{ssec:summary_attack}

Once on-path, AS-level adversaries can fiddle with Bitcoin connections by
arbitrarily dropping, delaying or even modifying the messages exchanged. We
consider two different attacks (\textbf{[A1]} and \textbf{[A2]}) against
Bitcoin by either partitioning a subset of the Bitcoin network or by delaying
the propagation of blocks. The two attacks offer different tradeoffs in terms
of effectiveness (measured in the amount of disruption they can create), the
amount of connection they require to intercept and the visibility in doing so
(which correlates with how likely is the attacker to be discovered).

\myitem{[A1] Partitioning: highly disruptive, at the node \emph{and} network-wide level; require full interception; highly visible.}
The goal of this attack is to isolate a set of nodes from the Bitcoin network
such that no information can flow between them. To do so an attacker should
intercept and cut or filter \emph{all connections} from the isolated set of
nodes to the rest of the network. The difficulty of performing this attack
depends on the target (node-level or network-wide) and especially the type of
bitcoin clients (simple client or gateways large mining pools).

Isolating small set of nodes (or a single node) is relatively easy and can be
performed by active attackers, located anywhere, or by passive attackers which
happen to be crossed by all connections naturally. For instance, AS4 can
isolate node J from the network by cutting all its connections or by filtering
incoming information from the network. The same result can be accomplished by
the active attacker AS8 hijacking J's prefix.

In contrast, isolating a large set of nodes or large mining pools is
considerably harder considering the presence of multi-homed mining pools, NATed
nodes and relays. Only an active attacker can overcome these difficulties as
passive attackers (even when considering country-wide coalition) are unlikely
to be on-path for enough connections. To isolate the one or more muti-homed
mining pools, an active attacker can hijack the prefixes pertaining to all the
gateways. We discuss in Section~\ref{} how an attacker can discover these
gateways automatically. Even when considering that mining pools can be gateways
in as many as 15 ASes, we show that isolating 50\% of mining power is within
reach of any active attacker hijacking less than 400 prefixes.

In Section~\ref{sec:bitcoin_interception}, we also investigate on how an active
attacker can encompass other challenges such as limiting the amount of diverted
traffic. We also investigated the long term influence of a 50\%-50\% partition
after the hijack has been mitigated in a testbed of 1050 nodes running the
default bitcoind (Section~\ref{fig:partition}). We show that the Bitcoin network almost heals immediately from a partition attack in the sense that consensus is quickly reached again once the partition starts to leak, i.e. whenever (even few) connections start bridging the once-disconnected components. 

%Despite this, it takes a lot of time for the isolated components to re-establish connections to each
%other nodes within them reach consensus almost immediately.

\myitem{[A2] Delaying propagation: disruptive, mainly for targeted attacks;
works with partial interception; invisible.} The goal of this attack is to
eclipse nodes by delaying the delivery of blocks to them, without disrupting
their connections or actively connecting to them. Delay attacks can be
performed by both active and passive attackers. Yet, they are more likely to be
adopted by the former as they are invisible and effective \emph{even} if the
attacker intercept parts of the victim's traffic. As an illustration, AS3 can
successfully eclipse node J even though it does not intercept all of its
connections. If J receives an \textsf{INV} message for a new block from nodes A
B and H and either A or B advertised the block before H then AS3 can delay its
delivery for 20 minutes, effectively eclipsing J. This is in practice a more
complicated procedure requiring the attacker to fiddle with both the TCP and
the Bitcoin protocol to avoid detection and disconnection. We verified the
practicality of the attack by implementing a complete prototype which we use to
attack our own bitcoin nodes and found that an attacker can eclipse a victim
for 63\% of its uptime even when intercepting half of its connections (see
Section~\ref{sec:delay}).

We further evaluated the effectiveness of delay attacks when performed
network-wide using a realistic simulator. We found that the effectiveness of
delay attacks decreases with the degree of multi-homing adopted by the mining
pools. Indeed, we show that even the most powerful passive attacker, i.e. a
country-wide coalition of all the US-based networks together, cannot cause
considerable damage to the network if each of the main pools is hosted in at
least 5 ASes.

\subsection{\textbf{[S2]} Impact on Bitcoin}
\label{ssec:summary_impact}

The impact of the attack varies with respect to the number and type of the impacted bitcoin nodes. At the node-level such attacks can keep the victim eclipsed, essentially performing a successful denial of service attack or rendering it vulnerable to 0-confirmation double spends. If the node is a gateway of a pool such attacks can be used to engineer block races.
Network-wide attacks such as a isolating a considerable amount of mining power or sufficiently delaying the propagation of blocks to increase the fork rate renders the network extremely vulnerable to all sorts of exploits. As a sufficient number of blocks are discarded, the  miner's revenue is deducted and the network is more vulnerable to double spends. Especially in the case of the partition, all transactions included in the chain of the side with the least mining power are likely to be reversed. In the case of delaying, significant slowdown of block transmission can be used to launch selfish mining attacks by adversaries with mining power.


==> sp copy/abstract.tex <==
\begin{abstract}
As the most successful cryptocurrency to date, Bitcoin constitutes a target of choice for attackers. While many attack vectors have already been uncovered, one important vector has been left out though: attacking the currency via the
Internet routing infrastructure itself. Indeed, by manipulating routing
advertisements (BGP hijacks) or by naturally intercepting traffic,
Autonomous Systems (ASes) can intercept and manipulate a large fraction of Bitcoin
traffic. %As of now, the potential impact of these network attackers on the cryptocurrency is unknown.
 %Actually, traffic for at
%least 100 Bitcoin nodes end up diverted by BGP hijacks \emph{each month}.
%By leveraging natural Internet routing or
%manipulating advertisements (BGP hijacks), ASes can indeed intercept and
%manipulate Bitcoin traffic.

This paper presents the first taxonomy of routing attacks and their impact on
Bitcoin, considering both small-scale attacks, targeting individual nodes, and
large-scale attacks, targeting the network as a whole. While challenging, we
show that two key properties make routing attacks practical: \emph{(i)} the
efficiency of routing manipulation; and \emph{(ii)} the significant
centralization of Bitcoin in terms of mining and routing. Specifically, we
find that any network attacker can hijack few (<100) BGP prefixes to isolate
{\raise.17ex\hbox{$\scriptstyle\sim$}}50\% of the mining power---even when
considering that mining pools are heavily multi-homed. We also show that
on-path network attackers can considerably slow down block propagation by interfering with few key Bitcoin messages.

We demonstrate the feasibility of each attack against the deployed Bitcoin
software. We also quantify their effectiveness on the current Bitcoin topology
using data collected from a Bitcoin supernode combined with BGP routing data.

The potential damage to Bitcoin is worrying. By isolating parts of the network
or delaying block propagation, attackers can cause a significant amount of
mining power to be wasted, leading to revenue losses and enabling a wide range
of exploits such as double spending. To prevent such effects in practice, we provide both short and long-term countermeasures, some of which can be
deployed immediately.

\end{abstract}





\remove{We demonstrate the feasibility of each attack against the deployed Bitcoin software and quantify both the node-level and network-wide impact using data collected from a bitcoin supernode combined with BGP routing data. The potential damage to Bitcoin is worrying. }

==> sp copy/acknowledgement.tex <==
\vfill
\section*{Acknowledgments}

We would like to thank Christian Decker for sharing Bitcoin data with us as
well as for his valuable comments in the beginning of the project. We would
also like to thank David Gugelmann for his support in one of our experiments.
Finally, we are grateful to Tobias B\"uhler, Edgar Costa Molero, and Thomas Holterbach from ETH
Z\"urich as well as Eleftherios Kokoris Kogias from EPFL for their helpful
feedback on early drafts of this paper. Aviv Zohar is supported by the Israel
Science Foundation (grant 616/13) and by a grant from the Hebrew University
Cybersecurity Center.

==> sp copy/background.tex <==
\section{Background}
\label{sec:background}

\subsection{BGP}

\myitem{Protocol} BGP~\cite{rfc1771} is the de-facto routing protocol that
regulates how IP packets are forwarded in the Internet. Routes associated with
different IP prefixes are exchanged between neighboring networks or Autonomous
Systems (AS). For any given IP prefix, one AS (the origin) is responsible for
the original route advertisement, which is then propagated AS-by-AS until all
ASes learn about it. Routers then set their next hop and pick one of the
available routes offered by their neighbors (this is done independently for
each destination).

In BGP, the validity of route announcements is not checked. In effect, this
means that any AS can inject forged information on how to reach one or
more IP prefixes, leading other ASes to send traffic to the wrong location.
These rogue advertisements, known as BGP ``hijacks'', are a very effective
way for an attacker to intercept traffic en route to a legitimate
destination.

\myitem{BGP hijack} An attacker, who wishes to attract all the traffic for a legitimate prefix $p$ (say,
100.0.0.0/16) by hijacking could either: \emph{(i)} announce $p$; or \emph{(ii)} announce a more-specific (longer) prefix of $p$. In the first
case, the attacker's route will be in direct competition with the legitimate
route. As BGP routers prefer shorter paths, the attacker will, on average,
attract 50\% of the traffic~\cite{goldberg_how_secure_are_interdomain_routing_protocols}. In the
second case, the attacker will attract all the traffic (originated anywhere on the Internet) addressed to the destination as Internet routers forward traffic according to the longest-match entry. 
%We speak of a \emph{global} hijack. 
Note that traffic internal to an AS cannot be diverted via hijacking as it does not get routed by BGP but by internal routing protocols (e.g., OSPF).

For instance, in order to attract all traffic destined to
$p$, the attacker could advertise 100.0.0.0/17 \emph{and} 100.0.128.0/17.
Routers in the entire Internet would then start forwarding any traffic destined to the original /16 prefix according to the two covering /17s originated
by the adversary. Advertising more-specific prefixes has its limits though as BGP operators will often
filter prefixes longer than /24~\cite{Karlin:2006:PGB:1317535.1318378}. Yet, we show
that the vast majority of Bitcoin nodes is hosted in shorter prefixes
(Section~\ref{sec:topology}) and is thus susceptible to hijacking.

By default, hijacking a prefix creates a black hole at the attacker's location. However, the attacker can turn a hijack into an
\emph{interception} attack simply by making sure she leaves at least one path untouched to the
destination~\cite{defcon_mitm, goldberg_how_secure_are_interdomain_routing_protocols}.

\subsection{Bitcoin}

%We briefly provide background on the Bitcoin protocol and refer the reader to~\cite{nakamoto2008bitcoin, zohar2015bitcoin} for a broader
%introduction.

\myitem{Transactions} Transaction validation requires nodes to be aware of the
ownership of funds and the balance of each Bitcoin address. All this
information can be learned from the Bitcoin blockchain: an authenticated data
structure that effectively forms a ledger of all accepted transactions.
Bitcoin main innovation lies in its ability to synchronize the blockchain in
an asynchronous way, with attackers possibly attempting to disrupt the
process. Synchronization is crucial: conflicting transactions attempting to
transfer the exact same bitcoins to different destinations may otherwise be
approved by miners that are unaware of each other.

%\footnote{This is in fact a manifestation of the Byzantine consensus problem.}

\myitem{Block creation} Bitcoin's blockchain is comprised of blocks, batches of transactions, that are
appended to the ledger serially. Each block contains a cryptographic hash of
its predecessor, which identifies its place in the chain, and a proof-of-work.
The proof-of-work serves to make block creation difficult and reduces the
conflicts in the system. Conflicts, which take the form of blocks that extend
the same parent, represent alternative sets of accepted transactions. Nodes
converge to a single agreed version by selecting the chain containing the
highest amount of computational work as the valid version (usually the longest
chain). The proof-of-work also serves to limit the ability of
attackers to subvert the system: they cannot easily create many blocks, which
would potentially allow them to create a longer alternative chain that will
be adopted by nodes and thus reverse the transfer of funds (double spend).

The difficulty of block creation is set so that one block is created in the
network every 10 minutes on average which is designed to allow
sufficient time for blocks to propagate through the network. However, if delays
are high compared to the block creation rate, many forks occur in the chain as
blocks are created in parallel. In this case, the rate of discarded blocks (known as the
\emph{orphan rate} or the \emph{fork rate}) increases and the security of the
protocol deteriorates~\cite{decker2013information,garay2015bitcoin,sompolinsky2015secure}. Newly
created blocks are propagated through the network using a gossip protocol. In
addition to the propagation of blocks, nodes also propagate transactions
between them that await inclusion in the chain by whichever node creates
the next block.

\myitem{Network formation} Bitcoin acts as a
peer-to-peer network with each node maintaining a list of IP addresses of
potential peers. The list is bootstrapped via a DNS server, and additional
addresses are exchanged between peers. By default, each node randomly initiates 8 \emph{unencrypted} TCP connections to peers in
different /16 prefixes. Nodes additionally accept connections initiated by
others (by default on port 8333). The total number of connections nodes
can make is 125 by default.

Nodes continually listen to block announcements which are sent via \textsf{INV} messages containing the hash of the
announced block. If a node determines that it does not hold a newly announced block, it sends a \textsf{GETDATA} message to a \emph{single}
neighbor. The peer then responds by sending the requested information in a
\textsf{BLOCK} message. Blocks that are requested and do not arrive within 20
minutes trigger the disconnection of the peer and are requested from another.
Transaction propagation occurs with a similar sequence of \textsf{INV},
\textsf{GETDATA}, and \textsf{TX} messages in which nodes announce, request,
and share transactions that have not yet been included in the blockchain.

\myitem{Mining pools}
Mining pools represent groups of miners that divide block creation rewards between them in order to lower the high
economic risk associated with infrequent (but high) payments. They usually operate using the Stratum protocol \cite{bitcoin:book}. The
pool server is connected to a bitcoind node that acts as a gateway to the Bitcoin network. The node collects
recent information regarding newly transmitted transactions and newly built blocks which are then used to construct a
new block template. The template header is then sent via the Stratum server to the miners who attempt to complete
it to a valid block. This is done by trying different values of the nonce field in the header. %\footnote{In fact
%miners have additional degrees of freedom to change the block structure to increase the search space that they
%may operate over}. 
If the block is completed, the result is sent back to the Stratum server,
which then uses the gateway node to publish the newly formed block to the network.%\footnote{Miners also submit
%partial solutions to the pool which are used to measure their mining rate for the purpose of reward division.}

\myitem{Multi-homing} Mining pools often use multiple gateways hosted by diffrent Internet
Service Providers. We refer to the number of different ISPs a
pool has as its multi-homing degree. %Practically this number is equal to the
%number of different ASes its gateways are hosted in.



==> sp copy/conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}

This paper presented the first analysis of the vulnerabilities of the Bitcoin
system from a networking viewpoint. Based on real-world data, we showed that
Bitcoin is heavily centralized. Leveraging this fact, we then demonstrated and
quantified the disruptive impact that AS-level adversaries can have on the
currency. We showed that attackers can partition the Bitcoin network
by hijacking less than 100 prefixes. We also showed how AS-level adversaries
can significantly delay the propagation of blocks while remaining undetected.
Although these attacks are worrying, we also explained how to counter them with both short-term and long-term measures, some of which are easily deployable today.

==> sp copy/countermeasures.tex <==
\section{Countermeasures}
\label{sec:countermeasures}

% Short-term countermeasures
	% Client-side measures:
		% Prevention:
			% AS- and Prefix-aware path selection:
				% Select nodes in /24
				% Select nodes according to AS-PATH or # hops away they are
			% Check that your AS is multihomed and that it monitors its prefixes
		% Monitoring:
			% RTTs to detect BGP hijack~\cite{}
			% the connection distribution, rough changes
			% the rates of block creates/forks
	% Network-side measures
% Long-term countermeasures:

In this section, we present a set of countermeasures against routing attacks.
We start by presenting measures that do not require any protocol change and can
be partially deployed in such a way that early adopters can benefit from higher
protection (Section~\ref{ssec:short_term}). We then describe longer-term
suggestions for both detecting and preventing routing attacks
(Section~\ref{ssec:long_term}).

\subsection{Short-term measures}
\label{ssec:short_term}

%We now describe a set of countermeasures which do not require changes in the
%bitcoin protocol. This mean that early adopter can immediately benefit of
%higher protection. We start by describing local prevention techniques that
%Bitcoin nodes could apply to decrease their attack surface. We then describe
%monitoring techniques to detect when a routing attack is taking place.

%\subsubsection{Prevention}


\myitem{Increase the diversity of node connections} The more connected an AS
is, the harder it is to attack it. We therefore encourage Bitcoin node owners to ensure they are multi-homed. 
Observe that even
single-homed Bitcoin nodes could benefit from extra connectivity by using one or
more VPN services through encrypted tunnels so that Bitcoin
traffic to and from the node go through multiple and distinct ASes.
Attackers that wish to deny connectivity through the tunnel would need to
either know both associated IP addresses or, alternatively, disrupt
all encrypted traffic to and from nodes---making the attack highly noticeable.

\myitem{Select Bitcoin peers while taking routing into account} Bitcoin
nodes randomly establish 8 outgoing connections. While randomness is important
to avoid biased decisions, Bitcoin nodes should establish a
few \emph{extra} connections taking routing into consideration. For this,
nodes could either issue a \verb+traceroute+ to each of their peers and
analyze how often the same AS appears in the path or, alternatively, tap into the BGP feed of their network and select their peers based on the AS-PATH. In both cases, if the same AS appears in all paths, extra random connections should be established.
%While this has the advantage of being less forgeable, it is also considerably harder to acquire and process. 
%\subsubsection{Detection}

\myitem{Monitor round-trip time (RTT)} The RTT towards hijacked destinations
increases during the attack. By monitoring the RTT towards its peers, a node could detect sudden changes and establish extra random connections as a protection mechanism.

\myitem{Monitor additional statistics} Nodes should deploy anomaly detection mechanisms to recognize sudden changes in: the distribution of connections, the time elapsed between a request and the corresponding answer, the simultaneous disconnections of peers, and other lower-level connection anomalies. Again, anomalies should spur the establishment of extra random connections.

\myitem{Embrace churn} Nodes should allow the natural churn of the network to
refresh their connections. A node with disabled incoming connections or even one that is behind a NAT or a firewall will never receive a random incoming
connection from the rest of the network. If the node is hijacked for a few
minutes and isolated from a part of the network, it will only reconnect to the other part upon reboot or when one of its outgoing connections fails.

\newpage
\noindent\textbf{Use gateways in different ASes} While inferring the topology we noticed that many pools were using gateways in the same AS. Hosting these gateways in different ASes would make them even more robust to routing attacks.

\myitem{Prefer peers hosted in the same AS and in /24 prefixes} As the traffic
of nodes hosted in /24 prefixes can only partially be diverted (Section~\ref{sec:background}). Hosting all
nodes in such prefixes would prevent partition attacks at the cost of
({\raise.17ex\hbox{$\scriptstyle\sim$}}1\%) increase of the total number of
Internet prefixes. Alternatively, nodes could connect to a peer hosted in a /24
prefix which belongs to their provider. By doing so they maintain a stealth
(intra-AS) connection with a node that is at least partially protected against
hijack.
%Indeed, on average, all Bitcoin nodes would fit in only 5{,}650 prefixes.


\subsection{Longer-term measures}
\label{ssec:long_term}

%We now describe a set of changes to the Bitcoin protocol or to the Internet
%infrastructure that would render routing attacks much harder.
\myitem{Encrypt Bitcoin Communication and/or adopt MAC} While encrypting Bitcoin connections
would not prevent adversaries from dropping packets, it would
prevent them from eavesdropping connections and modifying key messages. Alternatively, using a Message Authentication Code (MAC) to validate that the content of each message has not been changed would make delay attacks much more difficult. 

% . \aviv{Need to check the following. I think other ports can be used as they are simply propagated in addr messages. As long as they are not changed too often, they will be effective.}

\myitem{Use distinct control and data channels} A key problem of Bitcoin is
that its traffic is easily identifiable by filtering on the default port
(8333). Assuming encrypted connections, the two ends could negotiate a set of random TCP ports upon connecting to each other using
the well-known port and use them to establish the actual TCP connection, on
which they will exchange Bitcoin data. This would force the AS-level adversary
to look at \emph{all the traffic}, which would be too costly. 

A simpler (but poorer) solution would be for Bitcoin clients to use randomized TCP port (encoded in clear with the \textsf{ADDR} message) as it
will force the AS-level adversary to maintain state to keep track of these ports.
Although a node can already run on a non-default port,
such a node will receive fewer incoming connections (if any) as the default client strongly prefers peers that run on the default port.
%\maria{We should mention here that UDP would make the job of the attacker easier since 1. no state is required 2. attacker can be in any of the paths to drop packets} 
%\aviv{pushed text below. Check that I'm not repeating something from elsewhere.}

\myitem{Use UDP heartbeats} A TCP connection between two Bitcoin nodes may take
different forward and backward paths due to asymmetric routing, making AS-level
adversaries more powerful (as they only need to see one direction, see Section~\ref{sec:delay}). In addition to TCP connections, Bitcoin clients could
periodically send UDP messages with corroborating data (\emph{e.g.}, with
several recent block headers). These UDP messages can be used as a heartbeat
that will allow nodes to discover that their connection was partially
intercepted. As UDP messages do not rely on return traffic, this would
enable node to realize that they are out-of-sync and establish new connections.
%These UDP messages can be sent rarely enough so that they do not significantly
%affect bandwidth demands. %Moreover, Bitcoin clients themselves could bounce
%these UDP messages so as to increase the connection diversity.

\myitem{Request a block on multiple connections} Bitcoin clients could ask
multiple peers for pieces of the block. This measure would prevent misbehaving
nodes from deliberately delaying the delivery of a block, simply because in
such a case the client will only miss one fraction of the block, which it can
request from one of its other peers.




%Such a measure does not come at odds
%with the scalability requirements of the protocol, since the client will
%receive the same amount of data. Note that the 20 minutes threshold a client
%waits by default for a node to deliver a block was added was a scalability
%measure.




==> sp copy/delay.tex <==
%%Fig.~\ref{fig:res_fork_rate_passive}
\section{Delaying Block Propagation}
\label{sec:delay}


While partitioning attacks (Section~\ref{sec:partition}) are particularly effective and can be performed by
 any AS, they require full control over the victim's traffic and are also highly visible. In this section, we
explore \emph{delay attacks}, which can cause relatively severe delays in block propagation, even when an attacker intercepts only one of the victim's connections, and wishes the attack to remain relatively undetectable. 

In this attack, the adversary delays the delivery of a block by modifying the content of specific messages.
This is possible due to the lack of encryption and of secure integrity checks of Bitcoin messages. In addition to these, the attacker leverages the fact that nodes send block requests to the first peer that advertised each block and wait 20 minutes for its delivery, before requesting it from another peer. 

The first known attack leveraging this 20 minutes timeout~\cite{Gervais:2015:TDB:2810103.2813655} mandates the adversary to be connected
to the victim and to be the first to advertise a new block. After a successful
block delay, the connection is lost. In contrast, network-based delay attacks are
more effective for at least three reasons: \emph{(i)} an attacker can act on
existing connections, namely she does not need to connect to the victim which
is very often not possible (e.g, nodes behind a NAT); \emph{(ii)} an attacker
does not have to be informed about recently mined blocks by the
victim's peers to eclipse it; and \emph{(iii)} the connection that was used for
the attack is not necessarily lost, prolonging the attack.

Particularly, the effectiveness of the delay attack depends on the direction and
fraction of the victim's traffic the attacker intercepts. 
Intuitively, as Bitcoin clients request blocks from one peer at a time, the probability that the attacker will intercept such a connection increases proportionally with the fraction of the connections she intercepts. In addition, Bitcoin connections are bi-directional TCP connections, meaning the attacker may intercept one 
direction (e.g., if the victim is multi-homed), both, or none at all. Depending on the direction she intercepts, the attacker fiddles with different 
messages. In the following, we explain the mechanism that is used to perform the attack if the attacker intercepts traffic \emph{from} the victim  (Section~\ref{ssec:outgoing_attack}) or \emph{to} the victim node (Section~\ref{ssec:incoming_attack}). While in both cases the attacker does delay block propagation for 20 minutes, the former attack is more effective. \remove{The node-level attack can be easily extended to a network level attack, in which case the adversary delays all blocks propagated through the connections she intercepts.}

\begin{figure}[t]
 \centering
 \begin{subfigure}[t]{0.45\columnwidth}
 \includegraphics[width=\columnwidth]{figures/delay_attack_left}
 \caption{$\curvearrowleft$ Attacker $\curvearrowleft$ victim}
 \label{fig:delay_attack_left}
 \end{subfigure}
 \hfill
 \vrule
 \hfill
 \begin{subfigure}[t]{0.45\columnwidth}
 \includegraphics[width=\columnwidth]{figures/delay_attack_right}
 \caption{$\curvearrowright$ Attacker $\curvearrowright$ victim}
 \label{fig:delay_attack_right}
 \end{subfigure}
 \caption{An attacker can perform different delay attacks depending on the direction of traffic she intercepts. When on the path from the victim, it can modify the \textsf{GETDATA} message (a), while it can modify the \textsf{BLOCK} message when intercepting the opposite path (b).}
 \label{fig:delay_attack_figure}
\end{figure}

 \remove{

We now explain the mechanism of attacking a single node. This mechanism can be easily extended to a network level attack, in which case the adversary, delays all blocks propagated through the connections she intercepts.
Particularly, the effectiveness of the attack depends on the direction and
fraction of the victim's traffic the attacker intercepts. Bitcoin nodes
establish connections with many peers. To effectively delay the delivery of a block to a victim node the
attacker should intercept the connection between the victim and the first of its peers which advertised this particular block to it. 
This is due to the fact that a bitcoin client only requests a block from the first peer which advertised it.
Intuitively, the largest the fraction of connections the attakcer intercepts the higher her chance to delay the delivery of a blcok to it
All these connection are bi-directional TCP connections, meaning the attacker can intercept one direction (e.g., if the victim is multi-homed), both or none at all. We start by describing the most effective attack, which can be performed by an
adversary that intercepts at least a fraction of the traffic that originates
\emph{from} the victim (\S\ref{ssec:outgoing_attack}).
We then describe another attack that can be performed by a MITM observing at least a 
fraction of the traffic destined \emph{to} the victim (\S\ref{ssec:incoming_attack}). Both
attacks allow  an adversary to delay blocks by 20 minutes, but the
former is less visible.
}

\subsection{The attacker intercepts outgoing traffic}
\label{ssec:outgoing_attack}

Once a node receives a notification that a new
block is available via an \textsf{INV} message, it issues a download request
to its sender using a \textsf{GETDATA} message. As an illustration in Fig.~\ref{fig:delay_attack_left} the victim requests Block 42
from the first of its peers that advertised the block. 
Since the attacker intercepts the traffic from the 
victim to this peer, she can modify this \textsf{GETDATA} message to request an older block, instead of the original one.
In Fig.~\ref{fig:delay_attack_left} for example, the attacker replaces the hash corresponding to block 42 with that of block 30. The advantage of doing so, over just dropping the packet, is that the length of the message is left unchanged. Notice that if the packet was dropped the attacker would need to intercept both directions of the connection and update the TCP sequence numbers of all following packets to ensure that the connection is not dropped. If the block is not delivered, the victim node will disconnect after 20 minutes.
 To avoid a disconnection, the attacker can use another
\textsf{GETDATA}, sent within the 20 minute window, to perform the reverse
operation. Specifically, she modifies the hash back to the original one, requested by the victim. 
Since the \textsf{GETDATA} message for blocks and transactions have the same structure, the attacker is more likely
to use the latter as these are much more common. In Fig.~\ref{fig:delay_attack_left} for example, she changes the hash of
the transaction (Tx \#123) to the hash of block 42. Since the block is delivered within the timeout neither of the nodes disconnects or has any indication of the attack (e.g., an error in the log files).

\remove{Also, the large majority of Bitcoin nodes uses the
default TCP port (8333) to communicate, rendering the task of identifying
Bitcoin traffic trivial.

As an illustration in Fig.~\ref{fig:delay_attack_left} the victim node asks for the Block 42 from the first of its peers that advertised it, and sets a timer for 20 minutes. Once this period has elapsed,
it will request the block from another peer. The attacker changes the hash requested with the \textsf{GETDATA} message effectively causing the
peer to deliver another block which the victim ignores. Before the 20 minutes timeout the attacher trigers the deliver of the Block 42 by restoring the corresponding hash to a random \textsf{GETDATA} of a transactions as these are more common. Since the block is delivered within the time-out neither of the nodes disconnects or have an indication of the attack (e.g. an error in the log files).
}




\remove{This practice was adopted by Bitcoin core as a scalability measure. To avoid a disconnection, which would deprive 
her from the MITM position, the attacker can use another
\textsf{GETDATA}, sent within the 20 minutes window, to perform the reverse
operation. Specifically, she modifies the hash back to the original one, requested from the victim. In practice, another
\textsf{GETDATA} sent by the victim is almost always guaranteed to be found
within 20 minutes of the original, as \textsf{GETDATA} messages for transactions (Tx\#123 in Fig.~\ref{fig:delay_attack_left})), which are much more common in the Bitcoin network, can be also used.
}

\remove{
Three reasons make this attack extremely effective.
\emph{Firstly}, it works even if the adversary does not intercept all
of the victim's connections. \remove{ Even 50\% of all connections is enough to eclipse the victim for 63\% of its uptime. }    
\emph{Secondly}, the victim has
no clear indication that it is under attack, since there is no error in its log
files. 
% \aviv{this is not correct:} Actually, even the frequency of received blocks is legitimate. 
\emph{Thirdly}, by making sure that the victim
receives the block within 20 minutes, the attacker avoids disconnection and maintains her influence over time.
This matters especially when she intercepts only a relatively small fraction of
the victim's connections. Without doing so, the attacker looses one connection
per delayed block, as the victim will likely pick connections the attacker does not intercept.
%every 10 minutes, assuming that she delays all blocks and one block is
%mined every ten minutes. \remove{  \laurent{why 10 and not 20?}}In this case, her power will rapidly degrade.
Observe that the attacker could increase its effectiveness even more using
hijacks or Eclipsing methods~\cite{heilman2015eclipse} so as to bias the selection of peers and intercept more of the victim's connections.
}

\subsection{The attacker intercepts incoming traffic}
\label{ssec:incoming_attack}

We now describe the mechanism an attacker would use if she intercepts traffic
towards the victim, \emph{i.e.} she can see messages received by the victim, but not the messages that it sends.
This attack is less effective compared to the attack working in the opposite direction, 
as it will 
eventually result in the connection being dropped 20 minutes after the first delayed block (similarly to~\cite{Gervais:2015:TDB:2810103.2813655}).
\remove{Yet, this attack still allows a MITM intercepting only this direction to effectively delay the delivery of a block to a node for 20 minutes.}
In this case, the attack focuses on the
\textsf{BLOCK} messages rather than on the \textsf{GETDATA}. A naive attack
would be for the attacker to simply drop any \textsf{BLOCK} message she sees. As Bitcoin
relies on TCP though, doing so would quickly kill the TCP connection. A
better, yet still simple approach is for the attacker to corrupt the contents of a
\textsf{BLOCK} message while preserving the length of the packet (see Fig.~\ref{fig:delay_attack_right}). This simple operation causes the \textsf{BLOCK} to be
discarded when it reaches the victim, because of a checksum mismatch. Surprisingly
though, we discovered (and verified) that the victim will \emph{not} request the block again, be
it from the same or any other peer. After the 20 minute timeout elapses,
the victim simply disconnects because its requested block did not arrive on time.

An alternative for the adversary is to replace the hash of the most recent
\textsf{Block} with a hash of an older one in all the \textsf{INV} messages the
victim receives. This attack however would fail if the attacker intercepts only
a fraction of the connections, as the victim will be informed via other connections. As such, this practice is only useful when the attacker
hijacks and thus intercepts all the traffic directed to the victim.


\remove{
In this Section we focus on the process of attacking a single node. The same procedure can be applied to attack a larger set of nodes or the network as a whole.


describe how a network adversary
can leverage some key features of the protocol to attack a single node,



 The key difference of this attack in comparison to a partition attack is that it does not require the attacker to control all connections of his victims. As such even adversaries with partial view of the victim's traffic can eclipse it for a considerable percentage of its up-time.


}



\remove{In section \ref{sec:delay_results}, we prove the practicality and effectiveness of our attack in practice against a single node and  by performing it in the live bitcoin network against our own nodes. We also show its 
Three factors make this attack possible: \emph{(i)} Bitcoin nodes request the block from one of their peers only and wait 20 minutes for it to be delivered; \emph{(ii)} Bitcoin traffic is unecrypeted 
\emph{(iii)} Bitcoin traffic incorporate no authenticity test.
}

\remove{ 
Delay attacks require fiddling with the Bitcoin messages. Thus, only specific AS-level adversaries can launch them. Particularly,\emph{(i)} any AS that is naturally traversed by some of the bitcoin traffic of a node can perform a delay attack against it; while \emph{(ii)} only very powerful network attackers that intercept a considerable percentage of the overal bitcoin traffic can attack the bitcoin network as a whole. 
}
\remove{ 
Such attacks are completely invisible, yet very effective in eclipsing specific nodes, as well as in disrupting the bitcoin consensus mechanism in general. This effectiveness is a consequence of the 20 minutes delay an attacker can cause to the delivery of a block, which also creates a cascading effect when many nodes are attacked in parallel. 20 minutes make up a large time interval for Bitcoin, given that the median
propagation delay of blocks is around 7 seconds and the block creation rate is
10 minutes ~\cite{neudecker2015simulation}. During this time, the delayed nodes mine on an obsolete branch, are uninformed of the latest authorized transactions and do not serve the P2P
network by propagating blocks.



We investigate the practicallity and effectiveness of delay attacks at the node and network-level.

With regards to node-level delay attacks, 
in Section \ref{ssec:network_single_node_attack}, we describe how a network adversary
can leverage some key features of the protocol to attack a single node, she
intercepts traffic from or towards. We evaluate the attack on actual Bitcoin
nodes that we control and are connected to the live network. We show that a
node can stay uninformed during 85\% of the time it is under attack without
detecting it. 

With regards to network-wide delay attacks, in Section \ref{ssec:network_delay_attack}, we
investigate the effectiveness of AS-level adversaries in the current Bitcoin topology. For this, we built a realistic Bitcoin simulator. Using it, we show that delay attacks against the current bitcoin network can be disruptive if performed by powerful attacker such as US and China. We further investigate the rubustness of the bitcoin network as a function of the degree of multi-homing pools adopt. Particularly we show that an adequately higher degree of multi-homing than that pools adopt today would render network-wide attacks almost imposible, even for the US. However, we also acknoledge that delay attacks would have been much more disruptive if mining pools had been single-homed.
}




==> sp copy/delay_results.tex <==
\section{Delaying Block Propagation: Evaluation}
\label{sec:delay_results}

In this section, we evaluate the impact and practicality of delay attacks
through a set of experiments both at the node-level and at the network-wide
level. We start by demonstrating that delay attacks against a single node work
in practice by implementing a working prototype of an interception software that we then use to delay our own Bitcoin nodes
(Section~\ref{ssec:network_single_node_attack}). We then evaluate the impact of
network-wide delay attacks by implementing a scalable event-driven Bitcoin simulator. In constrast to partitioning attacks, and to targeted delay attacks, we show that Bitcoin is well-protected against network-wide delay attacks, even
when considering large coalitions of ASes as attackers (Section~\ref{ssec:network_delay_attack}).

\subsection{How severely can an attacker delay a single node?}
\label{ssec:network_single_node_attack}

%To answer this question, we implemented a working prototype of an interception
%software that an attacker could run on intercepted traffic. We then used our
%prototype to measure the effectiveness of an attacker in function on how many
%connections she intercept.

\myitem{Methodology} 
We implemented a prototype of our interception software on top of Scapy~\cite{scapy}, a
Python-based packet manipulation library. Our prototype follows the methodology of Section~\ref{sec:delay} and is efficient both
in terms of state maintained and processing time. Our
implementation indeed maintains only 32B of memory (hash size) for each peer of the
victim node. Regarding processing time, our implementation leverages pre-recompiled
regular expressions to efficiently identify critical packets (such as those
with \textsf{BLOCK} messages) which are then
processed in parallel by dedicated threads. Observe that the primitives required for the interception software are also supported by recent programmable data-planes~\cite{bosshart2014p4} opening up the possibility of performing the attack entirely on network devices.

%% These two lines are not enough to claim the P4 implementation as a contribution. Given that we have already too much, I'd not include its
%To reduce the latency further we investigated an alternative implementation on programmable hardware, particularly on P4 switches. 
%As the results do not differ between the two implementations we measured the effectiveness of the attack using the former.

%For forwarding packets from kernel to the user
% space we used  nfqueue \cite{nfq} and simple IPTABLE rules. 

We used our prototype to attack one of our own Bitcoin nodes
(v/Satoshi:0.12.0/, running on Ubuntu 14.04). The prototype ran on a machine acting as a gateway to the
victim node. Using this setup, we measured the effectiveness of an attacker in
delaying the delivery of  blocks, by varying the percentage of connections she intercepted. To that end, we measured the fraction of time during which the victim was uninformed of the most recently mined block.
We considered our victim node to be uninformed when its
view of the main chain is shorter than that of a reference node. The reference
node was another Bitcoin client running the same software and the same number of peers as the victim, but without any attacker.

%To co attackers that intercepts different fraction of connections, we
%programmed our prototype to only try to delay the delivery of a block with
%probability equal to that fraction. In essence, we assumed that every peer has
%equal chance of advertise the block first to the victim. \maria{Maybe remove
%that}The reason why we chose not to forward only this fraction of connection
%through the prototype, is that we noticed that a client is mostly informed by a
%small fraction of its peer. Had we chosen such a solution, we would need many
%more experiments to reach a statistically correct result.

\newpage
\noindent\textbf{Delay attackers intercepting 50\% of a node's connection can waste 63\% of its mining power} 
Table~\ref{tab:node_results} illustrates the percentage of the victim's uptime, during which it was uniformed of the last mined block, considering that the attacker intercepts 100\%, 80\%, and 50\% of its connections.
Each value is the average over an attack period of {\raise.17ex\hbox{$\scriptstyle\sim$}}\emph{200 hours}. To further evaluate the practicality of the attack, the table also depicts the fraction of Bitcoin nodes for which there is an AS, \emph{in addition to their direct provider}, that intercepts 100\%, 80\%, and 50\% of its connections.

Our results reflect the major strength of the attack, which is its
effectiveness even when the adversary intercepts only a fraction of the
victim's connections. Particularly, we see that an attacker can waste 63\% of a
node's mining power by intercepting half of its connections. Observe that, even
when the attacker is intercepting all of the victim's connections, the victim eventually
gets each block after a delay of 20 minutes.

Regarding the amount of vulnerable nodes to this attack in the Bitcoin
topology, we found that, for 67.9\% of the nodes, there is at least one AS
\emph{other than their provider} that intercepts more than 50\% of their
connections. For 21.7\% of the nodes there is in fact an AS (other than their provider) that intercepts all their connections to other nodes. In short, 21.7\% of the nodes can be isolated by an AS that is not even
their provider.

\begin{table}[t]

\centering
\small
\def\arraystretch{1.1}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lclclcl@{}}

\toprule
%Attack && Active(How much) && Passive(Who can) &&  \% ForkRate && Implications\\
\centering

\% intercepted connections  && 50\% && 80\%  && 100\% \\
\midrule
\% time victim node is uniformed	&& 63.21\% 	&& 81.38\%  && 85.45\% 	\\
\% total vulnerable Bitcoin nodes && 67.9\%  &&  38.9\%  &&  21.7\%  \\
\bottomrule
\end{tabular}
\caption{67.9\% of Bitcoin nodes are vulnerable to an interception of 50\% of their connections by an AS \emph{other than their direct provider}.
Such interception can cause the node to lag behind a reference node 63.21\% of the time.}
\label{tab:node_results}
\end{table}



\subsection{Can powerful attackers delay the entire Bitcoin network?}
\label{ssec:network_delay_attack}

Having shown that delay attacks against a single node are practical, we now quantify the network-wide effects of delaying block propagation. 

Unlike partitioning attacks, we show that network-wide delay attacks (that do not utilize active hijacking) are unlikely to happen in practice. Indeed, only extremely powerful attackers such
as a coalition grouping all ASes based in the US could significantly delay the
Bitcoin network as a whole, increasing the orphan rate to more than 30\% from
the normal 1\%. We also investigate how this effect changes as a function of the degree of multi-homing that pools adopt.

\myitem{Methodology} Unlike partition attacks, the impact of delay attacks on the network is difficult to ascertain. One would need to actually slow down the network
to fully evaluate the cascading effect of delaying blocks. We therefore built a
realistic event-driven simulator following the principles
in~\cite{neudecker2015simulation} and used it to evaluate such effects.

\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

% Laurent: I've removed the table as we need space, but happy to put it back if deemed needed!
\remove{
\begin{table*}
	\centering
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		\specialcell{Monitored\\connection} & The attack & \specialcell{Preserve\\TCP} & \specialcell{Preserve\\BTC} & Outcome \\
		\hline
		any & drop tcp packets & no & no & connection lost after tcp timeout\\
		\hline
		from node & \specialcell{change block hash in getdata\\ message} & yes & no & bitcoind drops connection after 20 min\\
		\hline
		from node & \specialcell{change block hash in getdata\\ message, inject again within 20 min} & yes & yes & \specialcell{block delayed 20 min \\ (connetion kept)}\\
		\hline
		to node & make block header invalid & yes & no & bitcoind drops\left(  connection after 20 min\\
		\hline
	\end{tabular}
	\caption{The effect of different attacks}
\end{table*}
}

Our simulator models the entire Bitcoin network and the impact of a delay
attack considering the worst-case scenario for the attacker. Specifically, it
assumes that the communication between gateways of the same pool cannot be
intercepted. Also, pools act as relay networks in that they propagate all blocks that
they receive via all their gateways. Moreover, the simulator assumes that the
delay attacker is only effective if she intercepts the traffic \emph{from} a node that receives a block (essentially if she is able to perform the
attack depicted in Fig.~\ref{fig:delay_attack_left}). 
We provide further details on our simulator and how we evaluated it in Appendix~\ref{ssec:simulation}.

We ran our simulator on realistic topologies as well as on synthetic ones with
higher or lower degrees of multi-homing. The realistic topology was inferred as
described in Section~\ref{sec:topology}. The synthetic ones were created by
adding more gateways to the pools in the realistic topology until all pools
reached the predefined degree of multi-homing.

%\laurent{We need to explain where does the realistic topology come from?}

\begin{table}[t]
\centering
\small
\def\arraystretch{1.1}
\setlength{\tabcolsep}{6.5pt}
\begin{tabular}{cccccc}

\toprule
%Attack && Active(How much) && Passive(Who can) &&  \% ForkRate && Implications\\
\multirow{2}{*}{\textit{Coalition}} & \multirow{2}{*}{\textit{Realistic topology}} & \multicolumn{4}{c}{\textit{Multihoming degree of pools}} \\
\cmidrule{3-6}
& (Section~\ref{sec:topology})	& \textit{1}		& \textit{3}		& \textit{5} & \textit{7} \\
\midrule
US & 23.78 & 38.46 & 18.18 & 6.29 & 4.20 \\
DE & 4.20 & 18.88 & 2.10 & 1.40 & 1.40 \\
CN & 4.90 & 34.27 & 1.40 & 0.70 & 0.70 \\
\bottomrule
\end{tabular}
\caption{Orphan rate (\%) achieved by different network-wide level delay attacks performed by coalitions of \emph{all} the ASes in a country, and considering either the topology inferred in Section~\ref{sec:topology} or synthetic topologies with various degrees of pool multi-homing. The normal orphan rate is \raise.17ex\hbox{$\scriptstyle\sim$}1\%.}
\label{tab:sim_results}
\vspace{-.3cm}
\end{table}

\myitem{Due to pools multi-homing, Bitcoin (as a whole) is not vulnerable to delay attackers, even powerful ones} Our results are summarized in Table~\ref{tab:sim_results}. We see that multi-homed pools considerably increase the robustness of the Bitcoin network against delay attacks. In essence, multi-homed pools act as protected relays for the whole network. Indeed, multi-homed pools have better chances of learning about blocks via at least one gateway and can also more efficiently propagate them to the rest of the network via the same gateways.
%Also, once it learns about a block, the multi-homed pool will propagate it to
%the network using all its gateways. 

If we consider the current level of multi-homing, only powerful
attackers such as a coalition containing \emph{all} US-based ASes could effectively disrupt the network by increasing the fork rate to 23\%
(as comparison, the baseline fork rate is 1\%). In contrast, other powerful
attackers such as all China-based or all Germany-based ASes can only increase
the fork rate to 5\%. As such coalitions are unlikely to form
in practice, we conclude that \emph{network-wide} delay attacks do not constitute a threat for Bitcoin.

\myitem{Even a small degree of multi-homing is enough to protect Bitcoin from
powerful attackers.} If all mining pools were single-homed, large coalitions
could substantially harm the currency. The US for instance, could increase the
fork rate to 38\% while China and Germany could increase it to 34\% and 18\%
respectively. Yet, the fork rate drops dramatically as the average multi-homing
degree increases. This is a good news for mining pools as it shows that even a
small increase in their connectivity helps tremendously in protecting them against delay attacks.

%According to our results, increasing the average degree of multi-homing pools adopt, would significantly increase robustness of the network against delay attacks. Particularly, moderate degree of multi-homing (5 or more) if adopted by all pools, would protect the network even from the most powerful attackers.

==> sp copy/interception.tex <==
\section{Measurement Analysis - Insides}
\label{sec:topology}

In this section, we explain the datasets and the techniques used to infer the
Internet and Bitcoin topologies including a thorough study of mining pools
connectivity.

We inferred our datasets in four steps. First, we obtained the AS-level
topology and AS-to-AS forwarding paths using BGP control-plane information.
Second, we collected the bitcoin IPs of the public nodes using a supernode.
Third, we assigned mining power to pools. Fourth, we mapped the connectivity of
each pool using its Stratum servers along with delay information collected by
our supernode which enables us to study the impact of routing attacks in
function of the multihoming degree of pools.

We now describe each step as well as the datasets used. Our full dataset spans
between October 2015 and March 2016. As the results of our analysis
do not change much through time, we focus on the results computed over a 10-days period between November 5 and November 2015 unless noted otherwise.

\myitem{Step 1: BGP AS-level topology and AS-to-AS forwarding paths} We
collected \emph{2.5 million} BGP routes (covering all Internet prefixes) along
with \emph{4 billion} BGP updates advertised on 182 BGP sessions maintained by
3 RIPE BGP collectors~\cite{ripe:ris} (rrc00, rrc01 and rrc03). We collected
these routes and updates daily, for 4 months, between Oct 2015 and Jan 2016. We
also collected inferred AS-level topologies computed by
CAIDA~\cite{caida_as_level}. An AS-level topology is an undirected graph, in
which a node corresponds to an AS and a link represents an inter-domain
connection between two neighboring ASes. Links are labeled with the business
relationship linking the two ASes (customer, peer or provider). Using this
data, we computed the forwarding path taken by each AS following the routing
tree algorithm described
in~\cite{goldberg_how_secure_are_interdomain_routing_protocols}, which takes
into account the business relationships between ASes.

%Using this data, we identified which AS is hosting each Bitcoin node by mapping
%its IP address with the AS advertising the most-specific covering prefix. To
%protect our mapping from BGP hijacks, we only consider prefixes that have been
%advertised consecutively for at least one day. We then computed the sequence of
%ASes traversed when any two Bitcoin nodes communicate. 

\myitem{Step 2: Bitcoin nodes IP addresses} Each day, for 10 days, we collected
around 6{,}000 IP addresses of Bitcoin nodes using a Bitcoin supernode which
continuously crawled the Bitcoin network to discover new nodes. Our supernode
connected to approximately 2{,}000 bitcoin nodes per day (with a mean of 2174
and a median of 1875). It saw a total of 7{,}477 distinct IPs during the 10
days and was relayed a total of 1{,}440 blocks. By combining this dataset with the BGP one, we then created  node-to-AS mapping
each Bitcoin IP address to the origin AS advertising the most-specific prefix
covering it, giving us a .

%The list of IP addresses is available online~\cite{bitcoinstats_census}.

\myitem{Step 3: Mining pools distribution} We collected the
list of mining pools along with the blocks they mined using publicly-available
statistics computed on the blockchain~\cite{blockchain}. We then attributed a
share of the total mining power to each pool proportionately to the blocks
mined by the pool during the 10 days. As highlighted by previous
studies~\cite{pools,miller2015discovering}, mining power is highly skewed, with
{\raise.17ex\hbox{$\scriptstyle\sim$}}70\% of the mining power held by four
mining pools: F2Pool (21\%), AntPool (19\%), Bitfurry (15\%) and BTCC
(13\%).

\myitem{Step 4: Mining pools connectivity} For each mining pool, we
inferred the AS it uses to interconnect to the Bitcoin network. We assign pools
to ASes, taking into account multi-homing, in two consecutive steps: \emph{(i)}
considering the location of their (publicly known) Stratum server; and
\emph{(ii)} by using block propagation information crawled by our supernode.

As described in Section~\ref{sec:background}, Stratum servers are publicly
known servers used by miners to connect to the pools.
Coinscope~\cite{miller2015discovering} noted that Stratum servers tend to be
co-located in the same AS as the pools gateway to the Bitcoin network. We
therefore assign pools to ASes using the public IPs of the Stratum servers.
Overall, we found more than thirty IPs pertaining to the fifteen largest pools
by searching their websites and/or by connecting directly to them.

Relying only stratum servers to infer the gateways result in only few pools
being multi-homed. As in practice pools tend to be
multi-homed~\cite{miller2015discovering}, we augmented our pool-to-AS mapping
by considering the timing of the \textsf{INV} messages received by our
super-node. In particular, we considered that pool gateways are most likely to
be the first to learn about the blocks each pool mines. As such, we infer the
position of extra gateway nodes used by a pool by tracking down the number of
times a node is amongst the first ones to propagate a block mined by that pool.
To avoid outliers, we only consider a node as possible gateway for a pool only
if it has relayed blocks of that pool more than once during the 10-days time
frame. Using this technique, we mapped each pool to all the nodes located in (a
maximum of) 1,5,10,15 ASes by selecting the most frequent nodes in descendent
order.

\laurent{Clarify all these levels: IPs, nodes, ASes, it is not very clear at which one we operate right now.}





\begin{table}[t]
\centering
\small
\def\arraystretch{1.1}
\begin{tabular}{@{}lccccc@{}}
\toprule
%Attack && Active(How much) && Passive(Who can) &&  \% ForkRate && Implications\\
\textbf{Degree of multi-homing} && {\emph{1}} & \emph{5} & {\emph{10}} & \emph{15} \\
\color{gray}{\# ASes used to access the Bitcoin network} && & & & \\
\midrule
\textbf{F2Pool} && 1 & 10 &  16 & 22  \\
\textbf{AntPool} && 1  & 8 &  17 & 23 \\
\textbf{Bitfurry} && 1  & 5 &  13 & 19  \\
\textbf{BTCC}  && 1 & 6 &  11 & 17  \\
\bottomrule
\end{tabular}
\caption{Number of gateways for each of the four biggest pools as a function of the degree of multi-homing they adopt.}
\label{tab:ips}
\end{table}






\begin{figure}[t]
 \centering
 \includegraphics[width=.65\columnwidth]{figures/nb_hijacks_required_pools}
 \caption{The number of prefixes to hijack needed to isolate a mining pool increases as they get better connected. Yet, hijacking only 246 prefixes is enough to isolate F2Pool, the largest pool with 21\% of the mining power. Overall, hijacking less than 400 prefixes is needed to isolate 50\% of the mining power assuming pools are multi-homed in 15 ASes. This is \emph{well} within what is currently seen in the Internet (see Fig.~\ref{fig:hijack_number}).}
 \label{fig:interception_pools}
\end{figure}

%%
%%
%%%% SECTION BEGINNING
%%
%%

We start the section with describing some key-characteristics of the bitcoin network that enable passive and active attackers to intercept a large amount of bitcoin traffic ~\ref{ssec:bitcoin_topology}. As passive adversaries have no control of which connections they will intercept, we elaborate only on how active adversaries can pick a suitable set of prefixes to hijack to increase their effectiveness in ~\ref{ssec:active_interception_attacks}.



\subsection{Measurement analysis}
\label{ssec:bitcoin_topology}



 In the  following we summarize the characteristics that render the network extremely vulnerable to AS-level adversaries. results are based on routing and Bitcoin measurements described described in Section~\ref{sec:datasets}



\myitem{The Bitcoin network is \emph{extremely} centralized} Very few ASes host the
majority of the nodes in the network. Fig.~\ref{fig:cdf_bitcoin_per_ases} depicts the
cumulative fraction of Bitcoin nodes as a function of the number of hosting
ASes. We see that only 13 (\emph{resp.} 50) ASes host 30\% (\emph{resp.} 50\%) of the entire
Bitcoin network. %Table~\ref{tab:ases_number_ranking} lists the top 10 ASes in terms of
%hosted number of nodes. 
These ASes pertain to broadband providers such as Comcast (US), Verizon (US) or Chinanet (CN) as well as to cloud providers such as Hetzner (DE), OVH (FR) and Amazon (US). We observe the same kind of concentration, at the distribution of Bitcoin nodes per IP prefix: only 63 prefixes
(0.012\% of the Internet) host 20\% of the network.

\begin{figure}[t]
 \centering
 \begin{subfigure}[t]{0.47\columnwidth}
\includegraphics[width=.9\columnwidth]{figures/bitcoin_per_ases_cummulative}
	 \caption{Only
13 ASes host 30\% of the entire network, while 50 ASes host 50\% of the
network.}
	 \label{fig:cdf_bitcoin_per_ases}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.47\columnwidth} 	\includegraphics[width=.9\columnwidth]{figures/crossed_connections_per_as_cummulative}
	 \caption{Few ASes intercept large percentages of Bitcoin traffic: 3 of them intercept 60\% of all possible Bitcoin connections.}
	 \label{fig:cdf_connection_per_ases}
 \end{subfigure}
 \caption{Bitcoin is heavily centralized from a routing viewpoint.}
 \label{fig:centralization}
\end{figure}
%(Hurricane, Level3 and Telianet)

\myitem{Few ASes see a substantial part of Bitcoin traffic}
Fig.~\ref{fig:ases_connections} depicts the cumulative percentage of
connections that can be intercepted by an increasing number of ASes
(\emph{e.g.}, by colluding with each other). We see that only \emph{three}
ASes, namely Hurricane Electric, Level3, and Telianet, can together intercept
\emph{more than 80\% of all possible Bitcoin connections}, with Hurricane alone
being on path for 32\% of all connections. In general, large transit
providers (\emph{i.e.}, Tier-1s) are traversed by a large fraction of all Bitcoin connections.

%Table~\ref{tab:ases_ranking_connections} lists the top 7 ASes in terms of the
%percentage of total connections they can intercept. We see that large transit
%providers (\emph{i.e.}, Tier-1s) are traversed by a large fraction of
%all Bitcoin connections.

\myitem{$>$90\% of Bitcoin nodes are vulnerable to hijacks} 93\% of all
prefixes hosting Bitcoin nodes are shorter than /24, making them vulnerable to
a global IP hijack using more-specific announcements. Indeed, prefixes strictly
longer than /24 are typically filtered by default by many ISPs. Note that the
remaining 7\% of nodes that are in /24 prefixes are \emph{not} necessarily
safe. These can still be hijacked by another AS performing a shortest-path
attack, i.e., the attacker, who will advertise a /24 just like the victim will
attract traffic from all ASes that are closer to it than they are to the victim
(in terms of number of hops).
%This will, on average, allow him to hijack traffic to the
%victim from around half of the internet.
 %(but really depends on the exact topology).

\myitem{Bitcoin routing properties are stable} While numerous nodes join and
leave the Bitcoin network all the time, the routing properties highlighted in
this section are stable. For validation, we ran our analysis daily over a 4
month period, during which the same IPs were present on average for 15.2
consecutive days (excluding IPs that were seen only once). Moreover, our
observations regarding the network's centrality are also extremely stable: 50
ASes hosted each day 49.5\% of Bitcoin clients (standard deviation: 1.2\%)
while 24.7\% of Bitcoin nodes are found daily in just 100 prefixes (standard
deviation: 1.77\%).

\subsection{Actively Interception attacks using centralization}
\label{ssec:active_interception_attacks}
%who?
In this section we show how an active or hybrid adversary can overcome the challenges of multi-homing, NATed nodes, and relays as well as reduce the cost of the attack in diverted bandwidth and number hijacked of prefixes. 
%how
We particularly focus on a 50\% partition, intuitively any smaller partition is easier to be formed.








Active attackers are able to completely isolate
any set containing regular nodes or/and multi-homed pools, effectively creating a 
partition of nodes or mining power respectively even as large as 50\%. 
For isolating any set of regular nodes an AS adversary would need to 
intercept all their traffic. By hijacking all the prefixes of these nodes the attacker 
intercept all traffic destined to them. As such the attacker can simply prevent them 
from connecting to any node outside the set.
For isolating a pool an attacker needs to make sure  all  
gateways of a pool are hijacked. For that an AS adversary would need to know all gateways belonging to the pools he wants to include in the isolated set. 




\myitem{NATed or hidden nodes cannot bridge the partition.}
NATed nodes can only connect to public IPs. By hijacking the prefixes corresponding to a 
partition, the attacker gains control over every connection crossing it, including the 
ones from NATed nodes. By killing any bitcoin connection crossing the partition, the 
attacker effectively disconnects any bridge created by a NATed node. 

\myitem{New nodes that join the network cannot bridge the partition.}
New nodes that are in the hijacked prefixes would 
have all their connection to the other side of the partition dropped by the attacker.
Similarly nodes that are not in the hijacked partition would never be allowed to connect to
the hijacked side.

\myitem{Bitcoin relays ~\cite{relays} cannot guarantee the security of the protocol.}
They indeed improve the performance of Bitcoin. They might even be able to secure bitcoin 
against known attacks but they are still far from guaranteeing routing security. Indeed, 
the IPs of the relays are publicly available; ISPs are sometimes chosen based on pricing (
acknowledged on the website), and BGPSec is not used. All these facts make relays also 
vulnerable to both hijacking and passive attacks.

\myitem{Multi-homed pools do not prevent a partition}
Indeed multi-homing is a practice which make the network much more robust to routing 
adversaries. Even so, an active attacker can hijack all gateways of a pool effectively 
placing the whole pool in one side of the partition, given that the attacker knows the 
complete set of gateways of that pool.
In Section~\ref{sec:discussion} we further investigate how an attacker can use hijacking to discover unknown or hidden gateways.
 

\myitem{nodes in the same AS should be in one side}
Nodes in the same AS should be either all included in isolated set or all excluded from it. 
 This is because an active attacker cannot intercept the communication between nodes in the same AS. For instance in Figure~\ref{fig:overview} assume that nodes A and B have IPs 1.0.1.2 and 1.0.2.2, these belong to different /24 prefixes. If the attacker hijacks only 1.0.1.0/24 he would intercept all traffic destined to A except from the traffic from B to A. This essentially means that if the two nodes are placed in different parts of a partition they would act as a bridge if they connect to each other. Thus, in the following we assume that an attacker either hijacks all prefixes with bitcoin nodes of an AS or none. 



%

After ensuring a complete cut between the two parts The attacker's goal is to lower its footprint,
\emph{i.e.} the amount of prefixes hijacked. In the following we explain the methodology we used to estimate the smallest amount of prefixes needed to create partitions of diffrent sizes.
We always consider
the
extreme case, in which the AS-level adversary: \emph{i)} does not see \emph{any} traffic
naturally; and \emph{ii)} does not host any Bitcoin nodes.
Especially for the partition of mining power we further investigate the influence of multi-homing degree per pool in the cost of such a partition.

 
\myitem {Estimating the cost of isolating mining power.}
For each mapping of IPs to a pool we calculate the cost of isolating it in number of prefixes 
that need to be hijacked. The exact results for the four biggest pools under five 
assumptions regarding the degree of multi-homing are 
presented in Table~\ref{tab:hijacks50}  Due to the concentration of bitcoin from the 
routing perspective we found 
significant overlap among the required hijacked prefixes to isolate distinct pools. As such 
the cost of a largest partition is considerably limited in comparison to the sum of prefixes 
required per pool. We present the results for partitions containing from 49\% to 50\% of mining power. Intuitively there are smaller partitions that require  require less prefixes. We calculated these numbers using exhaustive search over all the subsets of pools partitions of 49\% to 51\% and picked the one with the least required prefixes. We found that 
only 381 prefixes needed to be hijacked even in the extreme case that the four biggest 
pools accounting for almost 70\% of mining power are hosted in 15 ASes each. When considering lower degree of multi-homing such as 5 ASes per pool  the number is reduced to half.

\myitem {Estimating the cost of isolating regular 
nodes.} For each AS with bitcoin nodes we assign a score that equals to the ratio of the number of nodes nodes it
contains over the number of prefixes with Bitcoin nodes it advertises. The
attacker then hijacks the ASes with the higher scores first. We found that \emph{870 prefixes} need to be hijacked to isolate 50\% of the public bitcoin nodes while 119 hijacked [refix would isolate 20\% of the public bitcoin nodes.% until reaching 50\% of all mining power.



\myitem{Dealing with hijacked bandwidth}
While deciding the right prefixes to hijack an attacker should also take bandwidth demands associated with the hijacked prefixes into consideration. In light of that the attacker might prefer to increase the hijacked prefixes to decrease the traffic that would be diverted to his infrastructure even if such a practice requires hijacking more prefixes. 
Going back to our example in figure ~\ref{fig:overview} if AS8 can indeed hijack one prefix namely 1.0.0.1/16 to intercept all traffic destine to nodes A and B. In this case the attacker would have to deal with all the traffic destined to a /16 prefix. However if A and B belong to a common more specific prefix then an attacker would for sure prefer to hijack this one as the diverted load would be less. The attacker can reduce the load even further by advertising only /24 prefixes even if that means he needs to advertise more prefixes. 

 \laurent{Rephrase the above in lights of the hijack study}.




%Indeed, almost of all of the mining power
%is distributed in only 20 pools, 7 of which together reach 88\%. From the
%network perspective, mining pools are \emph{even more centralized} with 15 ASes
%(in the \emph{distributed} case) or 13 (in the \emph{centralized} case) hosting
%90\% of mining power.



\myitem{Hybrid attackers} 
%
In practice, nothing prevents AS-level adversaries to combine active and passive
attacks to reduce their footprint even
further. To give an idea of such approach we present what the cost of creating the same partitioning would be if performed by the AS that was harder to hijack  (require more prefixes). For isolating 50\% of the nodes , X
prefixes are enough for a hybrid attacker. For isolating 50\% of mining power a hybrid attacker would need 13, 123,253 and 337 prefixes under the assumption that mining pools are hosted at most at 1,5,10 and 15 ASes respectively.  







\begin{table}[t]
	\centering
	\small
	\def\arraystretch{1.1}
	\begin{tabular}{@{}lclcccc@{}}
		\toprule
		\cmidrule(lr){5-6}
		\textbf{Country} && \textbf{Connections} (\%) && \emph{Partition regular nodes} \\			
		\midrule
		US && 89.8 && 37.0 \\
		DE && 32.8 && 8.8  \\
		GB && 31.4 && 5.4  \\
		SE && 26.7 && 2.0  \\
		CN && 12.2 && 5.4  \\
%		HK && 11.3 && 0.7 && 0.0 \\
		\bottomrule
	\end{tabular}
	\caption{Cumulated power ASes in the same country have over Bitcoin measured in \% of connections they intercept and the most disruptive partition of regular nodes they can achieve. \laurent{Update results} %Values are computed assuming a complete graph ie each node is connected to every other  
	}
	\label{tab:country_partition}
\end{table}











==> sp copy/intro.tex <==
\section{Introduction}
\label{sec:introduction}

With more than 16 million bitcoins valued at {\raise.17ex\hbox{$\scriptstyle\sim$}}17 billion USD and up to
300{,}000 daily transactions (March 2017), Bitcoin is the most successful
cryptocurrency to date. Remarkably, Bitcoin has achieved this as an open and fully
decentralized system. Instead of relying on a central entity, Bitcoin nodes build a large overlay network between them and use consensus to
agree on a set of transactions recorded within Bitcoin's core data structure: the
blockchain. Anyone is free to participate in the network which boasts
more than 6{,}000 nodes~\cite{bitnodes21} and can usually connect to
any other node. 

Given the amount of money at stake, Bitcoin is an obvious target
for attackers. Indeed, numerous attacks have been described targeting different aspects of
the system including: double spending~\cite{rosenfeld2014analysis}, eclipsing~\cite{heilman2015eclipse}, transaction malleability~\cite{decker2014bitcoin}, or attacks targeting mining~\cite{eyal2014majority,DBLP:journals/corr/SapirshteinSZ15,DBLP:journals/iacr/NayakKMS15} and mining pools~\cite{eyal2015miner}. %aimed at decreasing the revenue of competitors. 

One important attack vector has been overlooked though: attacking
Bitcoin via the Internet infrastructure using \emph{routing attacks}. As
Bitcoin connections are routed over the Internet---in clear text and without
integrity checks---any third-party on the forwarding path can eavesdrop, drop, modify, inject, or delay
Bitcoin messages such as blocks or transactions. Detecting such attackers is
challenging as it requires inferring the exact forwarding paths taken by the Bitcoin traffic using measurements (e.g., traceroute) or routing data (BGP
announcements), both of which can be forged~\cite{defcon_mitm}. Even ignoring
detectability, mitigating network attacks is also hard as it is essentially a
human-driven process consisting of filtering, routing around or disconnecting
the attacker. As an illustration, it took Youtube close to 3 hours to locate
and resolve rogue BGP announcements targeting its infrastructure in
2008~\cite{dyn_pakistani_bgp}. More recent examples of routing attacks such as
\cite{hijack_november_15} (resp. \cite{hijack_june_15}) took 9 (resp. 2) hours
to resolve in November (resp. June) 2015.

%This is hard
%except maybe for the direct providers of single-homed bitcoin nodes but even
%them do not have an incentive to attack the nodes they host as it would harm
%their reputation, and revenues.

One of the reasons why routing attacks have been overlooked in Bitcoin is that they
are often considered too challenging to be practical. Indeed, perturbing a
vast peer-to-peer network which uses random flooding is hard as an attacker
would have to intercept many connections to have any impact. 
Yet, two key characteristics of the Internet's infrastructure make routing
attacks against Bitcoin possible: \emph{(i)} the
efficiency of routing manipulation (BGP hijacks); and \emph{(ii)} the centralization 
of Bitcoin from the routing perspective.
First, individuals, located anywhere on the Internet, can manipulate
routing to intercept all the connections to not only
one, but many Bitcoin nodes. As we show in this paper, these routing manipulations are
prevalent today and do divert Bitcoin traffic. Second, few ASes host
most of the nodes and mining power, while others intercept a considerable fraction of the connections.

\remove{ 
 Actually, even if Bitcoin
traffic was encrypted~\cite{bitcoin_bip_151}, a network-level adversary could
still drop packets to bias or disrupt connectivity. 
}

\remove{

This argument could explain
why routing attacks have been overlooked. However, given the centralization of
the Bitcoin network together with the ability of individuals to attract the
traffic of any node via BGP manipulation (BGP hijack), routing attacks have the
potential to be very disruptive.

attacks practical: \emph{(i)} routing manipulation (BGP hijacks); and
\emph{(ii)} traffic concentration in the Internet core. \maria{that does not sound btc specific} \emph{First},
individuals, located anywhere in the Internet, can manipulate routing to
systematically intercept all the Bitcoin connections to not only one but many
Bitcoin nodes. As we show in this paper through measurements, these routing
manipulations are already prevalent today and do end up diverting Bitcoin
traffic. \emph{Second}, large Autonomous Systems (ASes) such as Internet
Service Providers (ISPs) or Internet Exchange Points (IXPs) are
\emph{naturally} crossed by many connections, potentially including a lot of
Bitcoin traffic.
}
%
\remove{
As an illustration, Fig.~\ref{fig:hijack_number} illustrates the number of BGP
hijacks we accounted by processing more than \emph{4 billions} BGP updates over
6 months\footnote{We consider an update for a prefix $p$ as a hijack if the origin AS differs from the origin AS seen during the previous month. To avoid false positives, we do not consider a prefixes which have seen multiple origin ASes during the previous month.
We account for one hijack per prefix per origin: if AS $X$
hijacks the prefix $p$ twice over a day, it only accounts for one hijack.}.
We see that there are \emph{hundreds of thousands} of hijack events \emph{each
month}. While most of these hijacks involve a single IP prefix, large hijacks
involving between 300 and 30,000 prefixes are seen every month (right axis).
Fig~\ref{fig:hijack_size} depicts the number of Bitcoin nodes impacted by these
hijacks and for which traffic was diverted. Each month, at least 100 Bitcoin
nodes are victim of hijacks. In November 2015, 447 distinct
({\raise.17ex\hbox{$\scriptstyle\sim$}}7.8\% of the entire Bitcoin network)
ended up hijacked at least once. %While already worrying, 

While frequent, BGP hijacks are hard to diagnose and slow to resolve. As BGP
securities extensions (BGPSec~\cite{bgpsec}, RPKI~\cite{rfc6480}) are seldom
deployed~\cite{lychev_bgpsec_deployment}, operators rely on simple monitoring
systems that dynamically analyze and report rogue BGP announcements
(e.g.,~\cite{yan2009bgpmon,chi2008cyclops}). When detected, solving an hijack
takes hours as it is a human-driven process consisting in filtering or
disconnecting the attacker. As an illustration, it took Youtube close to 3
hours to locate and resolve a hijack of its prefixes in
2008~\cite{dyn_pakistani_bgp}. More recent examples include a
16{,}123~\cite{hijack_november_15} (resp. 179{,}000~\cite{hijack_june_15})
prefixes hijack which took 9 (resp. 2) hours to be solved in November (resp.
June) 2015.
}

\myitem{This work} In this paper, we present the first taxonomy of routing
attacks on Bitcoin, a comprehensive study of their impact, and a list of deployable countermeasures. We consider two
general attacks that AS-level attackers can perform.
First, we evaluate the ability of attackers to isolate a set of nodes from the Bitcoin network, effectively partitioning it. Second, we evaluate the impact of delaying block
propagation by manipulating a small number of key Bitcoin messages. For both
exploits, we consider \emph{node-level} attacks along with more challenging,
but also more disruptive, \emph{network-wide} attacks.

\noindent\textbf{Partitioning attacks} The goal of a partition attack is to \emph{completely} disconnect a set of nodes from the network. This requires the attacker to divert and cut all the connections between the set of nodes and the rest of the network. 

We describe a complete attack procedure in which an attacker can
\emph{verifiably} isolate a selected set of nodes using BGP hijacks. Our
procedure is practical and only requires basic knowledge of the Bitcoin
topology, namely the IP addresses of the nodes the attacker wants to isolate.
Due to the complexity of the Bitcoin network (e.g. multi-homed pools, and
secret peering agreements between pools), the initial isolated set might contain
nodes that leak information from and to the rest of the network. We explain how
the attacker can identify and remove these leakage points until the partition
is complete.

\myitem{Delay attacks} The goal of a delay attack is to slow down the
propagation of blocks towards or from a given set of nodes. Unlike partition
attacks, which require a perfect cut, delay attacks
are effective even when a subset of the connections are intercepted. As
such, attackers can perform delay attacks on connections they are naturally intercepting, making them even harder to detect.

We again describe a complete attack procedure an attacker can run on
intercepted Bitcoin traffic so that the delivery of blocks
is delayed by up to 20 minutes. The procedure consists of modifying
 few key Bitcoin messages while making sure that the connections are not
disrupted. %The procedure works even if the attacker intercepts one
%direction of a connection hence it is compatible with asymmetric routing.

% Challenges for the attacker
% High-degree of multi-homing renders network-wide routing attacks (esp.
% delay attacks) harder, but not impossible.
\remove{
\myitem{Challenges} Large mining pools play a
critical role in the Bitcoin network. We therefore investigate the influence of
their connectivity (i.e., how much they are multihomed) on the effectiveness of
routing attacks. We show that isolation attacks do little dammage if the
partition is imperfect (e.g., due to non-intercepted gateways connections).
However, we describe ways in which strategic AS-level adversaries can actually
discover hidden gateways preventing the partition to be formed and hijack them.
Regarding delay attacks, we show that network-wide attacks do indeed become too
difficult for attackers (if powerful ones like country-wide coalitions) if
pools are multi-homed.
}
%investigate the trade-off between detectability and effectiveness

\myitem{Practicality} We showcase the practicality of each attack and evaluate
their network-wide impact using a comprehensive set of measurements,
simulations and experiments.

Regarding partitioning attacks, we show that hijacks are effective in diverting
Bitcoin traffic by performing a hijack in the wild against our own nodes. We
find that it takes less than 90 seconds to re-route all traffic flows through
the attacker once a hijack is initiated. We also show that \emph{any AS} in the
Internet hijacking \emph{less than 100} prefixes can isolate up to 47\% of the mining power, and this,
even when considering that mining pools are multi-homed. Hijacks involving
that many prefixes are frequent and already divert Bitcoin traffic.
%\laurent{need something here about the lifetime of a partition}

Regarding delay attacks, we show that an attacker intercepting 50\% of a
node connections can leave it uninformed of the most recent Bitcoin blocks
{\raise.17ex\hbox{$\scriptstyle\sim$}}60\% of the time. %For miners this implies that their hashing power during
%this period is wasted. 
We also show that intercepting a considerable percentage of Bitcoin
traffic is practical due to the centralization of Bitcoin at the routing level: one AS, namely Hurricane Electric, can \emph{naturally} 
intercept more than 30\% of \emph{all} Bitcoin connections.

\remove{
We also show that intercepting large amounts of Bitcoin
traffic is practical due to the important centralization of Bitcoin at the
the routing and mining level: 13 ASes host over 30\%
of the Bitcoin network. %and that some ASes such as Hurricane Electric can
%\emph{naturally} intercept more than 30\% of \emph{all} Bitcoin connections.
Yet, we also show that network-wide delay attacks, aiming at slowing down the
entire Bitcoin network, are not practical even for powerful
attackers.
}
%The fact that mining power is centralized in the hands of few
%pools~\cite{gervais2014bitcoin} renders routing attacks even more practical.

%We actually performed a partition attacks Even when accounting the heavy multi-homing some mining pools have, we show
%that \emph{any AS} in the Internet hijacking \emph{less than 400} prefixes can
%intercept Bitcoin connections pertaining to 50\% of the mining power. We show
%that BGP hijacks involving 400 prefixes are relatively small considering that
%some hijacks can involve 10,000s and even 100,000s prefixes.


% The potential impact on Bitcoin is worrying and ranges from loss of
% revenues to double spending and DoS attacks
\myitem{Impact on Bitcoin} The damages caused to Bitcoin in case of a
successful routing attack can be substantial. By isolating a part of the
network or delaying the propagation of blocks, attackers can force nodes to
waste part of their mining power as some of the blocks they create are
discarded. Partitioning also enables the attacker to filter transactions that
clients try to include in the blockchain. In both cases, miners lose potential
revenue from mining and render the network more susceptible to double spending
attacks as well as to selfish mining attacks~\cite{eyal2014majority}. Nodes representing merchants, exchanges and other large entities are thus unable to secure their transactions, or may not be able to broadcast
them to the network to begin with. The resulting longer-term loss of trust in
Bitcoin security may trigger a loss of value for Bitcoin. Attackers may even
short Bitcoin and gain from the resulting devaluation~\cite{kroll2013economics}.

Our work underscores the importance of proposed modifications which
argue for encrypting Bitcoin traffic~\cite{bitcoin_bip_151} or traffic exchanged among miners~\cite{lef}. Yet, we
stress that not all routing attacks will be solved by such
measures since attackers can still disrupt connectivity and isolate nodes by dropping Bitcoin packets instead of modifying them.

\myitem{Contributions} Our main contributions are:\footnote{Our software, measurements and scripts can be found online at \\ \texttt{\url{https://btc-hijack.ethz.ch}}}

\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{1pt}
%
\item The first comprehensive study of network attacks on Bitcoin
(Section~\ref{sec:overview}) ranging from attacks targeting a single node to attacks affecting the network as a whole.
%
\item A measurement study of the routing properties of Bitcoin (Section~\ref{sec:topology}). We show that Bitcoin is highly centralized: few ASes host most of the nodes while others intercept a considerable fraction of the connections. \remove{({\raise.17ex\hbox{$\scriptstyle\sim$}}30\%)}
%
\item A thorough evaluation of the practicality of routing attacks
(partitioning and delay attacks). Our evaluation is based on an extensive set of
measurements, large-scale simulations and experiments on the actual Bitcoin
software and network.
%
\remove{
\item An in-depth evaluation on persistence  of partition attacks
using a large testbed of 1{,}050 Bitcoin nodes (Section~\ref{sec:eval_partition}).
We show that partitions are not persistent after the attack due to the natural churn of the network.
}
%
\remove{
\item A fully-working implementation of a Bitcoin interception software
(Section~\ref{sec:delay_results}) that AS-level adversaries can use to delay block propagation; along with the implementation of a realistic
event-driven Bitcoin simulator to measure the network-wide effect of delay
attacks. We show that delay attacks are very effective for small subset of nodes, but not realistic at the network-wide level if pools are multi-homed enough.
}
%
\item A comprehensive set of countermeasures (Section~\ref{sec:countermeasures}), which can benefit even early adopters.

\end{itemize}

While our measurements are Bitcoin-specific, they carry important
lessons for other cryptocurrencies which rely on a
randomly structured peer-to-peer network atop of the Internet, such as Ethereum~\cite{ethereum}, Litecoin~\cite{litcoin}, and ZCash~\cite{zcash,sasson2014zerocash}.




==> sp copy/overview.tex <==
\section{Routing attacks on Bitcoin}
\label{sec:overview}

\begin{figure}[t]
 \centering
 \includegraphics[width=\columnwidth]{figures/summary_figure.pdf}
 \caption{Illustration of how an AS-level adversary (AS8) can intercept Bitcoin traffic by hijacking prefixes to isolate the set of nodes $P = (A,
B, C, D, E, F)$.}
 \label{fig:overview_partition}
\end{figure}

In this section, we give an overview of the two routing attacks we
describe in this paper: \emph{(i)} partitioning the Bitcoin network (Section~\ref{ssec:partition_overview}); and
\emph{(ii)} delaying the propagation of blocks. For each attack, we briefly
describe its effectiveness and challenges as well as its impact on the Bitcoin
ecosystem (Section~\ref{ssec:delay_overview}).

\remove{
\begin{figure}[t]
 \centering
 \includegraphics[width=\columnwidth]{figures/partition}
 \caption{Illustration of how an AS-level adversary (AS8) can intercept Bitcoin traffic by hijacking prefixes or leveraging natural connectivity and then attacking either specific nodes of the network as a whole. \laurent{Update caption}}
 \label{fig:partition_sumary}
\end{figure}
}

\subsection{Partitioning the Bitcoin Network}
\label{ssec:partition_overview}

In this attack, an AS-level adversary seeks to isolate a set of nodes $P$ from
the rest of the network, effectively partitioning the Bitcoin network into two
disjoint components. The actual content of $P$ depends on the attacker's
objectives and can range from one or few merchant nodes, to a set of nodes holding a considerable percentage of the total mining power.

\myitem{Attack} The attacker first diverts the traffic destined to nodes in
$P$ by hijacking the most-specific prefixes hosting each of the IP address. Once on-path, the attacker intercepts the Bitcoin traffic
(e.g., based on the TCP ports) and identifies whether the
corresponding connections cross the partition she tries to create. If so, the attacker drops the packets. If not, meaning the connections are contained within $P$, she monitors the exchanged Bitcoin messages so as to detect ``leakage points''. Leakage points are nodes currently within $P$, which maintain connections with nodes outside of $P$, that the attacker cannot intercept, namely ``stealth'' connections. The attacker can detect these nodes automatically and isolate them from others in $P$ (Section~\ref{sec:partition}). Eventually, the attacker isolates the maximal set of nodes in $P$ that can be isolated.

\myitem{Example} We illustrate the partition attack on the simple network in Fig.~\ref{fig:overview_partition} that is composed of 8 ASes, some of which host Bitcoin nodes. Two mining
pools are depicted as a green (left) and a red (right) region. Both pools
are multi-homed and have gateways in different ASes. For instance, the
red (right) pool has gateways hosted in AS4, AS5, and AS6. We denote the
initial Bitcoin connections with blue lines, and those that have been diverted via hijacking with red lines. Dashed black lines
represent private connections within the pools. Any AS on the path of a connection can intercept it.

Consider an attack by AS8 that is meant to isolate the set of nodes $P = (A,
B, C, D, E, F)$. First, it hijacks the prefixes
advertised by AS1, AS2 and AS6, as they host nodes within $P$,
effectively attracting the traffic destined to them. Next, AS8 drops all
connections crossing the partition: i.e., $(A,J)$, $(B,J)$ and $(F,G)$. 

Observe that node $F$ is within the isolated set $P$, but is also a gateway of the red pool with which $F$ most likely communicates. This connection may not be based on the Bitcoin protocol
and thus it cannot be intercepted (at least, not easily). As such, even if the attacker
drops all the Bitcoin connections she intercepts, node $F$ may still learn about transactions
and blocks produced on the other side and might leak this
information within $P$. Isolating $P$ as such is infeasible. However, AS8 can identify that node $F$ is the leakage point during the attack and exclude it
from $P$, essentially isolating $I'= (A, B, C, D, E)$ instead. This
$I'$ is actually the maximum subset of $P$ that can be isolated from the
Bitcoin network.

%For example AS2, AS3 and AS4 can intercept the connection from node $A$ to node $J$, while no AS can intercept the connection from node $F$ to the Stratum server of the pool it belongs.

\myitem{Practicality} We extensively evaluate the practicality of isolating sets of nodes of various sizes
(Section~\ref{sec:eval_partition}). We briefly summarize our findings.
\emph{First}, we performed a real BGP hijack against our own Bitcoin nodes
and show that it takes less than 2 minutes for an attacker to divert Bitcoin
traffic. \emph{Second}, we estimated the number of prefixes to hijack so as to
isolate nodes with a given amount of mining power. We found that hijacking only 39
prefixes is enough to isolate a specific set of nodes which accounts for almost 50\% of the overall mining
power. Through a longitudinal analysis spanning over 6 months, we
found that much larger hijacks happen regularly and that some of them have
already impacted Bitcoin traffic. \emph{Third}, we show that, while effective, partitions do not last long after the attack stops: the two components of the partition quickly reconnect, owing to natural churn. Yet, it takes hours for the two components to be densely connected again.

\myitem{Impact} The impact of a partitioning attack depends on the number of
isolated nodes and how much mining power they have. Isolating a few nodes essentially constitutes a denial of service attack and renders them
vulnerable to 0-confirmation double spends. Disconnecting a considerable amount of mining power can lead to the creation of two
different versions of the blockchain. All blocks mined on the side with the
least mining power will be discarded and all included transactions are likely
to be reversed. Such an attack would cause revenue loss for the miners on the
side with least mining power and a prominent risk of double spends. The side
with the most mining power would also suffer from an increased risk of selfish
mining attacks by adversaries with mining power.

\begin{figure}[t]
 \centering
 \includegraphics[width=.75\columnwidth]{figures/delay_overview}
 \caption{Illustration of how an AS-level adversary (AS8) which naturally intercepts a part of the traffic can delay the delivery of a block for 20 minutes to a victim node ($C$).}
 \label{fig:delay_overview}
\end{figure}

\subsection{Slowing down the Bitcoin network}
\label{ssec:delay_overview}

In a delay attack, the attacker's goal is to slow down the propagation of new
blocks sent to a set of Bitcoin nodes without disrupting their connections.
As with partitioning, the attack can be targeted, aimed at selected nodes,
or network-wide, aimed at disrupting the ability of the entire network to reach
consensus~\cite{decker2013information}. Unlike partitioning attacks though, an
attacker can delay the overall propagation of blocks towards a node even if
she intercepts a subset of its connections.

\myitem{Attack} Delay attacks leverage three key aspects of the Bitcoin
protocol: \emph{(i)} the asymmetry in the way Bitcoin nodes exchange blocks
using \textsf{INV}, \textsf{GETDATA}, and \textsf{BLOCK} messages
(Section~\ref{sec:background}); \emph{(ii)} the fact that these messages are
not protected against tampering (unencrypted, no secure integrity checks); and \emph{(iii)} the fact that a Bitcoin node
waits for 20 minutes after having requested a block from a peer before requesting
it again from another peer.
These protocol features enable an attacker intercepting even one direction of the victim's connection
to delay the propagation of a block, as long as this connection is traversed by either the actual
  \textsf{BLOCK} message or the corresponding \textsf{GETDATA}.

Specifically, if the attacker intercepts the traffic \emph{from} the victim,
she can modify the content of the \textsf{GETDATA} message the victim
uses to ask for blocks. By preserving the message length and structure and by
updating the TCP and Bitcoin checksums, the modified message is accepted by the
receiver and the connection stays alive. \remove{Next, the attacker can yet
again tamper with another \textsf{GETDATA} message to trigger a delayed (up to
20 minutes) delivery of the block to prevent the victim from disconnecting.} If
the attacker intercepts the traffic \emph{towards} a node, she can instead
corrupt the content of the \textsf{BLOCK} message such that the victim considers
it invalid. In both cases, the recipient of the blocks remains uninformed for 20
minutes. \remove{Modifying these messages is easy and could even be done in the
data plane (Section~\ref{sec:delay_results}).}

\remove{
Unlike partitioning attacks, an attacker can delay the overall propagation of
the blocks towards a node even if she intercepts a subset of the node
connections. Intercepting even one direction one of one connection is enough as
long as this connection sees some \textsf{BLOCK} or \textsf{GETDATA} of a block.
}

\myitem{Example} As an illustration, consider Fig.~\ref{fig:delay_overview}, and assume that AS8 is the attacker and $C$, the
victim. Suppose that $A$ and $B$ both advertise a block (say, block $X$)
to $C$ via an \textsf{INV} message and that, without loss of generality, the
message from $A$ arrives at $C$ first. $C$ will then send a \textsf{GETDATA}
message back to $A$ requesting block $X$ and start a 20 minute timeout count. By modifying the content of the \textsf{GETDATA} node $A$ receives, AS8 indirectly controls what node $A$ will send to node $C$.
This way the attacker can delay the delivery of the block by up to 20 minutes while avoiding detection and disconnection.
Alternatively, AS8 could modify the \textsf{BLOCK} message.


\myitem{Practicality} We verified the practicality of delay attacks by
implementing an interception software which we used
against our own Bitcoin nodes.
We show that intercepting 50\% of a node connections is enough to keep the node uninformed for 63\% of its uptime (Section~\ref{sec:delay_results}). %We also investigated other implementation
%alternatives, including hardware-based ones, to make the tool more scalable.

We also evaluated the impact that ASes, which are naturally
traversed by a lot of Bitcoin traffic, could have on the network using a
scalable event-driven simulator. We found that due to the relatively high
degree of multi-homing that pools employ, only very powerful coalitions of network
attackers (e.g., all ASes based in the US) could perform a network-wide delay attack. Such an attack is thus unlikely to occur in practice.
\remove{Particularly, all US-based ASes can increase the fork rate to 30\% from the
normal 1\%.} %However, a higher-degree of multi-homing (5 providers or more)
%would render even very powerful adversary ineffective.

\myitem{Impact} Similarly to partitioning attacks, the impact of a delay attack
depends on the number and type (e.g., pool gateway)
of impacted nodes. At the node-level, delay attacks can keep the
victim eclipsed, essentially performing a denial of service attack or rendering
it vulnerable to 0-confirmation double spends. If the node is a gateway of a
pool, such attacks can be used to engineer block races, and waste the mining power of the pool. Network-wide attacks
increase the fork rate and render the network vulnerable to other exploits. If a sufficient number of blocks are
discarded, miners revenue is decreased and the network is more vulnerable
to double spending. A slowdown of block transmission
can be used to launch selfish mining attacks by adversaries with mining power.

%the AS-level attacker exploits access this Bitcoin traffic to disrupt either a small set of nodes or the system as a whole (Section~\ref{ssec:summary_attack}).


%We start by describing how the attacker can get on path and discusses how does
%Despite this, it takes a lot of time for the isolated components to re-establish connections to each
%other nodes within them reach consensus almost immediately.






\remove{

In this attack the adversary aims at isolating a set of Bitcoin nodes from the rest of the network. The attacker might choose to isolate specific nodes, pools or a percentage of the overall mining power.

%Maybe it would be more precise to say that the difficulty of the attacks grows with the outside connectivity of a part to isolate? If an isolation island maintains a single connection out, tearing out that connection is enough. Maria: I don't agree in that you would still have to isolate all the prefixes of the island as you don't know the exact or future connectivity 
Intuitively the difficulty as well as the effectiveness of the attack grow with the number of ASes the isolated nodes are hosted as well as the complexity of their internal topology (degree of multi-homing, number of gateways).


Assume that the attacker has access to a BGP enabled network, a list of the IPs of the Bitcoin nodes as well as a mapping of gateways per pool. The attack is performed in two steps. Firstly, the attacker attracts all traffic destined to the Bitcoin nodes he wants to isolate. This is done by hijacking their prefixes. Secondly, he blocks the flow of information between the isolated part and the rest of the network, effectively forming a partition. This can be achieved either by destroying messages that contain specific information or by completely dropping connection crossing the partition. 

Three main factors make the attack challenging in practice: \emph{(i)} the attacker might have an incomplete or obsolete topology view; \emph{(ii)} mining pools are mostly multi-homed and their internal structure and/or protocols are private and complex; \emph{(iii)} hijacks cannot divert inra-AS traffic;
In Section ~\ref{sec:}, we show that the attacker can address these challenges by cumulatively constructing the partition. Particularly, the attacker needs to slowly increase the size of the isolated part, by increasing the number of hijacked prefixes, while ensuring that there is no leakage until the desired size is reached. Optionally, the attacker might use hijacking to augment his view of the topology prior to the actual attack ~\ref{sec:}. In section  ~\ref{sec:} we also discus how the attack could address additional challenges such as limiting the amount of prefixes, dealing with the diverted load.


As an illustration, consider that AS8 is an attacker in Fig.~\ref{fig:overview}. he should first find a feasible partition. For instance, a partition that leaves node G on one side and the rest of the network on the other is not feasible, because G belongs to a multi-homed pool and AS8 cannot intercept connections within the pool. Same holds for a partition that leaves node A alone on one side, as the attacker cannot intercept connection between A and B or A and C because they belong to the same AS. However, a partition with (A, B, C, D, E) in one side is feasible.  In this case the attacker needs to hijack all the prefixes advertised by AS1 and AS2. The attacker has to continually monitor the partition to detect leakage. Leakage can be caused if a new node hosted in AS2 but in a different prefix than that of nodes A, B, C, connects to the Bitcoin network and chooses to peer with any the isolated nodes (A, B, C, D, E) and any of the rest of the network.  In this case the attacker might need to hijack its prefix as well in order to enforce the partition. 

 We verified the practicality of the attack by hijacking and isolating our own Bitcoin nodes connected to the live network. We found that it only takes few seconds for a prefix hijack to propagate in the Internet and for the diverted traffic to reach the attacker. We describe this experiment in Section~\ref{sec:}We further evaluated the long term influence of a 50\%-50\% partition
after the hijack has been mitigated in a testbed of 1050 nodes running the
default bitcoind (Section~\ref{fig:partition}). We show that the Bitcoin network almost heals immediately from a partition attack in the sense that consensus is quickly reached again once the partition starts to leak, i.e. whenever (even few) connections start bridging the once-disconnected components. 
 
\subsection{Attack \#2: Delay Node traffic}
 In this attack, the attacker aims at delaying the propagation of blocks to a set of nodes of the network as a whole.
To do that, the attacker manipulates the exchanged Bitcoin messages. A 20 minutes delay of a block delivery is possible because of the way Bitcoin nodes request blocks from their peers to delay block delivery for 20 minutes by .

The attacker is assumed to be naturally traversed by either some of the Bitcoin traffic of the victim set of nodes or a considerable percentage of Bitcoin traffic in general.
This assumption implies that the attacker is most likely either the direct provider of the victim nodes or a large and well-established AS.
As such, the main challenge of the attacker is to avoid detection as that would severely harm its reputation. To address this challenge, the attacker needs to keep the packet manipulation opaque to both TCP and Bitcoin protocols. 


 As an illustration, AS3 can perform a delay attack against node J even though it does not intercept all of its connections. If J receives an \textsf{INV} message for a new block from nodes A
B and H and either A or B advertised the block before H then AS3 can delay its
delivery for 20 minutes, effectively eclipsing J. In practice, modifying the packets on-the-fly is challenging for the attacker as it must
ensure it goes unnoticed by the recipient. We explain how this can be done in Section \ref{}.


We verified the
practicality of the attack by implementing a complete prototype which we use to
attack our own Bitcoin nodes and found that an attacker can eclipse a victim
for 63\% of its uptime even when intercepting half of its connections (see
Section~\ref{sec:delay}).
We further evaluated the effectiveness of delay attacks when performed
network-wide using a realistic simulator. We found that the effectiveness of
delay attacks decreases with the degree of multi-homing adopted by the mining
pools. 



%the AS-level attacker exploits access this Bitcoin traffic to disrupt either a small set of nodes or the system as a whole (Section~\ref{ssec:summary_attack}).

%We start by describing how the attacker can get on path and discusses how does
%Despite this, it takes a lot of time for the isolated components to re-establish connections to each
%other nodes within them reach consensus almost immediately.



\subsection{Impact:}
\label{ssec:summary_impact}

The impact of both attacks varies with respect to the number and type (regular nodes or gateway of pool) of the impacted Bitcoin nodes. At the node-level such attacks can keep the victim eclipsed, essentially performing a denial of service attack or rendering it vulnerable to 0-confirmation double spends. \rremove{ If the node is a gateway of a pool such attacks can be used to engineer block races.}
Network-wide attacks such as a isolating a considerable amount of mining power or sufficiently delaying the propagation of blocks to increase the fork rate renders the network extremely vulnerable to all sorts of exploits. As a sufficient number of blocks are discarded, the  miner's revenue is deducted and the network is more vulnerable to double spends. Especially in the case of the partition, all transactions included in the chain of the side with the least mining power are likely to be reversed. In the case of delaying, significant slowdown of block transmission can be used to launch selfish mining attacks by adversaries with mining power.
}


==> sp copy/partition.tex <==
\section{Partitioning Bitcoin }
\label{sec:partition}

In this section we will extensively describe how an attacker plans, enforces and maintains a partition.
For clarifying the procedure we included a piece of pseudo-code summarizing the most important steps of the attack which we explain in detail in the following.

\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother

\begin{algorithm}
\caption{Create an effective partition}\label{euclid}
\begin{algorithmic}[1]
\algrenewcomment[1]{\(\triangleright\) #1}

%import bitcoin node IPs
%hijacked\_nodes;;;;

\Procedure{Partition}{}


\Comment{ \textbf{Attack Planning}} \ref{ssec:plan}

\State $\textit{IP\_list} \gets \text{list of IPs of bitcoin nodes }$




\State  $\textit{hijacked\_nodes} \gets \textit{pick\_component(IP\_list)}$


\Comment {\textbf{ Disconnect }} \ref{sssec:disconnect}

\For{each node $n$ in $hijacked\_nodes$}
%\State \texttt{<do stuff>}
\For{each node $p$ in $n.peers$}
\If {$p$ not in $hijacked\_nodes$}
\State drop connection(p, n)

\EndIf
\EndFor
\EndFor


\Comment {\textbf{ Maintain partition }} \ref{sssec:leakage}
\While {true}

%while true: if leakage is detected:
%node= leakahe
\State $\textit{node} \gets \text{Detect\_leakage()}$

\For{each node $p$ in $node.peers$}
\If {$p$  in $hijacked\_nodes$}
\State drop connection(p, node)
\EndIf
\EndFor
\EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{\textbf{Attack Planning}}
\label{ssec:plan}
We first look at how the attacker prepares his attack. The preparation phase includes two phases: \emph{(i)} discovering IPs of active bitcoin nodes;  \emph{(ii)} deciding on a partition.



\subsubsection{\textbf{Phase \#1: Inferring topology}} 


\label{ssec:augement_topo}

During this phase the attacker composes a list the active bitcoin nodes' IPs. Optimally, this list is accompanied with some of the gateways of known pools. We will refer to this information as topology. The attacker can simply downloading such a list from one of the known bitcoin sites to infer the topology \cite{bitnodes}. The effectiveness of the attacker though, can be significantly increased, had he used a more precise topology. To do that the attacker can
 discover more nodes and/or identify the pool gateways in the topology. 

Before mentioning some of the ways an attacker can discover more nodes we look at the reasons why the publicly available lists might be incomplete. Nodes that do not accept incoming connections to prevent DDoS attacks or just because they are behind a NAT, as well as nodes that are very new to the network are most likely not included in those list. That is due to the way nodes are discovered and of the time a complete crawling of the network takes. Among other things, the attacker could very easily use the following two methods to discover unknown nodes. First, the attacker can by itself have some bitcoin nodes which it uses to learn more IPs. Even a node that does not accept incoming connections is indeed connected to some nodes which are likely to advertise its IP via \textsf{ADDR} messages. Second, the attacker could combine different sources of information such as multiple sites as well as multiple consecutive versions of lists from the same source. Different source might have different ways of collecting the IPs and also combining information from multiples time frames limits the risk of not including nodes that were not active just during the crawling.


In addition, it would be also useful for the attacker to identify nodes as gateways of specific pools. This information can significantly help him in planning the partition as we will explain in the following Subsection \ref{ssec:plan} . To do that the attacker can use the techniques described in research papers such as \cite{coinscope} and/or leverage the access he can obtain to bitcoin traffic via hijacking as an active way to learn the topology. We briefly introduce two such methods.
First, the attacker may hijack the pool's stratum servers to discover connections that they establish and thus reveal the gateways they connect to. Connections to formed between the pool's stratum server and its gateways are via bitcoind's RPC access, and can be easily distinguished.
Second, the attacker can hijack the relay network to discover connections used by the large mining pools. The relay network has a public set of six IPs that pools connect to. By hijacking these, one may learn very critical points of the pool's infrastructure. Specifically, it will not be hard to identify a pool by observing the blocks it publishes to the relay network. 



\subsubsection{\textbf{Phase \#2: Finding a cut}}
\label{ssec:plan}


During this phase, the attacker decides which nodes one of the two components contains. The goal of the attacker is to find a partition that is more likely to be effective. We will first discus which partitions are effective as well as how the attacker can approximate such a partition.

%\myitem{Effective partition}
 The main threat of a partition's effectiveness is leakage. Leakage can occur when two nodes in different components are connected through a channel that the attacker cannot intercept. If all those connections (all pairs of nodes with such connections) are within one component the corresponding  partition is effective.
 We distinguish three types of connections the attacker cannot intercept: \emph{(i)} intra-AS connections;  \emph{(ii)} intra-pool connections; \emph{(iii)} direct pool to pool connections.

\myitem{intra-AS} Connection within the same AS cannot be intercepted by the attacker because their traffic is local to the AS and will thus not leave the AS.\maria{@laurent can you say it better?} For example, in Figure \maria{FILLME} nodes A and B are in the same AS. The traffic between them will never get outside of their AS even during a hijack. This situation can be problematic for the partition, if nodes A and B connect to each other and belong to different components of the partition. In this case they will exchange the state of the components they belong to, effectively leaking information from one component to the other. To address this issue the attacker would always put nodes of the same AS in the same component. This can be easily guaranteed as the attacker can easily infer which AS each IP is hosted to.

\myitem{intra-pool} Connections among nodes that belong to the same pool cannot be intercepted because they might use proprietary protocols. Since mining pools are multi-homed and distributed among different locations, their gateways might be hosted in different ASes, which can of course be placed in different components. If that happens, the pool they belong would get information from both components and probably disseminate this information from one component to the other, effectively acting as a bridge between them. For example in Figure \maria{FILLME} if AS1 is placed in one component and AS2 in the other then the green pool will get information from both components. The green pool then can instruct its gateways nodes E and D to propagate the learned information from E to D and from C to B. In this case, although there is no bitcoin connection crossing the partition the two components will still be connected. 
Intuitively, the attacker would need to include all gateways of a pool in the same component to address this issue. If the attacker is aware of all the gateways of a pool, he can easily avoid this indecent. If the attacker only knows some of the gateways or none at all, he can still try a partition and modify it on-the-fly until it is effective. We explain this procedure in \ref{sssec:leakage}.  


\myitem{Pool to Pool} 
Some pools might connect directly to each other with protocols different than bitcoin. Such a mesh connecting many large pools today is the bitcoin relays. 
Since the IPs of the relays are publicly available and the BGPsec is not used the attacker can hijack the relays and easily disconnect them. Note that this is different from a DoS attack directed to the IPs of relays, which are indeed easier to handle.
If pools have secret agreements to each other then they should be both placed in the same component. That cannot be done a priori as the attacker might not have  that information. However, the attacker can still infer such relations on-the-fly as explained in \ref{sssec:leakage} \maria{should we say here about the security/ obscurity?}


\subsection{\textbf{During the attack}}



The actual attack can be split into two phases. In the former phase the attacker cuts all connections between nodes of different components. In the latter phase the attacker continually detects leakage and disconnect its source from one of the component.


\subsubsection{\textbf{Phase \#1: Disconnect}}
\label{sssec:disconnect}

 Once the attacker decides on a partition, he needs to hijack all the prefixes that correspond to nodes in one of the components. We will refer to these nodes as hijacked nodes, the component they belong to as hijacked component and the ASes these nodes are hosted in as hijacked ASes. 

 The attacker will receive the traffic that is destined to the nodes whose prefixes he hijacked. At this point, he distinguishes the bitcoin traffic from the regular and investigate it further before sending it to the actual destination. From this traffic the attacker can discover all the connections the hijacked nodes have. He then classifies the connections each hijacked node has as one of three types: \emph{(i)} connections to peers hosted in hijacked prefixes; \emph{(ii)} connections to peers hosted in hijacked ASes but whose prefixes are not yet hijacked; \emph{(iii)}connections to peers hosted in hijacked ASes that are not hijacked. Connections are treated differently based on their type.
The first type of connections are entirely within the hijacked component and are thus allowed by the attacker. With regards to the second type, the existence of a peer hosted within the hijacked ASes, but whose prefix is not hijacked denotes that the attacker was unaware of this node. Since the attacker needs to include all nodes of an AS within the same component, the attacker would have to hijack the prefix of the sofar-unknown node as well. After that the connection would be allowed as it will be classified to the first type of connections. 
The third type of connections are connections that cross the partition. The attacker would drop such connections. If the connections was initially established by the hijacked node, it will try to establish a new connection to replace the dropped one. The new connection would be again classified and treated as described above.




\subsubsection{\textbf{Phase \#2: Partition Maintenance}}
\label{sssec:leakage}



 The methodology described above is enforced throughout the attack to ensure that there is no connection the attacker can control that crosses the partition. Even so, there will be connections that the attacker would not be able to intercept and do cross it. Thus the attacker would need to first detect the end of the connection that is within the hijacked component and then disconnect it from the rest of the nodes of this component.

Particularly, if there is a node within the hijacked nodes that is connected to the other component, it will learn about blocks that are mined in the other component. To propagate these blocks to nodes within the hijacked component it would first send an inventory message with the block's hash to a node in the component. As the attacker sees all traffic to the hijacked nodes and the hijacked nodes are only connected to each other, he sees all exchanged traffic/information within the partition. Once the attacker sees the hash being advertise he concludes that the sender has a connections to the other component. To avoid leakage of information from this node to the hijacked component the attacker cuts all its connections to the hijacked nodes. If the node never tries to propagate the block, it will indeed never be detected, but it will also never cause leakage, in which case it is not a threat for the partition. 
As the node might also have connections that the attacker cannot intercept within the hijacked component, cutting its bitcoin connections to hijacked nodes might not be enough to stop the leakage. In this case the nodes it is connected to will be also detected as points of leakage and excluded from the hijacked component. 


%when does leakage happen
%when is it dangerous for the partition




\remove{


\subsubsection{Why leakage can occur}

\myitem{The attacker might have an incomplete or obsolete topology view.}
In othe r owrds the attacker might not be aware of the existance of node X.
Node X who is hosted in ASX and routed according to PrefX can bridge the partition if and only if all the following hold
\begin{itemize}
\item ASX is within the isolated-hijacked part (if it is in the other half X will never be allowed to connect to any of the isolated nodes)
\item There is no other node is in the same prefX (if there is prefX is already hijacked)
\item X connected to at least one node in ASX (unlike to happen based on the prefix preference in bitcoind)
\item X connected to at least one node from the other part (to act as a bridge)
\end{itemize}

\myitem{Mining pools are mostly multi-homed and their internal structure and/or protocols are private and complex.}
This can be problematic for the partition if there is an unknown gateway unknown gateway G of pool X in ASX such that:
\begin{itemize}
\item G belongs to the isolated part
\item ASX is not in the isolated part 
\end{itemize}


  (b) Mining pools are mostly multi-homed and their internal structure and/or protocols are private and complex. (c)Hijacks cannot divert inra-AS traffic.






\subsection{Limitations -Leakage}

\subsubsection{Circumstances that can break the partition}

\myitem{a node X hosted in ASX and routed according to PrefX can break the partition iff}
\begin{itemize}
\item X is a new node (otherwise the adversary would know based on the assumptions and would have hijackes its prefix) \maria{maybe remove that to talk about pre-attack plans}
\item ASX is within the isolated-hijacked part (if it is in the other half X will never be allowed to connect to any of the isolated nodes)
\item There is no other node is in the same prefX (if there is prefX is already hijacked)
\item X connected to at least one node in ASX (unlike to happen based on the prefix preference in bitcoind)
\item X connected to at least one node from the other part (to act as a bridge)
\end{itemize}


\maria{not sure if we want to include this case , maybe it is covered by the assuption that the attacker knows the topology }

\myitem{secret agreement between pools in different parts}
The partition is not feasible the two pools must be seen as one. The attacker has to find another partition or drain all the hijacked traffic. But we focus on the default protocol



\subsubsection{Circumstances that cannot break the partition}
\maria{or find a way to include this cases above}



\myitem{NATed or hidden nodes cannot bridge the partition.}
NATed nodes can only connect to public IPs. By hijacking the prefixes corresponding to a 
partition, the attacker gains control over every connection crossing it, including the 
ones from NATed nodes. By killing any bitcoin connection crossing the partition, the 
attacker effectively disconnects any bridge created by a NATed node. 


\myitem{Bitcoin relays ~\cite{relays} cannot guarantee the security of the protocol.}
They indeed improve the performance of Bitcoin. They might even be able to secure bitcoin 
against known attacks but they are still far from guaranteeing routing security. Indeed, 
the IPs of the relays are publicly available; ISPs are sometimes chosen based on pricing (
acknowledged on the website), and BGPSec is not used. All these facts make relays also 
vulnerable to both hijacking and passive attacks.


\subsection{Detecting leakage}


\subsection{Reacting to leakage}
\begin{itemize}
\item increase hijacked prefixes randomly or based on the address books of nodes look for nodes even though they do not seem active at the moment  (new node)
\item analyze Stratum server (and relays) traffic to find which are the nodes they communicate with (new gateway)
\item act as a black hole (secret agreement)
\item recalculate a feasible partition assuming two pools as one (secret agreement)
\end{itemize}

\maria{In general this part is weak I think we should avoid saying that we do staff to discover the topology}
}







==> sp copy/partition_2.tex <==
\section{Partitioning Bitcoin}
\label{sec:partition}

% The basic work flow of an attacker is depicted in Fig.~\ref{fig:partition_sumary}.
 %Due to the dynamic and complex nature of the Bitcoin network the adversary might need to reconsider the atatck plan multiple times the three phases until his attack is successful.

\begin{figure*}[t]
	\centering
	\begin{subfigure}[t]{.22\textwidth}
  		\includegraphics[width=\textwidth]{figures/visible}
		\caption{Feasible partition}
		\label{fig:visible}
	\end{subfigure}
	%\hfill
	\qquad \qquad 
	\begin{subfigure}[t]{.22\textwidth}
		\includegraphics[width=\textwidth]{figures/intra_as}
		\caption{Infeasible partition because of intra-AS connections }
		\label{fig:intraAS}
	\end{subfigure}
 	%\hfill
	\qquad \qquad
	\begin{subfigure}[t]{.30\textwidth}
		\includegraphics[width=\textwidth]{figures/intra_pool}
		\caption{Infeasible partition because of intra-pool connections}
		\label{fig:intrapool}
	\end{subfigure}
  \caption{Not all Bitcoin connections can be diverted by an attacker implying that some partitions cannot be formed.}
 \label{fig:partition_possible}
\end{figure*}

In this section, we elaborate on partition attacks in which an AS-level adversary seeks to isolate a set of nodes $P$. We first describe which partitions are feasible by defining which connections may cause information leakage (Section~\ref{ssec:hidden}) to the isolated set.  We then discuss how an attacker may better select a $P$ that is feasible,
if she has some view of the Bitcoin topology (Section~\ref{sssec:plan}).
Next, we walk through the entire attack process, starting with the interception of Bitcoin traffic, the detection of leakage points and the adaptation of $P$ until the partition is successfully created (Section~\ref{ssec:disconnection}). In particular, we present an algorithm which, given a set of nodes $P$, leads the attacker to isolate the maximal feasible subset. Finally, we prove that our algorithm is correct (Section~\ref{ssec:proof}).


\remove{As well as why the latter are 
The main factor that makes the attack challenging is the existence of connections that the AS-level adversary does not see and that he cannot cut. If such connections cross the partition, information cannot be prevented from flowing from one component to the other in which case the partition is infeasible. Thus, the attacker should detect these connections and modify $P$ into a $P'$ (subset of P) such that they are no such connections bridging the partition. 
}
 

\remove{
\begin{algorithm}[t!]
	\small
	\SetKwInOut{Input}{Input}
	\KwIn{\textcolor{mygray}{-} $(G_1,G_2)$, a partition of the known Bitcoin IP addresses; and \newline 
	\textcolor{mygray}{-} $P = (P_1, \cdots, P_n)$, the sets of known Bitcoin IP addresses acting as gateways for each mining pool.}
	\KwOut{\emph{true} or \emph{false}}
	\Begin{
			\If{$AS(G_1) \cap AS(G_2) \neq \varnothing$}{
				\Return{false}\,\;
			}
			\For{$P_i \in P$}{
				\If{$\neg (AS(P_i) \cap AS(G_1) \oplus AS(P_i) \cap AS(G_2))$}{
					\Return{\text{false}}\,\;
				}
			}
			\Return{true}\,\;
	}
\caption{Algorithm testing whether a partition is feasible given a view of the Bitcoin topology.}
\label{alg:is_partition_possible}
\end{algorithm}
}

\subsection{Characterizing feasible partitions}
\label{ssec:hidden}

An attacker can isolate a set of nodes $P$ from the network if and
only if \emph{all} connections $(a,b)$ where $a \in P$ and $b \not\in P$
can be intercepted. We refer to such connections as \emph{vulnerable} and to
connections that the attacker cannot intercept as \emph{stealth}.

\myitem{Vulnerable connections:} A connection is \emph{vulnerable} if: \emph{(i)} an
attacker can divert it via a BGP hijack; and \emph{(ii)} it uses the Bitcoin protocol. The first requirement enables the
attacker to intercept the corresponding packets, while the second enables her to
identify and then drop or monitor these packets. %If both
%requirements are fulfilled the attacker can divert the connection and drop it.

As an illustration, consider Fig.~\ref{fig:visible}, and assume that the
attacker, AS8, wants to isolate $P=\{A,B,C\}$. By hijacking the prefixes
pertaining to these nodes the attacker receives all traffic from nodes $A$ and
$B$ to node $C$, as well as the traffic from node $D$ to node $A$. The path the
hijacked traffic follows is depicted with red dashed lines and the original path
with blue lines. As all nodes communicate using the Bitcoin protocol, their
connections can easily be distinguished, as we explain in
Section~\ref{ssec:disconnection}. Here, AS8 can partition $P$ from the rest of the network by dropping the connection from node $D$ to node $A$.

\myitem{Stealth connections:} A connection is \emph{stealth} if the attacker cannot intercept it. 
We distinguish three types of stealth connections:
\emph{(i)} intra-AS; \emph{(ii)} intra-pool; and \emph{(iii)} pool-to-pool. 

%For each type, we explain why a network attacker fails to intercept them and how these connections can bridge the two sides of a partition
%an attacker aims to create.
% In essence: put all the nodes beloning to one AS on one side of the partition...
\noindent\textit{\textbf{intra-AS:}} An attacker cannot intercept
connections within the same AS using BGP hijack. Indeed, internal traffic does
not get routed by BGP, but by internal routing protocols (e.g., OSPF, EIGRP).
Thus, any intra-AS connection crossing the partition border renders the partition infeasible. Such connections represent only 1.14\% of all the possible connection nodes can create (this percentage is calculated
based on the topology we inferred in Section~\ref{sec:topology}).

As an illustration, consider Fig.~\ref{fig:intraAS} and assume that
the attacker, AS8, wants to isolate $P=\{A,B,C\}$. By hijacking the
corresponding BGP prefixes, AS8 can intercept the connections
running between nodes $A$ and $B$ to node $C$. However, she does not intercept the intra-AS
connection between $A$ and $X$. This means that node $X$ will inform node $A$
of the blocks mined in the rest of the network, and node A
will then relay this information further within $P$. Thus, $P=\{A,B,C\}$ is not
feasible. Yet, observe that isolating $I=\{B,C\}$ is possible. In the
following, we explain how the attacker can detect that $A$ maintains a stealth
connection leading outside of the partition and dynamically adapt to
isolate $I$ instead.

%Mining pools include multiple gateways to interconnect with the peer-to-peer %network. 

\noindent\textit{\textbf{intra-pool:}} Similarly to intra-AS connections, an attacker
 might not be able to cut connections between gateways belonging to the same mining pool.
 This is because mining pools might rely on proprietary or even encrypted protocols for internal communication. %Actually, even if the attacker could intercept these

As an illustration, consider Fig.~\ref{fig:intrapool} and assume that the attacker, AS8, wants to isolate $P=\{A,B,C,D\}$. By hijacking the corresponding prefixes, she would intercept and cut all Bitcoin connections between nodes A, B, C, D and nodes E, F. However, nodes A and F would still be connected internally as they belong to the same (green) pool.
%As such, all the information from node a will be transmitted to and propagated from node A to the rest of $P$. 
Again, observe that while isolating $P=\{A,B,C, D\}$ is not feasible, isolating $I=\{B,C,D\}$ from the rest of the network is possible. 


\remove{
\textit{encrypted intra-pool or inter-pool connections:} An attacker
might not be able to cut connections between nodes that are using an encrypted private channel between them. These may belong to the same mining pool, or to different pools that have agreed to share such a private connection.
This is because %mining pools might rely on proprietary or even ecrypted protocols to communicate
%with their gateways, 
such connections may simply be difficult to identify. %Actually, even if the attacker could intercept these
%communications, they will be too hard to distinguish as the particularly used
%protocol might be different per pool 
 As such,
if a pool uses encrypted tunnels to connect between its multiple gateways or to another pool that is outside of $P$, this connection would act as a bridge, rendering the partition
infeasible.

}


\noindent\textit{\textbf{pool-to-pool:}} Finally, an attacker cannot
intercept (possibly encrypted) private connections, corresponding to peering agreements between mining pools. From
the attacker's point of view, these connections can be treated as intra-pool
connections and the corresponding pair of pools can be considered as one larger pool. Note that such connections are different than public initiatives to interconnect all pools, such as the Bitcoin relays~\cite{relays}. Unlike private peering agreements, relays \emph{cannot} act as bridges to the partition (see Appendix~\ref{ssec:faq}). 


\remove{
Consider Fig.~\ref{fig:partition_possible}, and assume that the attacker, AS8, wants to
isolate $P=\{A,B,C\}$ in each case. The path the hijacked traffic follows is
depicted with red dashed lines, the original path with blue lines.
In the first case (Fig.~\ref{fig:visible}), all nodes
communicate using the Bitcoin protocol, and connections can easily be intercepted and
distinguished as we explain in \ref{ssec:disconnection}. Here, AS8 can partition $P$ from the rest of the network by simply
dropping the connection from node A to node D.
In the second case (Fig.~\ref{fig:intraAS}) the attacker fails to intercept the intra-AS
connection between $A$ and $X$, and thus fails to establish the partition (observe that here isolating $I=\{B,C\}$ is still possible). Finally, in Fig.~\ref{fig:intrapool} nodes A and F maintain an intra-pool encrypted connection that the attacker fails to identify (the attacker may still isolate $P'=\{B,C,D\}$ in this case). 
}

\subsection{Preparing for the attack}
\label{sssec:plan}
In light of these limitations the attacker can apply two techniques to avoid having stealth connections crossing the partition she creates. First, she can
include in $P$ either all or none of the nodes of an AS, to avoid intra-AS connections
crossing the partition. This can be easily done as the mapping from IPs to ASNs is
publicly available~\cite{caida_ip_to_asn}. Second, she can include in $P$
either all or none of the gateways of a pool, to avoid intra-pool connections crossing
the partition. Doing so requires the attacker to know all the gateways of the
mining pools she wants to include in $P$. Inferring the gateways is outside the
scope of this paper, yet the attacker could use techniques described in~\cite{miller2015discovering} and leverage her ability to inspect the traffic
of almost every node via hijacking (see Appendix \ref{ssec:gw}). Even with the above measures, $P$ may still contain leakage points that the attacker will need to identify and exclude (see below). Yet, these considerations increase the chances of establishing the desired partition as well as reducing the time required to achieve it.

\remove{In any case, due to the hardness of acquiring a perfect topological view and to
the dynamic nature of the Bitcoin network the attacker would need to adapt the partition
during the attack as described in the next Subsection. Even so, a good approximation
of a feasible partition would lead to a more effective attack as the $P'$ will
}

\begin{algorithm}[t]
	\small
	\SetKwInOut{Input}{Input}
	\KwIn{\textcolor{mygray}{-} $P$, a set of Bitcoin IP addresses to disconnect from the rest of the Bitcoin network; and \newline 
	\textcolor{mygray}{-} $S = [pkt_1, \cdots]$, an infinite packet stream of \newline diverted Bitcoin traffic resulting from the hijack of the prefixes pertaining to $P$.}
	\KwOut{False if there is no node $\in P$ that can be verifiably isolated;}
	\textbf{enforce\_partition($P,S$)}:
	
	\Begin{
%			$P' \gets P$\,\;
			$U \gets \varnothing$\,\;
			$L \gets \varnothing$\,\;
			\While{$P \setminus (L \cup U) \neq \varnothing$}{
				\For{$pkt \in S$}{
					\If{$pkt.ip\_src \in P \wedge pkt.ip\_src \notin L $}{ \label{line:is_node_inside}
						$last\_seen[pkt.ip\_dst] = now()$\,\;
						$U \gets U \setminus \{ pkt.ip\_src \}$ \,\;\label{line:add_inactive}
						$detect\_leakage(U, pkt)$\,\;\label{line:detect_leakage}
						
					}
					\Else{
						$drop(pkt)$\,\; \label{line:drop-visible}
					}
					
					\For{$src \in P \wedge src \notin L$}{
						\If{$last\_seen[src] > now() - threshold$}{
							$U \gets U \cup \{ src \}$ \label{line:removal_inactive}
							%$P' \gets P' \setminus \{ pkt.ip\_src \}$\,\; \label{line:removal_inactive}
						}
					}
				%$P'\gets P \setminus (L \cup U)$\,\;
				}
			}
			\Return{false}\,\;
	}
\caption{Partitioning algorithm.}
\label{alg:attack_algorithm}
\end{algorithm}

\begin{algorithm}[t]
	\small
	\SetKwInOut{Input}{Input}
	\SetKwFunction{FRecurs}{FnRecursive}
	\KwIn{\textcolor{mygray}{-} $U$, a set of Bitcoin IP addresses the attacker cannot monitor; and \newline 
	\textcolor{mygray}{-} $pkt$, a (parsed) diverted Bitcoin packet.}
	\textbf{detect\_leakage($U, pkt$)}:
	
	\Begin{
		\If{$contains\_block(pkt) \vee contains\_inv(pkt)$}{
			\If{$hash(pkt) \in Blocks(\neg (P \setminus L))$}{
				$L \gets L \cup \{pkt.ip\_src \}$\,\; \label{line:leakage_detection}
				$drop(pkt)$\,\; \label{line:drop_block}
			}
		}

	}
\caption{Leakage detection algorithm.}
\label{alg:leakage_algorithm}
\end{algorithm}

\subsection{Performing the attack}
\label{ssec:disconnection}

We now describe how a network adversary can successfully perform a partitioning
attack. The attack is composed of two main phases: \emph{(i)} diverting relevant Bitcoin traffic; and \emph{(ii)} enforcing the partition. In the
former phase, the adversary diverts relevant Bitcoin traffic using BGP
hijacking. In the latter phase, the attacker cuts all vulnerable connections
that cross the partition and excludes from $P$ nodes which are identified as leakage points.
Leakage points are nodes that are connected to the rest of the network via stealth connections.

\myitem{Intercept Bitcoin traffic:} The attacker starts by hijacking all the
prefixes pertaining to the Bitcoin nodes she wants to isolate, i.e. all the
prefixes covering the IP addresses of nodes in $P$. As a result, she receives
all the traffic destined to these prefixes, which she splits into two packet
streams: relevant and irrelevant. Relevant traffic includes any Bitcoin
traffic destined to nodes in $P$. This traffic should be
further investigated. Irrelevant traffic corresponds to the remaining traffic
which should be forwarded back to its legitimate destination. %This practice makes the hijack less disruptive to other protocols and thus more difficult to detect.

To distinguish between relevant and irrelevant traffic, the attacker applies
a simple filter matching on the IP addresses, the transport protocol and ports
used, as well as certain bits of the TCP payload. Specifically, the attacker
first classifies as irrelevant all non-TCP traffic as well as all traffic with
destination IPs which are not included in $P$. In contrast, the attacker
classifies as relevant all traffic with destination or source TCP port the
default Bitcoin port (8333)\remove{and other publicly advertised port numbers (e.g.
via \textsf{ADDR} messages)}. Finally, she classifies as relevant all packets
which have a Bitcoin header in the TCP payload. Any remaining traffic is considered irrelevant.

\myitem{Partitioning algorithm:}
Next, the attacker processes the relevant traffic according to Algorithms~\ref{alg:attack_algorithm} and~\ref{alg:leakage_algorithm}. We start by presenting their goal before describing them in more details.

The high-level goal of the algorithms is to isolate as many nodes in $P$ as possible. To do so, the algorithms identify $L$, the nodes that are
leakage points, and disconnect them from the other nodes in $P$. Also,
the algorithms maintain a set of verifiably isolated nodes  $P'= P\setminus \{U\cup L\}$, 
where $U$ corresponds to the nodes that cannot be monitored (e.g., because they never
send packets). In particular,  Algorithm~\ref{alg:leakage_algorithm} is in charge of identifying $L$,
while Algorithm~\ref{alg:attack_algorithm} is in charge of identifying $U$ and
performing the isolation itself. 

\remove{
The algorithms
also identify $U$, the nodes that cannot be monitored (e.g., because they never
send packets). It then provably isolate the nodes in $P \setminus L \setminus
U$. Algorithm~\ref{alg:leakage_algorithm} is in charge of identifying $L$,
while Algorithm~\ref{alg:attack_algorithm} is in charge of identifying $U$ and
performing the isolation itself.
}
%The goal of
%Algorithm~\ref{alg:attack_algorithm} is twofold. \emph{First}, it isolates $P
%\setminus L$, namely the initial set of nodes the attacker wanted to isolate
%minus the leakage points. \emph{Second}, it identifies nodes within $P$ for %which the attacker cannot detect whether they are isolated or not. We denote %this set of non-monitored nodes with $U$. By applying these
%two algorithms, the maximal feasible subset of nodes in $P$ is isolated as it
%is within $P \setminus L$, while the attacker is also aware of the maximum and
%minimum subset of nodes she might have in fact isolated. %which correspond to %$P \setminus L$ and $P \setminus L \setminus U$, respectively.

We now describe how the algorithms work. Algorithm~\ref{alg:attack_algorithm}
starts by initializing $L$ and $U$ to $\varnothing$. For every received packet,
the algorithm first decides whether the packet belongs to a connection internal
to $P \setminus L$ or to one between a node in $P \setminus L$ and an external
node based on the source IP address. If the source IP is in $P \setminus L$, the packet belongs to an
internal connection and it is given to Algorithm~\ref{alg:leakage_algorithm}
to investigate if the corresponding node acts as a leakage point  (Algorithm~\ref{alg:attack_algorithm},
Line~\ref{line:detect_leakage}). Otherwise, the packet belongs to a connection that crosses the
partition and is dropped (Algorithm~\ref{alg:attack_algorithm},
Line~\ref{line:drop-visible}).

Given a packet originated from $P \setminus L$,
Algorithm~\ref{alg:leakage_algorithm} checks whether the sender of the packet
is advertising information from outside of $P \setminus L$. Particularly, the
attacker checks whether the packet contains an \textsf{INV} message with the
hash of a block mined outside of $P \setminus L$ (or the block itself). If it
does so, the sender must have a path of stealth connections to a node outside of $P
\setminus L$ from which the block was transmitted. Thus the sender is a leakage
point and is added to $L$ (Algorithm~\ref{alg:leakage_algorithm},
Line~\ref{line:leakage_detection}). The actual packet is also dropped to
prevent this information from spreading.

To detect whether a node in $P \setminus L$ is a leakage point, an attacker
should be able to intercept at least one of that node's connections.
Specifically, the node should have a vulnerable connection to another node
within $P \setminus L$, so that the attacker can monitor the blocks it
advertises. To keep track of the nodes that the attacker cannot monitor,
Algorithm~\ref{alg:attack_algorithm} maintains a set $U$ which contains the
nodes she has not received any packets from for a predefined time threshold.
(Algorithm~\ref{alg:attack_algorithm}, Line~\ref{line:removal_inactive}).
Whenever one of these nodes manages to a establish a connection that the
attacker intercepts, it is removed from $U$ (Algorithm~\ref{alg:attack_algorithm}, Line~\ref{line:add_inactive}).

\myitem{Example:} We now show how the algorithms work on the example of Fig.~\ref{fig:intraAS} in which the attacker, AS8, aims to isolate $P=\{A,B,C\}$. By hijacking the prefixes corresponding to these nodes, the attacker intercepts the connections $(B,C)$ and $(A,C)$ and feeds the relevant packets to the algorithms. Recall that the partition is bridged by a stealth (intra-AS) connection between nodes $A$ and $X$ which cannot be intercepted by the attacker. When a block outside $P$ is mined, node $X$ will inform $A$ which then will advertise the block to $C$. The attacker will catch this advertisement and will conclude that node $A$ is a leakage point. After that, the attacker will drop the packet and will add $A$ to $L$. As such, all future packets from $A$ to other nodes within $P \setminus L =\{A,B\} $ will be dropped. Observe that the partition isolating $P \setminus L=\{B,C\}$ is indeed the maximum  feasible subset of $P$.

\remove{In Fig.~\ref{fig:intrapool}, the attacker, AS8, aims at isolating
$P=\{A,B,C,D\}$. The partition is bridged by a stealth (intra-pool) connection between nodes $A$ and $E$ which belong to the green pool. If the green pool learns about a block mined outside $P\setminus L$ by one of its gateways, namely node $F$, the pool will inform its other gateway, node $A$ about it. Node $A$ will then advertise this block to $D$. The attacker will catch this advertisement and will conclude that node $A$ is a leakage point. In this case, the attacker will again remove node $A$ from $P'$ and will be left with $P'=\{B,C,D\}$, which is again feasible.
}

\subsection{Correctness of the partitioning algorithm}
\label{ssec:proof}

We now prove the properties of Algorithm~\ref{alg:attack_algorithm}.

\begin{theorem}
Given $P$, a set of nodes to disconnect from the Bitcoin network, there exists a unique maximal subset $I\subseteq P$ that can be isolated. Given the assumption that Bitcoin nodes advertise blocks that they receive to all their peers,
Algorithm~\ref{alg:attack_algorithm} isolates all nodes in $I$, and maintains a set $P' = P\setminus \{U\cup L\}\subseteq I$ that contains all nodes in $I$ that have a monitored connection and are thus known to be isolated. 
\end{theorem}

\begin{proof}
	Consider the set of nodes $\mathcal{S}\subseteq P$ that has a path of stealth connections to some nodes not in $P$. 
	Clearly, nodes in $\mathcal{S}$ cannot be isolated from the rest of the network by the attacker. 
	Let $I = P\setminus \mathcal{S}$. Notice that $I$ is the maximal set in $P$ that can be disconnected by an attacker. 
	Now, notice that every node in $S$ is placed in sets $L$ or $U$ by the algorithm: 
	if the node has a monitored connection and is caught advertising external blocks it is placed in $L$ (Algorithm~\ref{alg:leakage_algorithm} Line~\ref{line:leakage_detection}).
	If it is not monitored then it is placed in $U$ (Algorithm~\ref{alg:attack_algorithm}, Line~\ref{line:removal_inactive}).
	
	Notice also that the entire set $I$ is isolated from the network. If some node has no stealth connection outside, and was removed solely for the lack of monitoring, it is still having all its packets from outside of $P \setminus L$ dropped -- Algorithm~\ref{alg:attack_algorithm} Line~\ref{line:drop-visible}).  

\end{proof}


\remove{
\begin{proof}
The proof is by contradiction. Suppose that there is a node $n$ in $P'$ which
learns about at least one block $X$ mined outside of $P'$. Let $n'$ be the first node
in $P'$ which learned about $X$ with possibly, $n = n'$. For $n'$ to learn $X$, it means that there must exist an edge $(n', m)$ such that $m \not\in P'$. There two cases to consider.

\begin{case}
	\textup{$(n', m)$ is vulnerable by the attacker. This leads to a contradiction as the attacker would drop $(n', m)$, preventing $n'$ from learning $X$ (see Algorithm~\ref{alg:attack_algorithm}, Line~\ref{line:drop-visible}).}
\end{case}

\begin{case}
	\textup{$(n', m)$ is not intercepted by the attacker. As $n' \in P'$, there must be at least one intercepted edge $(n', a)$ where $a \in P'$, as otherwise $n'$ would be considered as inactive and removed (see Algorithm~\ref{alg:attack_algorithm}, Line~\ref{line:removal_inactive}). By assumption, $n'$ advertises $X$ to $a$ via $(n',a)$. Since $(n',a)$ is intercepted, it implies that $n'$ is detected as leakage point and removed from $P'$ (see Algorithm~\ref{alg:leakage_algorithm}, Line~\ref{line:leakage_detection}). Therefore, we have that $n' \not\in P'$ which also leads to a contradiction.}
\end{case}
\end{proof}


\begin{theorem}
Given $P$, a set of nodes to disconnect from the Bitcoin network, Algorithm~\ref{alg:attack_algorithm} will find the maximum subset $P$ of nodes that can be guaranteed to be isolated by a AS-level adversary.
\end{theorem}
\begin{proof}
To prove that $P'$ is the maximum subset of $P$ that the attacker can be sure that is isolated from the rest of the network, we will prove that for all the nodes that were removed from $P$ the attacker could either not prevent them from being informed about a block that was mined outside $P$ or could not detect if they were informed. For every node $a \in P \wedge a \not\in P'$, namely for every node a removed from $P$, there two cases to consider.

                   

\begin{case2}
	\textup{node a has no connection the attacker can monitor} This means that node a either has  no Bitcoin connections or has only connections to nodes whithin the AS it is hosted in. As such the attacker cannot guarantee that node a has no information about blocks mined outside $P$. Thus, node a should not be considered isolated.
\end{case2}
\begin{case2}
	\textup{node a was caught adverting a block mined outside $P$} There might be a node $b$ which transmitted the block to node a. This transmission must have been made via a stealth connection $(a,b)$ otherwise the connection would have been cut (Algorithm~\ref{alg:leakage_algorithm}, Line \ref{line:drop_block}). We have again two cases here:
	\begin{case3}
\textup{ $b \not\in P$} The peer that transmitted the block to node a is not in P Node a has a stealth connection to a node outside $P$. The attacker cannot cut this connection, node a will always learn new mined blocks, node a should thus be removed.
\end{case3}

\begin{case3}
\textup{ $b \in P$} The peer that transmitted the block to node a is in P, node a has a connection to a node b that has a direct connection of a path to a node outside $P$. All nodes 
in the path included node a will always learn about blocks mined outside $P$ and should thus all be removed.
\end{case3}


\end{case2}

\end{proof}
}
\remove{
\subsection{Limitations}
\myitem P' ming not be the maximal feasible subset of P.
Due to its heuristic nature our algorithm does not guarantees that the P' is is the largest subset of P that is possible. This is only true if we assume that all peers of a node A advertised a block to each peers within small intervals in comparison with the time it takes for the block to be delievred to one of them. 
In more detail if node a has two 

\myitem{Attack time is in fact constrained}
Although the algorithm will indeed manage to find a feasible partition P' that is close to the initial P the time this procedure will take is indeed critical for the impact of the attack. Recall that hijacks are visible attacks, as such the adversary will only have a few hours to complete her attack. As such if she built a large partition completely with no intuition of the structure it quite likely that she will waste most of her attack time in creating the partition. 
}
\remove{

\myitem{Gathering information on the Bitcoin topology and mining pools.} 

To infer the IPs of all Bitcoin nodes such a list can be downloaded from public
sites such as~\cite{bitnodes}. \laurent{NATed nodes?}
\laurent{The following is a bit handwavy. Can we do anything more specific?}
With regards to the gateways, the attacker can use the techniques described in
\cite{coinscope} and leverage her ability to inspect the traffic of almost
every node via hijacking. First, the attacker may hijack the pool's stratum
servers to discover connections that they establish and thus reveal the
gateways they connect to. Connections formed between the pool's stratum server
and its gateways are via Bitcoind's RPC access, and can be easily
distinguished. Second, the attacker can hijack the relay network to discover
connections used by the large mining pools. The relay network has a public set
of six IPs that pools connect to. By hijacking these, one may learn very
critical points of the pool's infrastructure. Specifically, it will not be hard
to identify a pool by observing the blocks it publishes to the relay network.

%To perform a partition attack, the adversary needs to have a view of the topology. Particularly, he needs to have a list of the IPs of the Bitcoin nodes as well as the IPs of the gateways of pools. 
%of the The more accurate this information, the better chance there is to create a complete partition with few if any iteration in the attack loop.   of his prospective victims. If he wishes to perform a network-level attack, he needs to have a view over all the Bitcoin nodes as well as the pool's gateways. If he wishes to perform a more targeted attack he should at least know the IPs of his victim nodes or the gateways of the victim pools. Even an incomplete list of Bitcoin nodes' IP downloaded from public sites such as \cite{bitnodes} offers adequate topology information to launch certain attacks such as disconnect a set of nodes from the rest of the network. However, more sophisticated objectives such as isolating a pool require more information such as the gateways of the pool that are not included in the public available data. 

\myitem{Effective vs ineftive} In order to be effective, a partition
must be complete meaning the attacker must be able to effectively cut all
connections crossing the partition.


Yet, sometimes, there can be nodes belonging to different components that are
connected via channels the attacker cannot intercept. In that case, the
partition is simply not possible.

We distinguish three types of connections the attacker cannot intercept: \emph{(i)} intra-AS;  \emph{(ii)} intra-pool; and \emph{(iii)} pool-to-pool. For each type we explain why a network attacker cannot intercept them and how he can plan the partition to prevent such connections from leaking information from one component to the other.

% In essence: put all the nodes beloning to one AS on one side of the partition...
\myitem{intra-AS} The attacker cannot intercept connection within the same AS, because their traffic is local and will thus not leave the AS. Note that only 1.14\% on average of the possible connections a bitcoin client can do is intra AS (number calculated based on the topology we inferred in Section ~\ref{sec:topology}).


\myitem{intra-pool} The attacker cannot intercept connection among nodes that belong to the same pool. Since mining pools are multi-homed and distributed among different locations, their gateways might be hosted in different ASes, which can of course be included in different components. If that happens, the pool they belong to would get information from both components and probably disseminate this information from one component to the other, effectively acting as a bridge between them.

Intuitively, the attacker would need to include all gateways of a pool in the
same component to address this issue. Thus, if the attacker is aware of all the
gateways of a pool, he can easily avoid this indecent. If the attacker only
knows some of the gateways or none at all, he will have to sacrifice some time
of the attack iterating between the planning and in the monitoring phase to
learn the gateways and adapt the partition accordingly.
}


\remove{
For example in Figure \maria{FILLME} if AS1 is placed in one component and AS2 in the other then the green pool will get information from both components. The green pool then can instruct its gateways nodes E and D to propagate the learned information from E to D and from C to B. In this case, although there is no Bitcoin connection crossing the partition the two components will still be connected. 

\myitem{Pool to Pool} 
The attacker cannot intercept connection among pools that are directly connected to each other with protocols other than Bitcoin. Such a mesh connecting many large pools today is the Bitcoin relays. 
Since the IPs of the relays are publicly available and the BGPsec is not used the attacker can hijack the relays and easily disconnect them. Note that this is different from a DoS attack directed to the IPs of relays, which can be easily mitigated.
If pools have secret agreements to each other then they should be both placed in the same component. Although, that is difficult to know before the actual attack, the attacker can still perform the attack by iterating between the monitoring and planning phase to adapt the partition.
}

\remove{
The goal of execution phase is to enforce the partition that was decided during the planning phase. Particularly, the attacker cuts all connections from one component to the other. The execution phase is composed of two steps which we explain in this subsection: \emph{(i)}  attacker hijack specific prefixes; and \emph{(i)} he cuts the appropriate connections. We refer to nodes whose prefixes are hijacked as hijacked nodes, the component they belong to as hijacked component and the ASes these nodes are hosted in as hijacked ASes. 

\myitem{Hijack}
The attacker hijacks the prefixes pertaining to the nodes of one of the components. The two criteria based on which the attacker chooses which prefixes to hijack are visibility of the attack and diverted traffic load. Particularly, the attacker might try to decrease the prefixes he hijacks to make his attack less visible. For that reason he might choose to hijack the component that requires the least prefixes. On the other hand though, the attacker might choose to advertise all the /24 sub-prefixes that correspond to this component, instead of the initial prefixes which would be more likely fewer, in order to decrease the diverted load.  

 In any case, the attacker does not act as a black-hole but instead keeps a path to the hijacked destination to forward the none Bitcoin traffic as well as the Bitcoin traffic he does not want to drop. As explained in \cite{} this is always possible. 

\myitem{Disconnect}
 The attacker will receive the traffic that is destined to the nodes whose prefixes he hijacked. At this point, he distinguishes the Bitcoin traffic from the regular and investigate it further before sending it to the actual destination. From this traffic the attacker can discover all the connections the hijacked nodes have. He then classifies the connections each hijacked node has as one of three types: \emph{(i)} connections to peers hosted in hijacked prefixes; \emph{(ii)} connections to peers hosted in hijacked ASes but whose prefixes are not yet hijacked; \emph{(iii)}connections to peers hosted in hijacked ASes that are not hijacked. The attacker treats the connections  differently based on their type.
The first type of connections are entirely within the hijacked component and are thus allowed by the attacker. With regards to the second type, the existence of a peer hosted within the hijacked ASes, but whose prefix is not hijacked denotes that the attacker was unaware of this node. Since the attacker needs to include all nodes of an AS within the same component, the attacker would have to hijack the prefix of the previously unknown node as well. After that the attacker allows the connection as it belongs to the first type. 
The third type of connections are connections that cross the partition. The attacker would drop such connections. For each of those connections that the hijacked nodes had initialized, they will try to establish a new connection to replace the dropped one. The attacker will again classify and treat the new connection as described above.
}

\remove{
\subsection{Phase \#3: Monitoring}
In this phase the attacker's goal is to ensure that the formed cut is complete by detecting leakage, identifying its cause and adapt the partition accordingly.
 Leakage can occur due to the incomplete topology the attacker used during the planning phase or even due to the dynamic nature of the Bitcoin network. Thus, the attacker should continually monitor the diverted traffic to detect leakage and react to it. In the following, we describe how an attacker can detect leakage, prevent it from spreading across the component and adapting the partition accordingly.

\myitem{Detect Leakage} To detect leakage the attacker uses the following simple observation. If there is a node within the hijacked nodes that is connected to the other component, it will learn about blocks that are mined in the other component. To propagate these blocks to nodes within the hijacked component it will first send an inventory message with the block's hash to a node in the component. As the attacker sees all traffic to the hijacked nodes and the hijacked nodes are only connected to nodes within the hijacked component, he sees all exchanged traffic/information within that component. Once the attacker sees the hash being advertise by a hijacked node, he concludes that this node has a connections to the other component. To avoid leakage of information from this node to rest of the hijacked component the attacker cuts all its connections to the other hijacked nodes. If the node never tries to propagate the block, it will indeed never be detected, but it will also never cause leakage, in which case it is not a threat for the partition. There is also the chance that the node also has connections that the attacker cannot intercept within the hijacked component, cutting its Bitcoin connections to hijacked nodes might not be enough to stop the leakage. In this case the nodes it is connected to will be also detected as points of leakage and excluded from the hijacked component. 

\myitem{Adapt partition} If there is a node which was included to the hijack component but has a connection to the other component that the attacker cannot intercept, then the initial topology the attacker used while planning is faulty. The attacker should update his topology and revisit the planning phase to adapt the partition so that this node is not included in hijacked component.   
}


\remove{
In this section we detail the three phases involved in a partition attack,
namely the \emph{planning}, \emph{execution} and \emph{monitoring} phases
(Fig.~\ref{fig:overview_partition}).
}

\remove{
The attacker creates a partition plan which is just 3 sets the union of which is set of all nodes and their intersection is null. This represeltation of the attacker's goals together with his view of the Bitcoin topology are used as input for the attacker to decide weather his objectives can be fulfill 

accurately calculating the nodes that would be in . In the following phase, Planning, the decides whether his objectives can be fulfilled or not. 

The first two sets contain the nodes the attacker wishes to disconnect, while the last set contains d can be placed in any of the two components. Given these sets together with some information of the topology the attacker can calculate the actual a partition 
 The attack planer should then try to come up with a partitioning G1, G2 which satisfy attacker's objectives and is possible given the topology. In section  \ref{ssec:rules} we describe which characteristics constitute a partition infeasible for a network attacker. As intuition it is not possible to disconnect a pool by locating some of its gateways to more than one component. If a possible partition is found then the adversary executes the attack by hijacking the prefixes of one of the components and cuts all connections crossing the partition. can be satisfied given the topology. As an intuition, not all partitions are possible. 
}
\remove{
\subsection{Phase \#1: Planning}

In this offline phase, the attacker decides: \emph{(i)} which Bitcoin nodes
will be included in each of the two components of the partition along with the
set of IP prefixes she needs to hijacks to intercept (and kill) any Bitcoin
connection cross the partition. Formally, given an inferred (and not
necessarily perfect) Bitcoin graph $G = (V,E)$, the attacker defines a
partition of the nodes $(V_1, V_2$), such that $V_1 \cup V_2 = V$, $V_1 \cap
V_2 = \varnothing$. The attacker then hijacks all the prefixes pertaining to
nodes in $V_1$ or to the nodes in $V_2$. Given that hijacking prefixes is
visible, we assume that the attacker goes for the attacking the size of the
partition requiring the least amount of prefixes.

Observe that the attacker only needs to know about the Bitcoin nodes
themselves, not the connections they establish. This is because by hijacking
one side of the partition, the attacker automatically sees \emph{all}
connections destined to that side of the partition. Also, $V$ does not have to
be perfectly equivalent to the real (and unknown) Bitcoin topology for the
attack to work. While imperfect $V$ might result in incomplete (and therefore
ineffective) partition, an attacker can detect these leakages and dynamically
adapt its view of $G$. Yet, the closer $G$ is initially from the real topology,
the faster the attacker will be in cutting the graph.

In practice, the content of the partition $(G_1, G_2)$ will depend on the
attacker's objectives. For instance, to perform targeted double spend attacks
against a specific set of merchants, it is sufficient to spread the merchants
across the partitions and inject conflicting transaction. Alternatively, an
attacker might want try to isolate 50\% of the mining power in one component,
causing the two parts of the topology to create their own blockchain.
Obviously, performing larger partitions is more visible and require more
resources than performing small ones. Specifically, larger partitions require
to hijack more prefixes and therefore to process more diverted traffic.

While the cost of performing a partition changes with its size, the modus
operandi of the attack does not. As such, we focus in the rest of the section
on how a given $(G_1, G_2)$ can be realized and explore the notion of cost at
length in Section~\ref{}. We first explain how an attacker can infer the
required topological information. We then describe how the attacker can detect
``leakages'' in the partition and work around them.
}

\remove{
\myitem{Objectives.} 
%Each potential attacker has some intuition of what the partition he wants to
%create looks like. This depends on the impact he wants his attack to have. 
We distinguish between two cases depending on whether the attacker wants to
target specific victims or the cryptocurrency in general. In both cases, there
might be many partitions that satisfy the objectives or none at all.

If the adversary wants to attack specific entities of the Bitcoin network
(nodes or pools), he knows which entities he wants to disconnect. For example,
if he wants to perform a double spend attack the adversary needs to make sure
that the two sellers receiving the same Bitcoins do not see both transactions.
This can only be achieved if each of them is in a different component of the
partition. Similarly, if the attacker wants to attack a pool he needs to make
sure that this pool is not informed about the latest blocks and thus wastes its
mining power on an obsolete chain. To do that the attacker needs to include
this pool within the component which contain less mining power.

Alternative, if the attacker wants to harm the Bitcoin system in general, he knows the property that should hold in the partition. For example, an attacker might try to split the mining power to half, causing the two parts of the topology to create their own blockchain. In this case the property that should hold that the mining power in each component should be close to 50\%.
 `%Since one of the chains would be deleted at the end, such an attack would cause serious revenue loss and increase the risk of double spending attacks and harm Bitcoin's reputation. 
 Similarly, an attacker might try to perform a denial of service attack against as many nodes as possible. Deprived of their ability to trade with Bitcoin for a considerable amount of time (couple of hours), sellers and consumers might switch to other cryptographies. In this case the property that should hold that the mining power should be disconnected from regular clients.
}



==> sp copy/partition_results.tex <==
\section{Partitioning Bitcoin: Evaluation}
\label{sec:eval_partition}

In this section, we evaluate the practicality and effectiveness of partitioning
attacks by considering four different aspects of the attack. \emph{First}, we show that
diverting Bitcoin traffic using BGP hijacks works in practice by performing
an actual hijack targeting our own Bitcoin nodes (Section~\ref{ssec:hijackExp}). \emph{Second}, we show that
hijacking fewer than 100 prefixes is enough to isolate a large
amount of the mining power due to Bitcoin's centralization (Section~\ref{ssec:nb_prefixes_hijack}). \emph{Third}, we show
that much larger hijacks already happen in the Internet today, some already
diverting Bitcoin traffic (Section~\ref{ssec:hijack_real}). \emph{Fourth}, we show that Bitcoin quickly recovers
from a partition attack once it has stopped (Section~\ref{ssec:methodology_experiment}).

\subsection{How long does it take to divert traffic with a hijack?}
\label{ssec:hijackExp}

We hijacked and isolated our own Bitcoin nodes which were connected to the
live network via our own public IP prefixes. In the following, we
describe our methodology as well as our findings with regard to the time it
takes for a partition to be established.

\myitem{Methodology} We built our own virtual AS with full BGP connectivity
using Transit Portal (TP)~\cite{peering}. TP provides virtual ASes with BGP
connectivity to the rest of the Internet by proxying their BGP announcements
via multiple worldwide deployments, essentially acting as a multi-homed provider to 
the virtual AS. In our experiment, we used the \texttt{Amsterdam} TP deployment as
provider and advertised 184.164.232.0/22 to it. Our virtual AS hosted six bitcoin 
nodes (v/Satoshi:0.13.0/). Each node had a public IP in 184.164.232.0/22 (.1 to .6 addresses)
 and could therefore accept connections from any other Bitcoin node in the Internet.

\remove{
traffic destined to IP addresses within that range will be routed first to the
Amsterdam01 TP, and then sent to our machines via the corresponding tunnel.
}

We performed a partition attack against our 6 nodes using BGP hijacking. For
this, we used \texttt{Cornell}, another TP deployment, as the malicious AS.
Specifically, we advertised the prefix 184.164.235.0/24 via the
\texttt{Cornell} TP. This advertisement is a more-specific prefix with respect
to the announcement coming from the \texttt{Amsterdam} TP and covers
all the IPs of our nodes. Thus, after the new prefix announcement is propagated
throughout the Internet, Bitcoin traffic directed to any of our nodes will
transit via \texttt{Cornell} instead of \texttt{Amsterdam}. To mimic an
interception attack (Section~\ref{sec:background}), we configured the
\texttt{Cornell} TP to forward traffic back to our AS. As such,
connections to our nodes stayed up during the hijack even though they
experienced a higher delay.

We performed the attacks 30 times and measured the time elapsed
from announcement of the most specific prefix until all traffic towards our
nodes was sent via the \texttt{Cornell} TP.

\begin{figure}[t]
 \centering
 \includegraphics[width=.6\columnwidth]{figures/hijack}
 \caption{Intercepting Bitcoin traffic using BGP hijack is fast and effective: all the traffic was flowing through the attacker within 90 seconds. Results computed while performing an \emph{actual} BGP hijack against our own Bitcoin nodes.}
 \label{fig:hijack}
\end{figure}

\myitem{Diverting Bitcoin traffic via BGP is fast (takes <2 minutes)} The
results of our experiment are shown in Fig.~\ref{fig:hijack}. The main insight
is that the attacker received the hijacked traffic very quickly. After only 20 seconds, more than 50\% of the connections are diverted. Within 1.5 minutes, all traffic was transiting via the malicious AS. Thus, attacked nodes are effectively isolated almost as soon as the hijack starts.
%, while it will take couple of hours for the hijack to be resolved even after detection.
%This constitutes an indication of the time it will take for the partition to be created.

We took great care to ensure that our experiments did not negatively impact the actual Bitcoin
network. We discuss the ethical considerations behind our experiments in
Appendix~\ref{sssec:ethic}.

\remove{More importantly this number should be compared to the time it will take to stop the attacker by disconnecting the attacker from the Internet which will take at least a couple of hours.}  

\remove{
\myitem{Practicality} 
Such an attack can be performed against the vast majority of the Bitcoin nodes in the current network. Particularly, to perform a partition attack the adversary needs to intercept all traffic from hijacked set to the rest of the network.  nodes are those which are hosted in AS with gateways as well as in ASes with nodes which use /24. That is because if we assume that a potential victim connects to a node in the same AS but which use /24 or is a gateway then the attacker will not intercept this traffic. Even if we consider these nodes safe 61\% of nodes are still vulnerable. Particularly, 92\% use a /24 prefix, 82.6\% have no /24 in their AS and 76\% have no gateway in their AS. It is very important to note here that the rest 40\% is also vulnerable to be affected by a partition attack. The difference is that for these nodes can be placed in any of the two components.
}


%\maria{no pool in their AS 76.367086424\ no \/24 in their AS  82.6116957047 no \/24 and no pool in their AS  60.841814731}

\subsection{How many prefixes must be hijacked to isolate mining power?}
\label{ssec:nb_prefixes_hijack}

Having shown that hijacking prefixes is an efficient way to divert Bitcoin
traffic, we now study the practicality of isolating a specific set of nodes $P$.
%holding an increasing amount of mining power. 
We focus on isolating sets holding
mining power because they are: \emph{(i)} more challenging to perform (as
mining pools tend to be multi-homed); and \emph{(ii)} more disruptive as
successfully partitioning mining power can lead to the creation of parallel
branches in the blockchain.

To that end, we first
estimate the number of prefixes the attacker needs to hijack to isolate a specific set of nodes as a function of the mining power they hold. In the following subsection, we evaluate how practical
a hijack of that many prefixes is with respect to the hijacks that frequently take place in the Internet. %We describe the sets we consider before we present our results.

\remove{we evaluate how practical
is a hijack of that many prefixes with respect to the hijacks that frequently take place in the Internet. }

\myitem{Methodology} As described in Section~\ref{sec:partition}, not all sets
of nodes can be isolated as some connections cannot be intercepted. We
therefore only determine the number of prefixes required to isolate sets $P$ that are
feasible in the topology we inferred in Section~\ref{sec:topology}. In
particular, we only consider the sets of nodes that contain: \emph{(i)} either
all nodes of an AS or none of them; and \emph{(ii)} either the entire mining pool, namely all of its 
gateways or none of them. With these restrictions, we essentially avoid the possibility of having any leakage point within $P$, that is caused by an intra-AS or intra-pool stealth connection. 
%Even in the case that 
%nodes within each AS form a connected component of stealth connections (which is
%unlikely in practice) and all gateways of each pools are connected internally  via proprietary, %encrypted protocols.
However, we cannot account for secret peering agreements that may or may not exist between pools. Such agreements are inherently kept private and their existence is difficult to ascertain. 





\remove{
6\%\-94\% && 2 && 86.0 && 20\\
7\%\-93\% && 7 && 72.0 && 23\\
8\%\-92\% && 32 && 69.5 && 14\\
30\%\-70\% && 83 && 83.0 && 1\\
39\%\-61\% && 32 && 51.0 && 11\\
40\%\-60\% && 37 && 80.0 && 8\\
41\%\-59\% && 44 && 55.0 && 3\\
45\%\-55\% && 34 && 41.0 && 5\\
46\%\-54\% && 78 && 78.0 && 1\\
47\%\-53\% && 39 && 39.0 && 1\\
}


\begin{table}[t]
\centering
\small
\def\arraystretch{1.1}
\setlength{\tabcolsep}{7.5pt}
%\begin{tabular}{@{}lclclclclclc@{}}
\begin{tabular}{l l l l}
\toprule
%Attack & Active(How much) & Passive(Who can) &  \% ForkRate & Implications\\
%\emph{Partition}&\multicolumn{2}{c}{\emph{\# Prefixes}}&\emph{\# Feasible partitions}   \\
%&\emph{Minimum}&\emph{Median}&   \\
%\emph{Partition}&\emph{Min \#Prefixes}&\emph{Med \#Prefixes}&\emph{\#Feasible Partitions}   \\
\begin{tabular}{@{}l@{}} \emph{Isolated} \\ \emph{mining power}\end{tabular} & \begin{tabular}{@{}l@{}} \emph{min. \# pfxes} \\ \emph{to hijack} \end{tabular} & \begin{tabular}{@{}l@{}} \emph{median \# pfxes} \\ \emph{to hijack}\end{tabular} & \begin{tabular}{@{}l@{}} \emph{\# feasible} \\ \emph{partitions}\end{tabular}   \\

\midrule
8\%\ & 32 & 70 & 14\\
30\%\ & 83 & 83 & 1\\
40\%\ & 37 & 80 & 8\\
47\%\ & 39 & 39 & 1\\
\bottomrule
\end{tabular}
\caption{Hijacking <100 prefixes is enough to feasibly partition {\raise.17ex\hbox{$\scriptstyle\sim$}}50\% of the mining power. Complete table in Appendix~\ref{ssec:partitions}.}
\label{tab:partition_costs}
\end{table}


\remove{ 
\myitem{Hijacking <100 prefixes is enough to isolate {\raise.17ex\hbox{$\scriptstyle\sim$}}50\% of Bitcoin mining power}
As described in Section~\ref{sec:partition}, not all sets of nodes can be
isolated as some connections cannot be intercepted. We therefore evaluate the
number of prefixes required to isolate sets $P$ that are feasible in the
topology we inferred in Section~\ref{sec:topology}. In particular, we only
consider the sets of nodes that contain: \emph{(i)} either all nodes of an AS
or none of them; and \emph{(ii)} either all gateways of a mining pool or none
of them. These restrictions restricts the values of the isolated mining power
to few discrete values (since not all partitions can be realized). Moreover,
some pairs of pools cannot be disconnected as they have gateways within the
same AS.

Particularly, an attacker can isolate a set of nodes $P$, if there are no stealth connections from nodes inside $P$ to nodes outside it. We explained in Section~\ref{sec:partition} how the attacker can prevent such connections from bridging the isolated set to the rest of the network by monitoring the connections she hijacks.
For the purpose of off-line estimating the number of required prefix hijacks though,\maria{with off-line I mean for estimating-inferring the number that would be needed as opposed to performing the attack and decide on the fly}
}

\myitem{Hijacking <100 prefixes is enough to isolate {\raise.17ex\hbox{$\scriptstyle\sim$}}50\% of Bitcoin mining power}
In Table~\ref{tab:partition_costs} we show the number of different feasible sets of nodes we found containing the same amount of mining power (4th and 1st column, respectively). We also include the minimum and median number of the prefixes the attacker would need to hijack to isolate each portion of mining power (2nd and 3rd column, respectively).
\remove{ Our results are summarized in Table I. The leftmost column describes the portion of mining power contained in the isolated set of nodes. We indicate the number of feasible sets containing the same amount of mining power along with the minimum and median amount of prefixes to hijack to create the partitions in practice.
}

As predicted by the centralization of the Bitcoin network
(Section~\ref{sec:topology}), the number of prefixes an attacker needs to hijack to create a
feasible partition is small: hijacking less than 100 prefixes is enough to
isolate up to 47\% of the mining power. As we will describe next, hijack events
involving similar numbers of prefixes happen regularly in the Internet. Notice
that the number of prefixes is not proportional to the isolated mining power.
For example, there is a set of nodes representing 47\% of mining power that can
be isolated by hijacking 39 prefixes, while isolating 30\% of the mining power belonging to different pools would require 83 prefixes. Indeed, an attacker can isolate additional mining power
with the same number of hijacked prefixes when several pools
in the isolated set are hosted in the same ASes.

\remove{
While our results are inherently dependent on the accuracy of our inferred
topology (Section~\ref{sec:topology}), we stress that attackers may slowly gain
better information, e.g., through repeated stealthy hijacks of the target. \maria{I don't understand that}
}

\begin{figure}[t]
	\centering
	\begin{subfigure}[t]{0.47\columnwidth}
		\includegraphics[width=\columnwidth]{figures/nb_hijacks_per_month}
		\caption{Each month sees \emph{at least} 100{,}000 hijacks, some of which involve \emph{thousands} of prefixes.}
		\label{fig:hijack_number}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.47\columnwidth} 	\includegraphics[width=\columnwidth]{figures/impacted_nodes_per_month}
		\caption{Each month, traffic for at least 100 \emph{distinct} Bitcoin nodes end up diverted by hijacks.}
		\label{fig:hijack_size}
	\end{subfigure}
	\caption{Routing manipulation (BGP hijacks) are prevalent today and do impact Bitcoin traffic.}
	\label{fig:hijack_analysis}
\end{figure}

\vfill
\subsection{How many hijacks happen today? Do they impact Bitcoin?}
\label{ssec:hijack_real}

Having an estimate of the number of prefixes that need to be hijacked to partition the entire network, we now look at how common such hijacks
are over a 6-months window, from October 2015 to March 2016. We show that BGP
hijacks are not only prevalent, but also end up diverting Bitcoin traffic.

\newpage
\noindent\textbf{Methodology} We detected BGP hijacks by processing \emph{4 billion} BGP
updates advertised during this period on 182 BGP sessions maintained by 3 RIPE
BGP collectors~\cite{ripe:ris} (rrc00, rrc01 and rrc03). We consider an update
for a prefix $p$ as a hijack if the origin AS differs from the origin AS
seen during the previous month. To avoid false positives, we do not consider
prefixes which have seen multiple origin ASes during the previous month. We
count only a single hijack per prefix and origin pair each day: if AS $X$
hijacks the prefix $p$ twice in one day, we consider both as part of a single
hijack.

\myitem{Large BGP hijacks are frequent in today's Internet, and already end up
diverting Bitcoin traffic}
Fig.~\ref{fig:hijack_analysis} summarizes our results. We see that there are \emph{hundreds of thousands} of hijack events \emph{each
month} (Fig.~\ref{fig:hijack_number}). While most of these hijacks involve a single IP prefix, large hijacks
involving between 300 and 30,000 prefixes are also seen every month (right axis).
Fig~\ref{fig:hijack_size} depicts the number of Bitcoin nodes for which traffic was diverted in these hijacks. Each month, at least 100 Bitcoin
nodes are victim of hijacks\footnote{The actual hijack attempt may have been aimed at other services in the same IP range, still, these nodes were affected and their traffic was re-routed.}. As an illustration, 447 distinct nodes
({\raise.17ex\hbox{$\scriptstyle\sim$}}7.8\% of the Bitcoin network)
ended up hijacked at least once in November 2015. %While already worrying, 


\remove{
While frequent, BGP hijacks are hard to diagnose and slow to resolve. As BGP
securities extensions (BGPSec~\cite{bgpsec}, RPKI~\cite{rfc6480}) are seldom
deployed~\cite{lychev_bgpsec_deployment}, operators rely on simple monitoring
systems that dynamically analyze and report rogue BGP announcements
(e.g.,~\cite{yan2009bgpmon,chi2008cyclops}). 

In Section~\ref{sec:bitcoin_interception}, we showed that any single AS can
intercept 50\% of the connections (and mining power) by hijacking few prefixes
({\raise.17ex\hbox{$\scriptstyle\sim$}}0.15\% of all prefixes). We now
investigate the influence an attacker might have by simply dropping all
messages on the intercepted connections, effectively partitioning the Bitcoin
network.

To measure the effect of a partition in a large-scale virtualized environment
composed of 1050 actual Bitcoin nodes
(\S\ref{ssec:methodology_experiment}). We describe two key findings. First, the network
quickly goes down after connections are disrupted. Second, while connections
crossing the partition slowly return as the partition heals (\S\ref{sec:partition_results}), the fork rate is quickly restored to normal. The latter result implies that
imperfect partitions are not useful in disrupting the network, which makes
partition attacks last only as long as the attacker successfully isolates the
different parts of the network.
}

\begin{figure}[t]
 \centering
 \includegraphics[width=.65\columnwidth]{figures/res_partition_health}
 \caption{Bitcoin heals slowly after large partition attacks. After 10h, only half as many connections cross the partition. Healing is even slower if the attacker is naturally on-path for 13\%, 18\%, 28\% of the connections.}
 \label{fig:partition_healing}
 \vspace{-.5cm}
\end{figure}

\subsection{How long do the effects of a partition attack last?}
\label{ssec:methodology_experiment}
Having investigated the methodology and the relative cost of creating a
partition, we now explore how quickly the Bitcoin network recovers from a partition attack. We found out that while the two components quickly reconnect, they stay sparsely connected for a very long time. We first describe the
experimental set-up. Next, we explain why partitions are not persistent in
practice and briefly hint on how an attacker could prolong their lifetime.

\myitem{Methodology} We build a testbed composed of 1050 Bitcoin clients
running the default \verb+bitcoind+ core (v0.12.1) in testnet mode. Each node
runs in a virtual machine connected to a virtual switch and is configured with
a different random IP address. Nodes automatically connect to other nodes in the testbed. We enforced a 50\%--50\% partition, by installing
drop rules on the switch which discard any packet belonging to a connection
crossing the partition. Observe that a 50\%--50\% split is the easiest partition to recover from, as
after the attack the chance that a new connection would bridge the two halves is maximal. We measure the partition recovery time by recording
the percentage of connections going from one side to the other in 30 minute intervals.

Bitcoin TCP connections are kept alive for extended periods. As
such, new connections are mostly formed when nodes reconnect or leave the
network (churn). To simulate churn realistically, we collected the lists of all
reachable Bitcoin nodes~\cite{bitnodes}, every 5 minutes, from February 10 to
March 10 2016. For every node $i$ connected in the network on the first day, we
measured $t_i$ as the elapsed time until its first disappearance. To determine
the probability of a node to reboot, we randomly associated every node in our
testbed with a type $t_i$ and assumed this node reboots after a period of time
determined by an exponential distribution with parameter
$\lambda=\frac{1}{t_i}$. The time for next reboot is again drawn according to
the same distribution. This method produces churn with statistics matching
the empirical ones. We repeat each measurement at least 5 times and report the median value found.

\myitem{Bitcoin quickly recovers from a partition attack, yet it takes hours for the network to be densely connected again}
We measured how long it takes for the partition to heal by measuring how
many connections cross it, before, during and after its formation (Fig.~\ref{fig:partition_healing}). We consider
two different attack scenarios: \emph{(i)} the adversary does not intercept any
bitcoin traffic before or after the attack; and \emph{(ii)} the adversary intercepts some connections naturally.

\emph{Case 1: The adversary intercepts no traffic after the attack.} It takes
2 hours until one fifth of the initial number of connections crossing the
partition are established, while after 10 hours only half of the connections
have been re-established. The slow recovery is due
to the fact that nodes on both sides do not actively change their connections
unless they or their neighbors disconnect.

\emph{Case 2: The adversary intercepts some traffic after the attack.} If an
AS-level adversary is naturally on-path for some of the connections, she can
significantly prolong the partition's lifetime. To do so, the attacker would
just continue to drop packets on connections she naturally intercepts. We measured
the effect of such attacks for attackers that are on-path for 14\%, 18\%, and
28\% of the connections, respectively (Fig.~\ref{fig:partition_healing}). We
see that an AS-adversary who is initially on-path for 28\% of the connections
can prolong the already slow recovery of the partition by 58\%. Many other ways to increase the persistence of a partition exist. Due to space constraints, we discuss some of them in Appendix~\ref{ssec:partition_life}.

Despite the long healing time, the orphan rate of the network returned to
normal even with 1\% of all connections crossing the partition. This fact shows
that partitions need to be perfect in order to affect the network significantly.

\remove{
\laurent{I reverted back to the previous structure. I didn't like the useful
conclusions too much which didn't really belong to the evaluation, rather to a
discussion.}
}
\remove{
\myitem{Useful conclusions}
These observations reveal concrete ways for the attacker to make the partition last for longer. The attacker needs to suppress the effect of churn in order to keep the victim nodes isolated. Two observations may help in this regard: 

\emph{(i) A smaller set of nodes will be easier to isolate for extended periods.} 
The smaller the set of nodes is, the more time will pass before any isolated node restarts (which will most likely cause it to attempt to establish links and break the partition). Similarly, if the set of nodes is small,  external nodes will connect to the isolated set with lower probability. 

\emph{(ii) All incoming connection slots can be occupied by connection from attacker nodes.}
Bitcoin nodes typically limit the number of incoming connections they accept. The attacker may use several nodes to aggressively connect to the isolated nodes, and maintain these connections even after BGP routing is restored. Connections initiated by external nodes would then be rejected by the isolated nodes (as all slots of connections remain occupied). This is naturally made easier for the attacker if the set of isolated nodes is small.

\emph{(iii) Outgoing connections can be biased via an eclipse attack~\cite{heilman2015eclipse}.}
Once an isolated node reboots, it will try to establish connections to nodes in its peer lists. These can be biased to contain attacker nodes, other isolated nodes, and IP addresses that do not actually lead to Bitcoin nodes. This is established by aggressively advertising these IPs to the victim nodes. The connections they form upon rebooting will then be biased towards those that maintain the partition.
}

\remove{
With regards to the Bitcoin clients, they should allow the natural churn of the network refresh their connections as that can protect them against partition attacks. A node with disabled incoming connections or even a node that is behind an NAT or a firewall will never receive a random incoming connection from the rest of the network. As such if the node is hijacked for a few minutes and isolated from a part of the network, it will only reconnect to this part when it reboots or when one of its outgoing connections fails. 

}

\remove{


Our min observation is that the connectivity between the two components is quickly re-established but the skewness in the connections remains for long. The Bitcoin protocol itself is responsible for the slow recovery, while the few connections that are establish are due to random events in the network such as new node joining and reboots which are commonly refer to as churn. As such, the healing time of an isolated set of nodes depends on their internal churn as well as their attitude towards the natural churn of the network. For example if a node never reboots and is behind a NAT or a firewall or does not accept incoming connections, the bias until its one of its outgoing connections reboot. On the other hand accepting all incoming connections might be even worse as it allows the attacker to saturate the node’s connections.

}




\remove{The fundamental question we answer in this section is how fast the network recovers from an abrupt change in its connectivity as well as which are the factors that influence this procedure.  Our main finding is that although the protocol it self is extremely slow to recover, the dynamic nature of the peer to peer network causes few connections to be establish 
}
\remove{

We start by giving a high-level view of our experimental set-up and the incorporation of churn. 
Our testbed is composed of 1050 Bitcoin clients running the default \verb+bitcoind+ core (v0.12.1) in testnet mode. Each node runs on a virtual machine connected to a virtual
switch and is configured with a different random IP address. To enforce a given
partition, we simply install drop rules on the switch which discard any packets
belonging to a connection crossing the partition. We measure the partition
recovery time by collecting the percentage of connection going from one side to
the other every 30 minutes.


\myitem{Churn} By design, Bitcoin TCP connections are kept alive for extended periods. As such, new connections are mostly formed when nodes reconnect of leave the network (churn). To simulate churn realistically, we collected the lists of
all reachable Bitcoin nodes~\cite{bitnodes}, every 5 minutes, from February 10 to March 10 2016. For every node $i$ connected in the network on the first day, we measured $t_i$ as the elapsed
time until its first disappearance. To determine the
probability of a node to reboot, we randomly associated every node in our
testbed with a type $t_i$ and assumed this node reboots after a period of time
determined by an exponential distribution with parameter
$\lambda=\frac{1}{t_i}$. The time for next reboot is again drawn 
according to the same distribution. This method produces 
churn with statistics identical to the empirical ones. We
repeat each measurement at least 5 times with
different sequences of reboots and report the median value found.

\myitem{Validation} We ensure the reliability of our results using three
methods. Firstly, we avoid potential interference between consecutive
experiment by rebooting each node before every experiment. Address books for the nodes (peers.dat) were generated through a random process of churn and are restored to their initial state in between different runs. 
%by adding 8 random addresses to each node in the testbed via the API and restarting all of them 2.5 times at random. 
All our nodes thus end up with
{\raise.17ex\hbox{$\scriptstyle\sim$}}800 addresses in their database. \remove{This
number corresponds to almost all the nodes running in our testbed, which allows them to form a well connected network before they are attacked. }
% is compliant with the actual Bitcoin network where nodes know about 6000 IPs.
Secondly, before each experiment, we count and report the number of connection that cross the
partition to ensure that there is no bias in the initialization process in favor of the partition. 

Thirdly, we made sure that the server running our testbed was moderately used during the entire experiment so that our results are not influenced by CPU spikes.



\subsection{Results}
\label{sec:partition_results}
We now measure how long it takes for a 50 partition to heal by measuring how
many connections cross it, before, during and after its formation. We consider
two different attack scenarios: \emph{i)} the adversary does not see any
Bitcoin traffic before or after the attack; and \emph{ii)} the adversary sees
some connections naturally. Fig.~\ref{fig:partition_healing} summarizes our
findings. We stress that our experimental results serve as a generic study of
partition recovery as they are independent of how the partition was formed.

In spite of the slow recovery time, the orphan rate of the network returned to normal even with 1\% of all connections crossing the partition. This fact shows that partitions need to be perfect in order to affect the network significantly. 

\myitem{Case 1: no connection crosses the attacker(s) naturally} As seen in Fig.~\ref{fig:partition_healing}, it takes 2 hours until one fifth of the initial number of connection crossing the partition are established, while after 10 hours only half of the connections has been recovered. The slow recovery is due to the fact that nodes on both sides do not actively change their connections unless they or their neighbors disconnect.

\begin{figure}[htbp]
 \centering
 \includegraphics[width=.80\columnwidth]{figures/res_partition_health}
 \caption{Bitcoin heals slowly after a 50 partition attack. After 10h, only 50\% of the connections which crossed the partition initially cross it again. The healing is even slower if the attacker is on-path for some connections (13\%, 18\%, 28\%) naturally.}
 \label{fig:partition_healing}
\end{figure}



\myitem{Case 2: some connections cross the attacker(s) naturally} If an
AS-level adversary is naturally on-path of some connection, she can
significantly prolong the partitions healing. To do so, the attacker would
just continue dropping packets on connections she is on-path for. We measured the effect of such attacks for attackers that are on-path for 14\%, 18\%, and 28\% of the connections, respectively. The results appear in Fig.~\ref{fig:partition_healing}. We see that an AS-adversary who is initially
on-path for 28\% of the connections can prolong the already slow recovery of the partition by 58\%. 


%l28 3 set(['DE', 'GB', 'US']) l18 5 set(['DE', 'NL', 'GB', 'US', 'SE']) l13 7 set(['RU', 'NL', 'CN', 'DE', 'US', 'GB', 'SE'])
\myitem{To delay the recovery even further} an adversary can pro-actively bias
the connections the nodes will accept and initialize after the attack. Firstly,
she can modify exchanged messages across the partition to cause nodes to ban
each other, prohibiting the re-establishment of the same connections for 24
hours. Secondly, the attacker can flood the nodes in each partition with
addresses of nodes belonging to the same partition~\cite{heilman2015eclipse} or modify the exchanged \textsf{ADDR} messages.
This essentially increase the probability that future connections will be
within the partition.


}



==> sp copy/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

%\laurent{Make sure we cite the NDSS paper and other recent work about BGP security and hijacks}

\myitem{AS-level adversaries} The concept of AS-level adversaries has been
studied before in the context of Tor~\cite{feamster:wpes2004, murdoch:pet2007,
Edman:2009:ATP:1653662.1653708,raptor2015,vanbever2014anonymity}. These works also illustrated the problems caused by centralization and
routing attacks on a distributed system running atop the Internet. Yet, Tor and
Bitcoin differ vastly in their behavior with one routing messages in an
Onion-like fashion, while the other uses \emph{random} connections to flood messages throughout the entire network.
Although random graphs are usually robust to attacks, this paper shows that
it is \emph{not} the case when the network is centralized at the routing-level.

\myitem{Bitcoin attacks} The security of Bitcoin from network-based attacks has
been relatively less explored compared to other attack scenarios. While eclipsing attacks~\cite{heilman2015eclipse,gervais2014bitcoin} have a similar impact than delay attacks when performed against a single node, they disrupt the victim's connections and assume that the attacker is directly connected to the victim (Section~\ref{sec:delay}).
%Gervais \emph{et. al.} consider other aspects of the centralization of Bitcoin and their consequences to the security of the protocol in~\cite{gervais2014bitcoin}. 
For more information about Bitcoin attacks, we refer the reader to a recent comprehensive survey on the Bitcoin protocol~\cite{bonneau2015sok}.
%Some attacks, like the Selfish mining
%attack~\cite{eyal2014majority,DBLP:journals/corr/SapirshteinSZ15} become more
%powerful when the network slows down. A recent paper suggests combining them
%with eclipse attacks in order to amplify the
%effect~\cite{DBLP:journals/iacr/NayakKMS15}. 

\myitem{BGP security issues} Measuring and detecting routing attacks has seen
extensive research, both considering BGP hijacks~\cite{shi:imc12,zhang:conext07,zhang:ton10} and
interception attacks~\cite{ballani:sigcomm07}. Similarly, there has been much
work on proposing secure routing protocols that can prevent the above
attacks~\cite{boldyreva:ccs12,gill:sigcomm11,hu:sigcomm04,oorschot:tissec07}. In
contrast, our work is the first one to show the
\emph{consequences} of these attacks on cryptocurrencies. 

==> sp copy/results.tex <==
\section{Simulation Results}
\label{sec:results}

\subsection{Validation Metrics}
Some of the simulation parameters are slightly modified for the needs of each attack and topology. For that reason  each time we study an attack scenario we will run the same simulation assuming there is  no network adversary. The measured values in the extra run is then compared to the corresponding values when an attack takes place to depict the impact of the attack and to the ground truth, to measure the reliability of each simulation instance.


\textbf {50th Percentile Delay:}  Average time until half of the network is informed about a specific block. A reasonable value for the time window the simulation refers to is (5..8sec) as it is reported in []\\

\textbf {outgoing block rate:} The average number of blocks a full node sends in a given time frame. This number is used to calculate the average outgoing bandwidth (excluding transactions)  per node and compare it with that of  our live nodes .  A reasonable value for the time window the simulation refers to is  (incoming ~ 13KBps, outgoing 65 KBps)

\textbf {incoming inv rate:} The average number of  inventory messages for blocks a full node receives in a given time frame. This number is used to calculate the average incoming bandwidth (excluding transactions) per node and compare it with that of our live nodes   A reasonable value for the time window the simulation refers to is DON’T KNOW YET

\textbf {Orphan rate:} the percentage of blocks that were mined but were not included in the blockchain.  reasonable value for the time window the simulation refers to is  1%-3%

\subsection{Evaluation Metrics }

\textbf {Orphan rate:} the percentage of blocks that were mined but were not included in the blockchain. Each time there is a fork ie two different versions of the main blockchain at least an orphan block is produced The consequences of an higher orphan rate for the currency could be summarized as follows.
1. Bitcoin mining becomes an unprofitable and thus unpopular investment.  The miners that produced the orphan blocks lose the corresponding revenue for their work. 
2. Bitcoin becomes a highly insecure currency. Two blocks of the same height can include conflicting transactions i.e double spends. In this case even a careful merchant that waits at least up to 20 minutes can be deceived. 
3.  Bitcoin becomes unsuitable for quick payments. The computational power, and consequently  the amount of generated blocks are stable. Each block is connected to the previous one so one could imagine that blocks form a tree whose longest path - ( height of the tree) is the Main chain. A higher node degree results in a shorter tree (of the given number of nodes). Equally more forks result in a shorter Main Chain. A shorter Main chain essentially means  lower block generation rate which increases the time it takes for a transaction to be included in a block.\\


\maria{\textbf{@aviv:} Can you descriope Bet over Lamda?}




\textbf {Generated blocks - In-chain Blocks:} This two metrics refer to the number of blocks a specific pool has mined and to the number of blocks she received revenue for. The former is always proportionate to the computational power of the pool. A large relative increase in the latter is interpreted as malicious behavior that was successful for the attackers, while a decrease denotes malicious behavior that resulted loss of revenue for the attacker it self.We will study the corresponding metrics of one specific pool which will also serve as attacker to have a consistent view of the impact the attack has in the network.


Graph1-Passive: Y: number of colluding ISPs, X orphan rate 3 lines Equal distribution, Decentralized Pools ,Centralized pools

Graph2-Passive-Active: Y: number of colluding ISPs, X orphan rate  -3 lines Equal distribution and 100 hijacked prefixes, Decentralized Pools 20 Hijacked Prefixes,Centralized pools, 10 hijacked prefixes Should that be one graph? or many

Graph 3 Passive-Pool :  Y:number of  ISPs that collude , X \% of unfair share gained. For example pool X has 20 \% mining power and she colludes with the ISPs she manage to put 25\% of her blocks in the Blockchain. We will see an increase because the always works on the latest block (The ISPS do not delay packets in her connection). She can follow 2 policies - two lines in the graph. Policy 1 propagate her blocks but not blocks mined by others. Policy 2 Do does selfish mining !!!!! for that we make an extra assumption  that she chooses other pools as her peers.

Graph 4 Passive-Active-Pool :  Y:number of  ISPs that collude , X \% of unfair share gained. 

Graph 2.1 2.2 2.3 2.4   Y:number of  ISPs that collude  :Lamda 



\subsection{Pure Networking Attacks}\laurent{The ``pure'' is ackward}
 
\myitem{Description:} At first we consider pure networking passive attacks, in that a number of AS (0 to 5) collude to attack bitcoin community exclusively by delaying unpreferentially all block messages that are naturally routed through their infrastructure. The aim of the attacker in this case is to destroy the currency by increasing the fork rate.


D0T0T0   23/28\% --> 23/29\%        2\%         100\%            6-11           6-11-7
D1T0T0   19/18\% --> 18/18\%        8\%         0\%             7-2430          7-12-7
D2T0T0   19/17\% --> 15/18\%        28\%        11\%            10-22024        7-12-7
D3T0T0   22/20\% --> 20/32\%        42\%        5\%             1217-23924      7-11-7
D4T0T0   25/27\% --> 23/46\%        47\%        3\%             1219-42965      6-11-6
D5T0T0   21/17\% --> 18/25\%        43\%        17\%            1223-38944      7-12-7

\textbf {Comments:}  If  network level adversaries collude then they can cause 30\% fork rate aka almost one out of three mined blocks are orphans. This percentage raises as more ISPs are added to the attacker's group. It is extremely worrying that only 6 ASes are enough to render most of the generated blocks orphans ie waste most of the computational power that is devoted to Bitcoin. Moreover, the network becomes more unfair as the attackers become more powerful. 50\% percent unfairness means that in half of the block races the node that generated the block first loses the corresponding revenue.


\textbf {Description:}	In this experiment we consider the case of a pool that colludes with ISPs. The ISPs are again  passive attackers, in that they only delay block messages. However in this instance of the simulation the network adverseries do not delay blocks that are destined to or send by the colluding pool. The pool never propagates the blocks which were mined by others. In other words she never uses its propagation advantage for serving the community. In regards to propagating the blocks she mines. she follows three different policies.\\
\textbf {Policy v1:}	The pool propagates the blocks she mines immediately.\\
\textbf {Policy v2:}	The pool performs shellfish mining in that she keeps a private chain of blocks she mined and works on them without propagating them to the network. The aim is to force the rest of the network to work on blocks that are destined to become orphans. Such an attack is successful if the pool manages to create a private longer chain which is then announced to the network, nullifying the work of the benign miners and gaining more revenue than her fair share.In our case (policy v2)  when the pool is on a block race (a block of of height equal to height of a block in the private chain  is propagated in the network), she propagates exactly one block, the one that has the same height as the one that is propagated regardless of the length of the private chain.\\
\textbf {Policy v3:}	The pool performs shellfish mining but propagates 2 blocks from the private chain when a block race occurs if possible (if the private chain contains at least 2 blocks)\\

Policy v1:\\
D0T8T0   26/25\% --> 26/25\%        0\%         0               5-11            6-11-17\\
D1T8T0   22/20\% --> 22/28\%        30\%        3\%             6-17340         7-11-15\\
D2T8T0   20/24\% --> 20/30\%        21\%        0\%             6-19037         8-12-16\\
D3T8T0   21/21\% --> 21/30\%        32\%        7\%             9-39220         7-11-14\\
D4T8T0   29/27\% --> 29/37\%        28\%        3\%             6-39329         7-12-15\\
D5T8T0   21/21\% --> 21/31\%        34\%        4\%             6-41463         7-12-14\\


Policy v3:\\
D0T8T2   21/23\% --> 18/26\%        25\%        13\%            6-12444         6-11-11\\
D1T8T2   23/25\% --> 17/25\%        28\%        28\%            6-33758         6-11-10\\
D2T8T2   22/17\% --> 21/27\%        38\%        2\%             8-30592         7-12-10\\
D3T8T2   29/26\% --> 27/40\%        39\%        5\%             7-37725         6-11-9\\
D4T8T2   24/21\% --> 24/35\%        39\%        0\%             6-35429         7-12-11\\
D5T8T2   19/20\% --> 18/33\%        43\%        9\%             9-37970         6-11-9\\

 When there is  no network adversary and no pool behave malisciously the fork rate is 1\%. When there is a pool that does selfish mining the fork rate increases as one would expect since this is a consequence for the attack. The crucial thing about our results which serves as a validation point is that the selfish pool does not manage to gain more revenue than her fair share despite its behavior when there is no network-level support .?? This is due to the fact that its computational power is beyond the limit of 33\% that is proven to be the minimum for performing a successful selfish mining attack in []:

The level unfairness also increases. I HOPE!!!!




==> sp copy/reviews.tex <==
\section{Previous reviews}

Prior to being submitted to IEEE Security \& Privacy 2017, this paper was
submitted to ACM CCS 2016 (where it was heavily discussed at the TPC meeting,
see highlighted part of Review \#262B below) and at USENIX Security 2016
(preliminary version). We include the reviews verbatim below.

The paper has been \emph{thoroughly} revised since then. We highlight (in 500
words) the improvements made to the paper and how we incorporated the feedback
from the reviewers in Appendix~\ref{appendix:answers}. We also add clickable references to the reviews below pointing to our answers.

\subsection{\textbf{Reviews from ACM CCS 2016}}

%---------------------------------------------------------------------------
\myitem{Review \#262A}
%---------------------------------------------------------------------------

\medskip
\noindent{\emph{Decision:}} 2. Reject (will argue against)

\medskip
\noindent{\emph{Summary:}} This paper studies large-scale network attacks on Bitcoin. It considers AS-level adversaries and traffic interception, routing, and traffic delay attacks.

\medskip
\noindent{\emph{Paper strengths:}} \\
- measurement study of Bitcoin using real world routing data \\
- experiments with partitioning, traffic delays

\medskip
\noindent{\emph{Paper weaknesses:}} Not sure to what extent these findings are about Bitcoin rather than about
Internet in general. I think the results would not change if you would select
6000 random servers on the Internet. So it is more about centralization of
global traffic by ASes and country-wise biases in global usage of Internet \reviewref{ans:bitcoin-specific}.

Another shortcoming is in oversimplified assumptions about miners, and their
network infrastructure. Miners are not simple peers, they are multi-homed, and
major pools form fully connected graph with direct links \reviewref{ans:multi-homing}.

\medskip
\noindent{\emph{Additional comments for authors:}} I think the paper would benefit from a more carefully study of several major mining pools, their topology and connectivity to each other and to the rest of the peers. There are some recent studies of topology of the bitcoin network, this could be a starting point. I think your Section 6 is closer to how such a study might look like \reviewref{ans:multi-homing}.

\medskip
\noindent{\emph{Response to rebuttal:}} I am still not convinced that 15 major pools are connected to the rest of the world by just 30 IPs. This would be prone to easy DoS attacks, and we know that major pools are frequently under DoS attacks and learned to survive them. It should be possible to find the real miner connectivity via methods used by recent topology discovery papers (i.e. make multiple connections to many peers over extended periods of time and discover peers who are the first to relay the blocks) \reviewref{ans:multi-homing}.


%===========================================================================
\myitem{Review \#262B}
%---------------------------------------------------------------------------

%---------------------------------------------------------------------------

\medskip
\noindent{\emph{Decision:}} 5. Accept (will argue for)

\medskip
\noindent{\emph{Summary:}} The authors investigate a number of disruption attacks on the Bitcoin network, which can be conducted by controlled groups of IP addresses (ASes). An attacker exploits the routing BGP protocol, which diverts the IP traffic using announcements of IP prefixes to neighbor ASes. They show that the centralization of the Bitcoin network makes it possible for a single AS to intercept 50\% of traffic by hijacking only about 800 BGP prefixes. The authors also discuss variations of the attack differing in visibility and effectiveness and propose countermeasures.

\medskip
\noindent{\emph{Paper strengths:}} \\
- Insight into the power of BGP hijacking attacks in the application to Bitcoin.\\
- A vast number of attacks with different profiles.\\
- Mining power centralization is taken into account.\\
- Detailed simulations.

\medskip
\noindent{\emph{Paper weaknesses:}} \\
- Bitcoin nodes behind NAT are not considered \reviewref{ans:nated-node}.\\
- BGP description is missing.

\medskip
\noindent{\emph{Additional comments for authors:}} The vast majority of Bitcoin nodes do not actually have a public IP and can not accept connections. As noted in Biryukov et al. ``Deanonymisation of clients in Bitcoin P2P network'', there are 10-12x more such nodes than regular ones, considered in this paper. Nevertheless, they can forward blocks and transactions. Thus even if you isolate public-IP nodes, the latter still may communicate through the NAT-hidden nodes. This will probably makes your attacks more difficult \reviewref{ans:nated-node}.

\medskip
\noindent{\emph{Comment after discussion:}} Please elaborate on how exactly the intercepting attack on Bitcoin would work. Do you break the miners-pool connections? Pool-Pool? Pool-Peer? Peer-peer? Note that in all cases but the last one the Bitcoin protocol is not used, and the number of 6000 nodes is irrelevant \reviewref{ans:confusion}. 

It is important to relate your attack to the following paragraph:
"In the centralized distribution, we attribute most of the
hash rate to few ASes. We attribute 92\% of the mining power
to pools and assume that the remaining 8\% is equally distributed
among all other nodes. We infer the distribution of
mining power among pools from [6], which contains statistics
sourced from the blockchain itself and refer to the first
week of Nov 2015. We assign pools to ASes using the public
IPs of the Stratum servers that are used by miners to connect
to those pools." Please elaborate how you got these IPs.

\medskip
\noindent{\emph{Response to rebuttal:}} The rebuttal addressed most the issues
I raised, though not to the sufficient detail due to the lack of space. The
authors should nevertheless elaborate on the attack description in the future
edit of the paper.

\textbf{After a very long discussion}, the paper was rejected because of: 1) a bit of overselling \reviewref{ans:overselling}; 2) the actual feasibility of the attack is in question \reviewref{ans:practicality}; 3) the reviewers do not believe that the pools have so weak connectivity in reality \reviewref{ans:multi-homing}.

I personally think that the paper will be a strong accept at a less competitive conference.

\newpage
%===========================================================================
\myitem{Review \#262C}
%---------------------------------------------------------------------------

\medskip
\noindent{\emph{Decision:}} 3. Weak reject (will not argue against)

\medskip
\noindent{\emph{Summary:}} Attackers can cause partitioning and other attacks on Bitcoin via BGP prefix hijacking.

\medskip
\noindent{\emph{Paper strengths:}} \\
- The P2P network is arguably the weak underbelly of cryptocurrencies, so network attacks deserve more research attention.\\
- There are several nice measurement results about the Bitcoin network, especially its centralization.\\
- Interesting simulation-based results on the time to recover from a partition.\\
- Good discussion of possible countermeasures.

\medskip
\noindent{\emph{Paper weaknesses:}}
The authors do not adequately justify their claim that hijacking hundreds of prefixes is feasible. The closest they come is in pointing out that BGPStream reported 1616 prefix hijacks in 6 months or ~8.8 per day. But it seems that the paper's attack would require hundreds of prefixes to be hijacked at the same time, which is orders of magnitude more than the reported rate \reviewref{ans:hijacking_many_pfxes}.

Most large miners run more than one node; in fact, they have geographically distributed setups. They do this to minimize latency, but it also helps resist partitions. This fact is also not considered \reviewref{ans:multi-homing}.

While the time to recover from a partition is important to know, the time to detect a partition is also important and should be considered. Exchanges and other entities have measures in place to freeze funds and minimize damage if a partition is detected. The authors should discuss in more detail how nodes might be able to detect a partition or other attacks.

Attacking mining pools might not be sufficient to isolate mining power, since miners can quickly switch to different pools.

\medskip
\noindent{\emph{Additional comments for authors:}} The summary of my comments above is that the paper seems to overstate the practical feasibility of the attack in various ways. It doesn't uncover any fundamental weakness of the protocol, but rather points out that a powerful adversary will be able to cause mayhem on the network. The crucial question for the paper, then, is just how powerful that adversary needs to be. While the paper goes a fair way toward answering this question using measurements and simulation, there are additional factors to be taken into account as pointed out above \reviewref{ans:overselling}.

The suggestion that "nodes should deploy anomaly detection mechanisms to
recognize sudden changes and alert operators" is a very good one. It would be nice to see a couple of such techniques prototyped and evaluated.

``Hosting all Bitcoin nodes in /24 would prevent such attacks at the cost of a marginal increase (1\%) of the total number of Internet prefixes.'' 1\% sounds like a pretty big increase.

A more equivalent but more scalable countermeasure can be found in 
``We show that a single AS could increase the orphan rate by a factor of 10 with respect to that of the current Bitcoin network, while the US could increase orphan rate up to 50\% and Germany up to 29\%.'' This statement was unclear at first. Clarity that you mean a single AS could increase it from 1\% to 10\%.

The number of prefixes that need to be hijacked when taking mining power into account is variously reported as 31\% and 37\%.

\medskip
\noindent{\emph{Response to rebuttal:}} After discussing the rebuttal with the
other reviewers, I'm unconvinced that the attack is as practically feasible as
the authors claim.

This paper makes a nice contribution, but the hyperbole detracts from its
value. My score is thus unchanged \reviewref{ans:practicality}.


\subsection{\textbf{Reviews from USENIX Security 2016}}

\myitem{Review \#52A}

\medskip
\noindent{\emph{Decision:}} 3. OK paper. I hope we can find better papers to accept.

\medskip
\noindent{\emph{Expertise:}} 3. Knowledgeable

\medskip
\noindent{\emph{Summary:}} This paper studies AS-level network disruption attacks on Bitcoin.

\medskip
\noindent{\emph{Paper strengths:}} This is an interesting, messy layer of Bitcoin that hasn't been studied in detail and there are some interesting conclusions and a good list of countermeasures is proposed. This paper serves reasonably well as a taxonomy of routing attacks on Bitcoin and countermeasures.

\medskip
\noindent{\emph{Paper weaknesses:}} The analysis is not very deep. In particular, I think the paper took the tack of trying to claim very powerful attacks are possible to make it look like a surprising result is being had here, at the expense of a balanced investigation into what kinds of attacks are possible or likely \reviewref{ans:overselling}. Lots of more subtle attacks aren't really analyzed.

\medskip
\noindent{\emph{Comments for authors:}} Most of the attacks here are
conceptually known in the Bitcoin community and it is not surprising that major
ASes could wreak havoc on Bitcoin if the desired. This is a very powerful
adversary (an AS willing to risk it's reputation by performing network
manipulation) and it's not clear an entity with this ability would want to do
this \reviewref{ans:practicality}.

In particular, the claims of ``only a few ASes need collude'' are somewhat weak
because these are huge ASes, e.g. Comcast. Does Comcast really want to risk a
major damage to its billion dollar business to fiddle with Bitcoin? These
attacks make more sense in the ``Goldfinger'' attack setting where the
attacker's goal is to take down Bitcoin for no monetary gain (e.g. a national
Chinese AS). They also probably could do this without sophisticated attacks and
this isn't surprising. Furthermore, Bitcoin would likely adapt \reviewref{ans:overselling}.

I think it would have been much more compelling to focus the paper not on what
a small coalition of the most prominent ASes could achieve (who are highly
unlikely to attack) but a smaller AS (or group) which is more reasonable to
assume would go rogue. I think this is a major drawback of this paper, as it
really only focuses on what the most powerful attackers could do \reviewref{ans:overselling}.

While this paper assumes a powerful attacker, it then makes very generous
assumptions about the Bitcoin network being highly connected. I understand the
authors did not crawl the Bitcoin network to observe its actual topology, but I
have no idea why they didn't just simulate a random network with Bitcoin's
degree of connectivity, which is what Bitcoin is meant to create anyways \reviewref{ans:multi-homing}.

The assumptions about the distribution of mining power were also somewhat
simplistic. I think it would have been very intersting to assume that certain
pools are actually multi-homed at different nodes and see how that affects
things. This is clearly the next step in how mining pools will adapt to routing
attacks \reviewref{ans:multi-homing}.

This paper misses quite a few types of attacks to discuss. Most prominently, an
AS could attack while new nodes are joining the network (or finding peers) to
try to ``shape'' the network. I was disappointed to see this possibility not
mentioned in the paper.

The discussion of partition attacks was very simplistic. A true partition
attack is probably impossible as all it takes is one node which is multi-homed
and relaying data between the partitions on a covert channel. The paper ignores
such dedicated ``relay networks'' based on a very shaky assumption in the
appendix that they could also be attacked. These are much easier however to
hide and move around and avoid attacks, I think it would be quite hard to block
all of them \reviewref{ans:practicality}.

Given that a full partition would probably not be stable, the paper fails to
provide a more nuanced discussion of what can be done with a near partition. In
particular, such an attacker can still delay propagation significantly and can
frontrun transactions and block (e.g. see transactions and replace them with
competing transactions) with high success. Even without partitioning the
network, this is a powerful attack. It make selfish mining attacks and many
other approaches possible even without a complete partition. This is usually
modeled in more recent selfish mining papers by a parameter $\gamma$, measuring
the fraction of the network for which the attacker can replace a targeted
transaction/block \reviewref{ans:practicality}.

With all of these limitations, the analysis in the paper was not as compelling
as it could have been. I still think this is important work and with some
refinement this will be a very strong paper, the modeling is just a bit simple
right now.

%===========================================================================
\myitem{Review \#52B}
%---------------------------------------------------------------------------
%---------------------------------------------------------------------------

\medskip
\noindent{\emph{Decision:}} 2. Weak paper. This paper should be rejected but I will not fight strongly against it.
                
\medskip
\noindent{\emph{Reviewer expertise:}} 4. Expert

\medskip
\noindent{\emph{Summary:}} This paper describes two attacks on Bitcoin based on
network concentration, assuming real world AS topology and IP usage, but
synthetic mining power distribution.

\medskip
\noindent{\emph{Paper strengths:}} Use of real world network topologies for
evaluating attacks is an excellent approach.

\medskip
\noindent{\emph{Paper weaknesses:}} The mining power distribution is the big
question: Mining power is known to be heavily concentrated in the hands of a
few players, but at the same time the miners, since they are negatively
effected by the attacks more than any other paper \reviewref{ans:multi-homing}.

Rather esoteric in actual practice, it may be more appropriate for a narrower
interest conference.

\medskip
\noindent{\emph{Comments for authors:}} You correctly flag that mining
distribution is the key parameter to evaluate the actual practicality of these
attacks, but at the same time, you simply state that it is a ``hard problem''
and use synthetic data. 

This paper would be much better if you solved that ``hard'' problem, because that problem is not that hard. Most miners advertise in the blocks themselves that they are responsible for discovering in the coinbase (it acts as both advertising and is commonly used for voting as well). So you can use that to mostly model the actual distribution of miners \reviewref{ans:multi-homing}.

Similarly, by crawling the Bitcoin network, you can also identify the set of
nodes responsible for creating these blocks. Yes, you won't always see the
origin IP for any given block, but you can take advantage of this
centralization and, by acting as a heavy block propagator in your network, also
exclude nodes as possible sources. Using this, you should be able to do a much
better evaluation of how the Bitcoin network generates new blocks \reviewref{ans:multi-homing}.

This would also be interesting from a social/measurement standpoint, since my
hunch is that ``the miners are Chinese, the users are American'', and this
would allow you to evaluate this maxim to see if it is true.

There is also, as a consequence of centralization, another defense to your
block slowing attack: The few centralized miners could run a few additional
scattered nodes, and maintain VPN tunnels to these nodes (so an adversary can't
see the traffic and the nodes can know if the trafic is being delayed or
disrupted by including heartbeats in the VPN), with these nodes acting to
aggressively rebroadcast blocks they discover. Since this also acts to reduce
the problem of orphan blocks for the miners, this provides a benefit even in
the absence of a routing attacker \reviewref{ans:multi-homing}.

I also think this would be better suited for a more narrowly focused
conference: This work isn't applicable to other networks, or necessarily even
other crypto-currencies, as it largely depends on:

\noindent1:  The deep centralization present in Bitcoin;\\
2:  The ability to easily distinguish Bitcoin traffic;\\
3:  The economic motivation present in Bitcoin to launch such an attack \reviewref{ans:bitcoin-specific}.

==> sp copy/small_summary.tex <==
%preamble 
\section{Routing attacks on Bitcoin}
\label{sec:summary}

In this section we give an overview of the various network attacks that we
consider in this paper (see Fig.~\ref{fig:taxonomy}). 

\myitem{Attacker model:} We consider that an AS-level attacker can \emph{only}
manipulate ``pure'' bitcoin connections and assume that mining pools can use
\emph{any} proprietary, secure and private protocol internally. The attacker
aims at disrupting either a given set of nodes ranging from a single node to
nodes controlling 50\% (or more) of the mining power. In the case of attacks
against mining power, the attacker should know at least some of the gateways.
We explain in Section~\ref{} how an attacker can discover these gateways using
publicly known information such as Stratum servers. The overall attack is split
into consecutive steps. In Step 1 (\textbf{[S1]}), the AS-level attacker
performs a hijack or leverage natural routing (if possible) to intercept the
relevant Bitcoin traffic (Section~\ref{ssec:summary_intercept}). After that, in
Step 2 (\textbf{[S2]}), the attacker either: \emph{(i)} isolates the set of
nodes (\textbf{[A1]}); or \emph{(ii)} delay the delivery of blocks towards them
(\textbf{[A2]}).

%the AS-level attacker exploits access this Bitcoin traffic to disrupt either a small set of nodes or the system as a whole (Section~\ref{ssec:summary_attack}).

\begin{figure}[t]
 \centering
 \includegraphics[width=\columnwidth]{figures/summary_figure}
 \caption{Illustration of how AS-level adversaries can intercept Bitcoin traffic by hijacking prefixes or leveraging natural connectivity and then attacking either specific nodes of the network as a whole. \laurent{Update caption}}
 \label{fig:overview}
\end{figure}

We now illustrate how each steps of the routing attacks work along with the
potential impact for Bitcoin. As an illustration, we consider a simple example
(Fig.~\ref{fig:overview}). Bitcoin nodes are connected to AS1, AS2, AS3, AS4,
AS5 and AS6. Each AS\emph{X} advertise one IPv4 prefix: \emph{X}.0.0.0/16. For
instance, AS1 advertises 1.0.0.0/16. Two mining pools are depicted as a green
(left) and a red (right) region. Both pools are multi-homed: they have gateways
in more than one AS. For instance, the right pool is hosted in 3 ASes, AS4,
AS5, AS6 hosting its gateways nodes, I, J, F.


%We start by describing how the attacker can get on path and discusses how does
%the attacker figures out what to hijack later.

\subsection{\textbf{[S1]} Intercepting Bitcoin traffic}
\label{ssec:summary_intercept}

Routing attacks are performed either by \emph{passive attackers} who intercept
Bitcoin traffic naturally, or by \emph{active attackers} who perform BGP
hijacks to actively get on path. Passive attackers are usually the direct
providers of the bitcoin nodes whose traffic they intercept or large,
well-established ASes that are crossed by many connections. Passive attackers
are only effective against specific connections but they can act almost
invisibly on them. For instance, AS3 can intercept the connections from node J
to nodes A and B but not from node J to node H. In contrast, the effectiveness
of active attackers grows as they increase the number of prefixes they hijack,
but their attack is highly visible. For instance AS8 could hijack 1 prefix to
intercept all traffic destined to bitcoin nodes A and B, except the traffic
between them.

\subsection{\textbf{[S2]} Attacking Bitcoin consensus}
\label{ssec:summary_attack}

Once on-path, AS-level adversaries can fiddle with Bitcoin connections by
arbitrarily dropping, delaying or even modifying the messages exchanged. We
consider two different attacks (\textbf{[A1]} and \textbf{[A2]}) against
Bitcoin by either partitioning a subset of the Bitcoin network or by delaying
the propagation of blocks. The two attacks offer different tradeoffs in terms
of effectiveness (measured in the amount of disruption they can create), the
amount of connection they require to intercept and the visibility in doing so
(which correlates with how likely is the attacker to be discovered).

\myitem{[A1] Partitioning: highly disruptive, at the node \emph{and} network-wide level; require full interception; highly visible.}
The goal of this attack is to isolate a set of nodes from the Bitcoin network
such that no information can flow between them. To do so an attacker should
intercept and cut or filter \emph{all connections} from the isolated set of
nodes to the rest of the network. The difficulty of performing this attack
depends on the target (node-level or network-wide) and especially the type of
bitcoin clients (simple client or gateways large mining pools).

Isolating small set of nodes (or a single node) is relatively easy and can be
performed by active attackers, located anywhere, or by passive attackers which
happen to be crossed by all connections naturally. For instance, AS4 can
isolate node J from the network by cutting all its connections or by filtering
incoming information from the network. The same result can be accomplished by
the active attacker AS8 hijacking J's prefix.

In contrast, isolating a large set of nodes or large mining pools is
considerably harder considering the presence of multi-homed mining pools, NATed
nodes and relays. Only an active attacker can overcome these difficulties as
passive attackers (even when considering country-wide coalition) are unlikely
to be on-path for enough connections. To isolate the one or more muti-homed
mining pools, an active attacker can hijack the prefixes pertaining to all the
gateways. We discuss in Section~\ref{} how an attacker can discover these
gateways automatically. Even when considering that mining pools can be gateways
in as many as 15 ASes, we show that isolating 50\% of mining power is within
reach of any active attacker hijacking less than 400 prefixes.

In Section~\ref{sec:bitcoin_interception}, we also investigate on how an active
attacker can encompass other challenges such as limiting the amount of diverted
traffic. We also investigated the long term influence of a 50\%-50\% partition
after the hijack has been mitigated in a testbed of 1050 nodes running the
default bitcoind (Section~\ref{fig:partition}). We show that the Bitcoin network almost heals immediately from a partition attack in the sense that consensus is quickly reached again once the partition starts to leak, i.e. whenever (even few) connections start bridging the once-disconnected components. 

%Despite this, it takes a lot of time for the isolated components to re-establish connections to each
%other nodes within them reach consensus almost immediately.

\myitem{[A2] Delaying propagation: disruptive, mainly for targeted attacks;
works with partial interception; invisible.} The goal of this attack is to
eclipse nodes by delaying the delivery of blocks to them, without disrupting
their connections or actively connecting to them. Delay attacks can be
performed by both active and passive attackers. Yet, they are more likely to be
adopted by the former as they are invisible and effective \emph{even} if the
attacker intercept parts of the victim's traffic. As an illustration, AS3 can
successfully eclipse node J even though it does not intercept all of its
connections. If J receives an \textsf{INV} message for a new block from nodes A
B and H and either A or B advertised the block before H then AS3 can delay its
delivery for 20 minutes, effectively eclipsing J. This is in practice a more
complicated procedure requiring the attacker to fiddle with both the TCP and
the Bitcoin protocol to avoid detection and disconnection. We verified the
practicality of the attack by implementing a complete prototype which we use to
attack our own bitcoin nodes and found that an attacker can eclipse a victim
for 63\% of its uptime even when intercepting half of its connections (see
Section~\ref{sec:delay}).

We further evaluated the effectiveness of delay attacks when performed
network-wide using a realistic simulator. We found that the effectiveness of
delay attacks decreases with the degree of multi-homing adopted by the mining
pools. Indeed, we show that even the most powerful passive attacker, i.e. a
country-wide coalition of all the US-based networks together, cannot cause
considerable damage to the network if each of the main pools is hosted in at
least 5 ASes.

\subsection{\textbf{[S2]} Impact on Bitcoin}
\label{ssec:summary_impact}

The impact of the attack varies with respect to the number and type of the impacted bitcoin nodes. At the node-level such attacks can keep the victim eclipsed, essentially performing a successful denial of service attack or rendering it vulnerable to 0-confirmation double spends. If the node is a gateway of a pool such attacks can be used to engineer block races.
Network-wide attacks such as a isolating a considerable amount of mining power or sufficiently delaying the propagation of blocks to increase the fork rate renders the network extremely vulnerable to all sorts of exploits. As a sufficient number of blocks are discarded, the  miner's revenue is deducted and the network is more vulnerable to double spends. Especially in the case of the partition, all transactions included in the chain of the side with the least mining power are likely to be reversed. In the case of delaying, significant slowdown of block transmission can be used to launch selfish mining attacks by adversaries with mining power.


==> sp copy/topology.tex <==
\section{How vulnerable is Bitcoin to routing attacks? A comprehensive measurement analysis}
\label{sec:topology}

Evaluating the impact of routing attacks requires a good understanding of the
routing characteristics of the Bitcoin network. In this section, we explain the
datasets and the techniques used to infer a combined Internet and Bitcoin
topology (Section~\ref{ssec:topo_datasets}). We then discuss our key findings and their impact on the effectiveness of the two routing attacks we consider (Section~\ref{ssec:topo_findings}). 

\subsection{Methodology and datasets}
\label{ssec:topo_datasets}

Our study is based on three key datasets: \emph{(i)} the IP addresses
used by Bitcoin nodes and gateways of pools; \emph{(ii)} the portion of mining power each pool possesses; \emph{(iii)} the forwarding path  taken between any two IPs.
%
While we collected these datasets over a period of 6 months, starting from
October 2015 through March 2016, we focus on the results from a 10
day period starting from November 5th 2015, as the results of our analysis do not
change much through time.

\remove{
\begin{figure}[t]
 \centering
 \includegraphics[width=.65\columnwidth]{figures/method_topo}
 \caption{Summary of our methodology for inferring the network characteristics of the Bitcoin topology based on network and Bitcoin data.}
 \label{fig:method}
\end{figure}
}

% Using a Bitcoin super-node.

\myitem{Bitcoin IPs} We started by collecting the IPs of regular nodes (which
host no mining power) along with the IPs of the gateways the pools use to connect to the network. We gathered this dataset
by combining information collected by two Bitcoin supernodes with publicly available
data regarding mining pools. One supernode was connected to {\raise.17ex\hbox{$\scriptstyle\sim$}}2000 Bitcoin nodes per day, collecting  block propagation information, while the other was crawling the Bitcoin network, collecting the {\raise.17ex\hbox{$\scriptstyle\sim$}}6{,}000 IPs of active nodes each day.


%\emph{(i)} using block propagation information crawled from a supernode;
%and \emph{(ii)} considering the location of their (publicly known) Stratum
%server.
We inferred which of these IPs act as the gateway of a pool in two steps.
\emph{First}, we used block propagation information (gathered by the first supernode), considering that the gateways of a pool are most likely the
first to propagate the blocks this pool mines. Particularly, we
assigned IPs to pools based on the timing of the \textsf{INV} messages received
by the supernode. We considered a given IP to belong to a gateway
of a pool if: \emph{(i)} it relayed blocks of that pool more than once during
the 10 day period; and \emph{(ii)} it frequently was the first to relay a block of
that pool (at least half as many times as the most frequent node for
that pool). \emph{Second}, we also considered as extra gateways the IPs of the
stratum servers used by each mining pool. Indeed, previous
studies~\cite{miller2015discovering} noted that stratum servers tend to be
co-located in the same prefix as the pool's gateway. Since the URLs of the
stratum servers are public (Section~\ref{sec:background}), we simply resolved
the DNS name (found on the pools websites or by directly connecting to them)
and add the corresponding IPs to our IP-to-pool dataset.

\myitem{Mining power} To infer the mining power attached to pools, we
tracked how many blocks each pool mined during the 10 days
interval~\cite{blockchain} and simply assigned them a proportional share of the
total mining power.

\myitem{AS-level topology and forwarding paths} We used the AS-level topologies
provided by CAIDA~\cite{caida_as_level} to infer the forwarding paths taken
between any two ASes. An AS-level topology is a directed graph in which a
node corresponds to an AS and a link represents an inter-domain connection
between two neighboring ASes. Links are labeled with the business relationship
linking the two ASes (customer, peer or provider). We computed the actual
forwarding paths following the routing tree algorithm described
in~\cite{goldberg_how_secure_are_interdomain_routing_protocols} which takes
into account the business relationships between ASes.

\remove{
We build a model of the Internet topology by processing more than \emph{2.5 million} BGP routes (covering all Internet prefixes) along with \emph{4 billion} BGP updates advertised on 182 BGP sessions maintained by 3 RIPE BGP collectors~\cite{ripe:ris} (rrc00, rrc01 and rrc03). We collected these routes and updates daily, for 4 months, between Oct 2015 and Jan 2016.
}

%Using this data, we identified which AS is hosting each Bitcoin node by mapping
%its IP address with the AS advertising the most-specific covering prefix. To
%protect our mapping from BGP hijacks, we only consider prefixes that have been
%advertised consecutively for at least one day. We then computed the sequence of
%ASes traversed when any two Bitcoin nodes communicate. 

\myitem{Mapping Bitcoin nodes to ASes} We finally inferred the most-specific
prefix and the AS hosting each Bitcoin node by processing more than \emph{2.5
million} BGP routes (covering all Internet prefixes) advertised on 182 BGP
sessions maintained by 3 RIPE BGP collectors~\cite{ripe:ris} (rrc00, rrc01 and
rrc03). The mapping is done by associating each prefix to the origin AS
advertising it and by validating the stability of that origin AS over time
(to avoid having the mapping polluted by hijacks).

%Grouping such results enabled us to see the general
%characteristics of the Bitcoin topology with regard to the centrality and
%routing. In addition to that, we inferred some of the gateways and observed
%their practices with regards to networking.


%% LV: I removed the table as we need the space (findings are already described in bold in the text.)
\remove{
\begin{table}[t]
\centering
\small
\def\arraystretch{1}
\begin{tabular}{@{}lclcl@{}}
\toprule
%Attack && Active(How much) && Passive(Who can) &&  \% ForkRate && Implications\\
\emph{Observation} && \emph{for partition}  && \emph{for delay}   \\
\midrule
>90\% of nodes in short prefixes && Good && Good  \\
Concentration in AS hosting && Bad && Good \\
Concentration in AS paths && - && Good  \\
Destributed/Muti-homed pools && Bad && Bad  \\

\bottomrule
\end{tabular}
\caption{We summarize here the relevant network characteristics of the Bitcoin network as well as their consequences with regards to our attacks. Bad means that it makes the attack more difficult and good easier. }
\label{tab:insides}
\end{table}
}

\subsection{Findings}
\label{ssec:topo_findings}

We now discuss the key characteristics of the Bitcoin network from the Internet routing perspective. We explain which of them constitute enablers or hindrances for an AS-level attacker. %We summarize our observations together with their impact partition and delay attacks in Table~\ref{tab:insides}.

\remove{
\begin{table}[t]
\centering
\small
\def\arraystretch{1.1}
\begin{tabular}{@{}lccccc@{}}
\toprule
%Attack && Active(How much) && Passive(Who can) &&  \% ForkRate && Implications\\
\textbf{Degree of multi-homing} && {\emph{1}} & \emph{5} & {\emph{10}} & \emph{15} \\
\color{gray}{\# ASes used to access the Bitcoin network} && & & & \\
\midrule
\textbf{F2Pool} && 1 & 10 &  16 & 22  \\
\textbf{AntPool} && 1  & 8 &  17 & 23 \\
\textbf{Bitfurry} && 1  & 5 &  13 & 19  \\
\textbf{BTCC}  && 1 & 6 &  11 & 17  \\
\bottomrule
\end{tabular}
\caption{Number of gateways for each of the four biggest pools as a function of the degree of multi-homing they adopt.}
\label{tab:ips}
\end{table}






\begin{figure}[t]
 \centering
 \includegraphics[width=.65\columnwidth]{figures/nb_hijacks_required_pools}
 \caption{The number of prefixes to hijack needed to isolate a mining pool increases as they get better connected. Yet, hijacking only 246 prefixes is enough to isolate F2Pool, the largest pool with 21\% of the mining power. Overall, hijacking less than 400 prefixes is needed to isolate 50\% of the mining power assuming pools are multi-homed in 15 ASes. This is \emph{well} within what is currently seen in the Internet (see Fig.~\ref{fig:hijack_number}).}
 \label{fig:

 interception_pools}
\end{figure}
}
%%
%%
%%%% SECTION BEGINNING
%%
%%
\remove{
Here we key-characteristics of the Bitcoin network that enable passive and active attackers to intercept a large amount of Bitcoin traffic ~\ref{ssec:bitcoin_topology}. As passive adversaries have no control of which connections they will intercept, we elaborate only on how active adversaries can pick a suitable set of prefixes to hijack to increase their effectiveness in ~\ref{ssec:active_interception_attacks}.



\subsection{Measurement analysis}
\label{ssec:bitcoin_topology}

}

\myitem{A few ASes host most of the Bitcoin nodes} Fig.~\ref{fig:cdf_bitcoin_per_ases} depicts the
cumulative fraction of Bitcoin nodes as a function of the number of hosting
ASes. We see that only 13 (resp. 50) ASes host 30\% (resp. 50\%) of the entire
Bitcoin network. %Table~\ref{tab:ases_number_ranking} lists the top 10 ASes in terms of
%hosted number of nodes. 
These ASes pertain to broadband providers such as Comcast (US), Verizon (US) or Chinanet (CN) as well as to cloud providers such as Hetzner (DE), OVH (FR) and Amazon (US). We observe the same kind of concentration when considering the distribution of Bitcoin nodes per IP prefix: only 63 prefixes
(0.012\% of the Internet) host 20\% of the network.

Regarding delay attacks, this high concentration makes Bitcoin traffic more
easy to intercept and therefore more vulnerable. With few ASes hosting many
nodes, any AS on-path (including the host ASes) is likely to intercept many
connections at once, making delay attacks more disruptive. Regarding partition
attacks, the effect of the concentration is a bit more nuanced. Indeed, high concentration reduces the total number of feasible partitions because of intra-AS connections that cannot be intercepted (Section~\ref{ssec:hidden}). At the same time, tough, the remaining feasible partitions are much easier to achieve since they require fewer hijacked prefixes (Section~\ref{sec:partition}).

%Specifically, since hijacking few IP prefixes is needed to intercept many
%connections, performing a disruptive partition attack requires less resource.
%On the other hand, as intra-AS connections cannot be intercepted , attackers
%cannot split these nodes apart and instead mandates the attacker to isolate
%whole ASes from the rest of the network.

\begin{figure}[t]
 \centering
 \begin{subfigure}[t]{0.47\columnwidth}
\includegraphics[width=.9\columnwidth]{figures/bitcoin_per_ases_cummulative}
	 \caption{Only
13 ASes host 30\% of the entire network, while 50 ASes host 50\% of the Bitcoin
network.}
	 \label{fig:cdf_bitcoin_per_ases}
 \end{subfigure}
 \hfill
 \begin{subfigure}[t]{0.47\columnwidth} 	\includegraphics[width=.9\columnwidth]{figures/crossed_connections_per_as_cummulative}
	 \caption{Few ASes intercept large percentages of Bitcoin traffic: 3 of them intercept 60\% of all possible Bitcoin connections.}
	 \label{fig:cdf_connection_per_ases}
 \end{subfigure}
 \caption{Bitcoin is heavily centralized from a routing viewpoint.}
 \label{fig:centralization}
\end{figure}
%(Hurricane, Level3 and Telianet)

\myitem{A few ASes naturally intercept the majority of the Bitcoin traffic}
Large transit providers (\emph{i.e.}, Tier-1s) tend to be traversed by a large fraction of all the Bitcoin connections.
Fig.~\ref{fig:cdf_connection_per_ases} depicts the cumulative percentage of
connections that can be intercepted by an increasing number of ASes
(\emph{e.g.}, by colluding with each other). We see that only \emph{three}
ASes, namely Hurricane Electric, Level3, and Telianet, can together intercept
\emph{more than 60\% of all possible Bitcoin connections}, with Hurricane alone
being on path for 32\% of all connections. %In general, large transit
%providers (\emph{i.e.}, Tier-1s) are traversed by a large fraction of all Bitcoin connections.

Regarding delay attacks, these few ASes could act as powerful delay attackers.
Regarding partition attacks, this observation does not have any direct
implication as partitioning requires a \emph{full} cut to be effective
(Section~\ref{sec:partition}).

%Table~\ref{tab:ases_ranking_connections} lists the top 7 ASes in terms of the
%percentage of total connections they can intercept. We see that large transit
%providers (\emph{i.e.}, Tier-1s) are traversed by a large fraction of
%all Bitcoin connections.

\myitem{$>$90\% of Bitcoin nodes are vulnerable to BGP hijacks} 93\% of all
prefixes hosting Bitcoin nodes are shorter than /24, making them vulnerable to
a global IP hijack using more-specific announcements. Indeed, prefixes strictly
longer than /24 (i.e., /25 or longer) are filtered by default by many ISPs. Observe that the remaining 7\% hosted in /24s are \emph{not}
necessarily safe. These can still be hijacked by another AS performing a
shortest-path attack, i.e., the attacker, who will advertise a /24 just like
the victim's provider will attract traffic from all ASes that are closer to her in terms of number of hops.

While this finding does not have a direct impact on delay attacks, it clearly helps partition attackers as they can divert almost all Bitcoin traffic to their infrastructure (modulo stealth connections, see Section~\ref{sec:partition}).
%This will, on average, allow him to hijack traffic to the
%victim from around half of the internet.
 %(but really depends on the exact topology).

\myitem{Mining pools tend to be distributed and multi-homed}
Mining pools have a complex infrastructure compared to regular nodes.
We found that \emph{all} pools use at least two ASes to connect to the
Bitcoin network, while larger pools such as Antpool, F2Pools,
GHash.IO, Kano use up to 5 ASes. 

%Assuming that the exact topology can stay
%private and the protocols used for intra-pool communication is secured, 

Pool multi-homing makes both network attacks more challenging and is one of the
main precaution measures node owners can use against routing attacks. While harder, routing attacks are still possible in the presence of multi-homing as
we illustrate in Section~\ref{sec:delay_results}.

\myitem{Bitcoin routing properties are stable over time} While numerous nodes
continuously join and leave the Bitcoin network, the routing properties
highlighted in this section are stable. As validation, we ran our analysis
daily over a 4 month period. We found that the same IPs were present on average
for 15.2 consecutive days (excluding IPs that were seen only once). Moreover, 50 ASes hosted each day 49.5\% of Bitcoin clients (standard deviation: 1.2\%)
while 24.7\% of Bitcoin nodes are found daily in just 100 prefixes (standard
deviation: 1.77\%).







\remove{
\myit{Actively Interception attacks using centralization}
\label{ssec:active_interception_attacks}
%who?
In this section we show how an active or hybrid adversary can overcome the challenges of multi-homing, NATed nodes, and relays as well as reduce the cost of the attack in diverted bandwidth and number hijacked of prefixes. 
%how

We particularly focus on a 50\% partition, intuitively any smaller partition is easier to create.





Active attackers are able to completely isolate
any set containing regular nodes or/and multi-homed pools, effectively creating a 
partition of nodes or mining power respectively even as large as 50\%. 
For isolating any set of regular nodes an AS adversary would need to 
intercept all their traffic. By hijacking all the prefixes of these nodes the attacker 
intercept all traffic destined to them. As such the attacker can simply prevent them 
from connecting to any node outside the set.
For isolating a pool an attacker needs to make sure  all  
gateways of a pool are hijacked. For that an AS adversary would need to know all gateways belonging to the pools he wants to include in the isolated set. 




After ensuring a complete cut between the two parts The attacker's goal is to lower its footprint,
\emph{i.e.} the amount of prefixes hijacked. In the following we explain the methodology we used to estimate the smallest amount of prefixes needed to create partitions of diffrent sizes.
We always consider
the
extreme case, in which the AS-level adversary: \emph{i)} does not see \emph{any} traffic
naturally; and \emph{ii)} does not host any Bitcoin nodes.
Especially for the partition of mining power we further investigate the influence of multi-homing degree per pool in the cost of such a partition.


 }


\remove{
\myitem {Estimating the cost of isolating mining power.}
For each mapping of IPs to a pool we calculate the cost of isolating it in number of prefixes 
that need to be hijacked. The exact results for the four biggest pools under five 
assumptions regarding the degree of multi-homing are 
presented in Table~\ref{tab:hijacks50}  Due to the concentration of Bitcoin from the 
routing perspective we found 
significant overlap among the required hijacked prefixes to isolate distinct pools. As such 
the cost of a largest partition is considerably limited in comparison to the sum of prefixes 
required per pool. We present the results for partitions containing from 49\% to 50\% of mining power. Intuitively there are smaller partitions that require  require less prefixes. We calculated these numbers using exhaustive search over all the subsets of pools partitions of 49\% to 51\% and picked the one with the least required prefixes. We found that 
only 381 prefixes needed to be hijacked even in the extreme case that the four biggest 
pools accounting for almost 70\% of mining power are hosted in 15 ASes each. When considering lower degree of multi-homing such as 5 ASes per pool  the number is reduced to half.

\myitem {Estimating the cost of isolating regular 
nodes.} For each AS with Bitcoin nodes we assign a score that equals to the ratio of the number of nodes nodes it
contains over the number of prefixes with Bitcoin nodes it advertises. The
attacker then hijacks the ASes with the higher scores first. We found that \emph{870 prefixes} need to be hijacked to isolate 50\% of the public Bitcoin nodes while 119 hijacked [refix would isolate 20\% of the public Bitcoin nodes.% until reaching 50\% of all mining power.



\myitem{Dealing with hijacked bandwidth}
While deciding the right prefixes to hijack an attacker should also take bandwidth demands associated with the hijacked prefixes into consideration. In light of that the attacker might prefer to increase the hijacked prefixes to decrease the traffic that would be diverted to his infrastructure even if such a practice requires hijacking more prefixes. 
Going back to our example in figure ~\ref{fig:overview} if AS8 can indeed hijack one prefix namely 1.0.0.1/16 to intercept all traffic destine to nodes A and B. In this case the attacker would have to deal with all the traffic destined to a /16 prefix. However if A and B belong to a common more specific prefix then an attacker would for sure prefer to hijack this one as the diverted load would be less. The attacker can reduce the load even further by advertising only /24 prefixes even if that means he needs to advertise more prefixes. 

 \laurent{Rephrase the above in lights of the hijack study}.




%Indeed, almost of all of the mining power
%is distributed in only 20 pools, 7 of which together reach 88\%. From the
%network perspective, mining pools are \emph{even more centralized} with 15 ASes
%(in the \emph{distributed} case) or 13 (in the \emph{centralized} case) hosting
%90\% of mining power.



\myitem{Hybrid attackers} 
%
In practice, nothing prevents AS-level adversaries to combine active and passive
attacks to reduce their footprint even
further. To give an idea of such approach we present what the cost of creating the same partitioning would be if performed by the AS that was harder to hijack  (require more prefixes). For isolating 50\% of the nodes , X
prefixes are enough for a hybrid attacker. For isolating 50\% of mining power a hybrid attacker would need 13, 123,253 and 337 prefixes under the assumption that mining pools are hosted at most at 1,5,10 and 15 ASes respectively.  







\begin{table}[t]
	\centering
	\small
	\def\arraystretch{1.1}
	\begin{tabular}{@{}lclcccc@{}}
		\toprule
		\cmidrule(lr){5-6}
		\textbf{Country} && \textbf{Connections} (\%) && \emph{Partition regular nodes} \\			
		\midrule
		US && 89.8 && 37.0 \\
		DE && 32.8 && 8.8  \\
		GB && 31.4 && 5.4  \\
		SE && 26.7 && 2.0  \\
		CN && 12.2 && 5.4  \\
%		HK && 11.3 && 0.7 && 0.0 \\
		\bottomrule
	\end{tabular}
	\caption{Cumulated power ASes in the same country have over Bitcoin measured in \% of connections they intercept and the most disruptive partition of regular nodes they can achieve. \laurent{Update results} %Values are computed assuming a complete graph ie each node is connected to every other  
	}
	\label{tab:country_partition}
\end{table}

}
\remove{
\remove{ with
{\raise.17ex\hbox{$\scriptstyle\sim$}}70\% of the mining power held by four
mining pools: F2Pool (21\%), AntPool (19\%), Bitfurry (15\%) and BTCC
(13\%).
}

\myitem{Bitcoin INV Messages} To infer the pool gateways we analyzed the INV messages advertising blocks which received by a super nodes. This node was connected to approximately 2{,}000 Bitcoin nodes per day (with a mean of 2174 and a median of 1875). It saw a total of 7{,}477 distinct IPs during the 10 days and was relayed a total of 1{,}440 blocks. We assigned to a pool based on how frequent this node was the first to advertise a block mined by this pool. 



By combining this dataset with the BGP one, we then created  node-to-AS mapping
each Bitcoin IP address to the origin AS advertising the most-specific prefix
covering it, giving us a .
}



\remove{
Nexious :    #ases 1    #ips 1
GHash.IO :    #ases 4    #ips 9   1.7
NiceHash :    #ases 1    #ips 1
21 :    #ases 2    #ips 2 3.5
A-XBT :    #ases 2    #ips 2
BitMinter :    #ases 2    #ips 2
Telco :    #ases 2    #ips 2
unknown :    #ases 1    #ips 1
Slush :    #ases 2    #ips 2  6
Kano :    #ases 5    #ips 6
BW.COM :    #ases 2    #ips 2   5
AntPool :    #ases 4    #ips 7 20
EclipseMC :    #ases 2    #ips 2  1.7
Bitcoin :    #ases 2    #ips 2
BitFury :    #ases 2    #ips 2  15
Eligius :    #ases 3    #ips 4
BTCC :    #ases 2    #ips 2
KnCMiner :    #ases 1    #ips 1
F2Pool :    #ases 3    #ips 6 21
BitClub :    #ases 2    #ips 2
}



